Generalization Guarantees for Neural Networks via Harnessing the Low-rank Structure of the Jacobian

Modern neural network architectures often generalize well despite containing many more parameters than the size of the training dataset. This paper explores the generalization capabilities of neural networks trained via gradient descent. We develop a data-dependent optimization and generalization theory which leverages the low-rank structure of the Jacobian matrix associated with the network. Our results help demystify why training and generalization is easier on clean and structured datasets and harder on noisy and unstructured datasets as well as how the network size affects the evolution of the train and test errors during training. Specifically, we use a control knob to split the Jacobian spectum into "information" and "nuisance" spaces associated with the large and small singular values. We show that over the information space learning is fast and one can quickly train a model with zero training loss that can also generalize well. Over the nuisance space training is slower and early stopping can help with generalization at the expense of some bias. We also show that the overall generalization capability of the network is controlled by how well the label vector is aligned with the information space. A key feature of our results is that even constant width neural nets can provably generalize for sufficiently nice datasets. We conduct various numerical experiments on deep networks that corroborate our theoretical findings and demonstrate that: (i) the Jacobian of typical neural networks exhibit low-rank structure with a few large singular values and many small ones leading to a low-dimensional information space, (ii) over the information space learning is fast and most of the label vector falls on this space, and (iii) label noise falls on the nuisance space and impedes optimization/generalization.

==> RadCompRowFro.tex <==
%\documentclass{article}
%%\title{End-to-end Training of a Non-Overlapping Convolutional Neural Network via Deep Tensor Decompositions}
%%\title{End-to-end Training of a Convolutional Neural Network\\via Deep Tensor Decomposition}
%%FastConvergence of 
%%\title{Solving Overparameterized or Overdetermined Least-Squares via Well-Conditioned Jacobian}
%%\title{Unified Approach to Overparameterized and Overdetermined Problems via Well-Conditioned Jacobian}%SGD 
%\title{%\LARGE{Fast Overparameterized Convergence:\\Gradient Descent Takes the Shortest Path}\\
%%Overparameterized Nonlinear Least-squares:\\
%Overparameterized Nonlinear Learning:\\
%Gradient Descent Takes the Shortest Path?
%%Gradient Descent Finds a Nearby Global Optima\\
%%Gradient Descent Finds a Global Optima in its Vicinity\\%\\
%%\MS{if we can prove the following}\\
%%Gradient Descent Finds a Nearby Global Optima by Taking the Shortest Path
%%Takes the Shortest Path
%}%/Overdetermined
%% or \title{End-to-end Learning of Convolutional Neural Networks\\via Deep Tensor Decompositions}
%
%\author{}
%%\date{}
%\pagestyle{plain}
%
%\input{notation}
%\usepackage{multirow}
%
%
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\title{Radamacher complexity of row bounded and Frobinus bounded}
%%\author{Mahdi Soltanolkotabi\\Ming Hsieh Department of Electrical Engineering\\University of Southern California, Los Angeles, CA, 90089}
%\date{March 2018}
%\begin{document}
%\maketitle

\section{Rademacher Complexity and Generalization Bounds}
%Population error can be upper bounded as
%\[
%\Lc_P(h)\leq \Lc_S(h)+2\Rc(
%\]
% parameterized by weights $\W$.
Let $\Fc$ be a function class. Suppose $f\in\Fc$ maps $\R^d$ to $\R^K$. Let $(\eps_{i,j})$ be i.i.d.~Rademacher variables. Given i.i.d.~samples $\Sc=(\x_i,\y_i)_{i=1}^n\sim \Dc$, we define the empirical Rademacher complexity to be
\[
\Rc_{\Sc}(\Fc)=\frac{1}{n}\E[\sup_{f\in\Fc} \sum_{i=1}^n \sum_{j=1}^\K \eps_{i,j} f_j(\x_i)]
\]
We first state a vector contraction inequality by Maurer \cite{maurer2016vector}. This is obtained by setting $h_i(f(\x_i))=h(\y_i,f(\x_i))$ in Corollary 4 of \cite{maurer2016vector}.
\begin{lemma} \label{lem multi}Let $f(\cdot):\R^d\rightarrow \R^\K$ and let $\ell:\R^\K\times \R^K\rightarrow\R$ be a $1$ Lipschitz loss function with respect to second variable. Let $(\eps_i)$'s be i.i.d.~Rademacher variables. Given i.i.d.~samples $(\x_i,\y_i)_{i=1}^n$, define
\[
\Rc_{\Sc}(\ell,\Fc)=\E[\sup_{f\in \Fc}\sum_{i=1}^n\eps_i \ell(\y_i,f(\x_i))].
\]
We have that
\[
\Rc_{\Sc}(\ell,\Fc)\leq \sqrt{2}\Rc_{\Sc}(\Fc).
\]
\end{lemma}

%\begin{lemma} Let $f(\cdot):\R\rightarrow \R$ and let $\ell_i:\R\rightarrow[0,1]$ be $1$ Lipschitz loss functions. Given i.i.d.~samples $(\x_i)_{i=1}^n$, consider the empirical loss
%\[
%\Lc(\ell,\W)=\frac{1}{n}\sum_{i=1}^n \ell_i(f(\x_i,\W)).
%\]
%With probability $1-\delta$ over samples, for all $f\in \Fc$, we have that
%\[
%\E[\Lc(\ell,\W)]\leq \Lc(\ell,\W)+2\Rc_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
%\]
%\end{lemma}
Combining above with standard generalization bounds based on Rademacher complexity \cite{bartlett2002rademacher} yields the following.
\begin{lemma} \label{standard rad}Let $\ell(\cdot,\cdot):\R^\K\times \R^\K\rightarrow [0,1]$ be a $1$ Lipschitz loss function. Given i.i.d.~samples $(\x_i,\y_i)_{i=1}^n$, consider the empirical loss
\[
\Lc(f,\ell)=\frac{1}{n}\sum_{i=1}^n \ell(\y_i,f(\x_i)).
\]
With probability $1-\delta$ over samples, for all $f\in \Fc$, we have that
\[
\E[\Lc(f,\ell)]\leq \Lc(f,\ell)+2\sqrt{2}\Rc_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
\]
\end{lemma}
\begin{proof} From \cite{bartlett2002rademacher}, we have that, with $1-\delta$ probability
\[
\E[\Lc(f,\ell)]\leq \Lc(f,\ell)+2\Rc_{\Sc}(\ell,\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
\]
We conclude by combining this with Lemma \ref{lem multi}.
\end{proof}

\begin{lemma} \label{rad rad bound}Let $\W\in\R^{k\times d}$ and $\Vb\in\R^{\K\times k}$ be input and output weight matrices respectively. Suppose $\tin{\Vb}\leq \sigma/\sqrt{k\K}$. Define the neural network function parameterized by input weights $\W$
\begin{align*}
f(\W,\vct{x})=\Vb\phi\left(\mtx{W}\vct{x}\right)
\end{align*}
Let $\W_0\in\R^{k\times d}$ be a reference input weight matrix. Define the function space
\begin{align}
\mathcal{F}_{\mathcal{W}}=\big\{f(\W,\vct{x})\quad\text{such that}\quad\W\in\mathcal{W}\big\}\quad\text{with}\quad\mathcal{W}=\big\{\W: \fronorm{\W-\W_0}\le M\quad\text{and}\quad \|\W-\W_0\|_{2,\infty}\le R\big\}\label{space func}
\end{align}
Let $(\xi_i)_{i=1}^n\in\R^\K$ be i.i.d.~vectors with i.i.d.~Rademacher entries. Consider empirical Rademacher complexity
\begin{align*}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right):=&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{f\in\mathcal{F}_{\mathcal{W}}}{\sup}\text{ }\sum_{i=1}^n \xi_i^Tf(\vct{x}_i)\Bigg].
\end{align*}
We have that %{\textcolor{red}{MOVE TO multiclass starting here!}} 
\begin{align}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right)\le  \sigma B(\frac{M}{\sqrt{n}}+R^2\sqrt{k})\label{emp rad comp}
\end{align} 
\end{lemma}
\begin{proof}
We shall use $\vct{w}_\ell$ to denote the rows of $\mtx{W}$ (same for $\W_0$ and $\Vb$). We will approximate $\phi\left(\langle \vct{w}_\ell,\vct{x}_i\rangle\right)$ by its linear approximation $\phi\left(\langle \vct{w}_\ell^0, \vct{x}_i\rangle\right)+\phi'(\langle\w_\ell^0,\vct{x}_i\rangle)\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)$ via the second order Taylor's mean value theorem. We thus have
\begin{align*}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right)\le&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\sum_{i=1}^n\xi^T_i\Vb\phi\left(\W_0\vct{x}_i\right)+\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n \xi^T_i\Vb\text{diag}\left(\phi'\left(\W_0\vct{x}_i\right)\right)\left(\W-\W_0\right)\vct{x}_i\Bigg]\\
&+\frac{1}{2n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k \sum_{j=1}^\K\xi^T_{i,j}\vct{v}_{j,\ell}\phi''\left((1-t_{i\ell})\langle\vct{w}_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\vct{w}_\ell,\vct{x}_i\rangle\right)\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)^2\Bigg]\\
=&\underbrace{\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n \xi^T_i\Vb\text{diag}\left(\phi'\left(\W_0\vct{x}_i\right)\right)\left(\W-\W_0\right)\vct{x}_i\Bigg]}_{\mathcal{R}_1}\\
&+\underbrace{\frac{1}{2n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k  \sum_{j=1}^\K\xi^T_{i,j}\vct{v}_{j,\ell}\phi''\left((1-t_{i\ell})\langle\vct{w}_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\vct{w}_\ell,\vct{x}_i\rangle\right)\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)^2\Bigg]}_{\mathcal{R}_2}
\end{align*}
We proceed by bounding each of these two terms. For the first term note that
\begin{align*}
\mathcal{R}_1\le& \frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\fronorm{\W-\W_0}\le M}{\sup}\text{ }\sum_{i=1}^n \xi^T_i\Vb\text{diag}\left(\phi'\left(\W_0\vct{x}_i\right)\right)\left(\W-\W_0\right)\vct{x}_i\Bigg]\\
\le& \frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\fronorm{\W-\W_0}\le M}{\sup}\text{ }\Big\langle\sum_{i=1}^n \text{diag}\left(\phi'\left(\W_0\vct{x}_i\right)\right)\Vb^T\xi_i\vct{x}_i^T,\W-\W_0\Big\rangle\Bigg]\\
\le&\frac{M}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\left(\sum_{i=1}^n \text{diag}\left(\Vb^T\xi_i\right)\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T\right)}\Bigg]\\
\le&\frac{M}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\left(\sum_{i=1}^n \text{diag}\left(\Vb^T\xi_i\right)\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T\right)}^2\Bigg]^{1/2}\\
=&\frac{M}{n}\Bigg[\sum_{i=1}^n\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\fronorm{ \text{diag}\left(\Vb^T\xi_i\right)\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T}^2\Bigg]^{1/2}\\
\le&\frac{M}{n}\Bigg[\sum_{i=1}^n\sum_{j=1}^\K\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\fronorm{ \diag{\xi_{i,j}\vb_j}\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T}^2\Bigg]^{1/2}\\
\le&\frac{M}{n}\Bigg[\sum_{i=1}^n\sum_{j=1}^\K\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\frac{\sigma^2}{k\K}\fronorm{\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T}^2\Bigg]^{1/2}\\
\le&\frac{M}{n}\Bigg[\sum_{i=1}^n\sum_{j=1}^\K\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\frac{\sigma^2}{k\K}B^2k\tn{\x_i}^2\Bigg]^{1/2}\\
\le&\frac{M}{n}(\sum_{i=1}^n\sum_{j=1}^\K \frac{\sigma^2}{{\K}}B^2\tn{\x_i}^2)^{1/2}\\
=&\frac{BM\sigma}{\sqrt{n}}.
%\le&\frac{M}{n}\infnorm{\vct{v}}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\sum_{i=1}^n \xi^T_i\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T}\Bigg]\\
%\le&\frac{M}{n}\infnorm{\vct{v}}\sqrt{\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\sum_{i=1}^n \xi^T_i\phi'\left(\W_0\vct{x}_i\right)\vct{x}_i^T}^2\Bigg]}\\
%=&\frac{M}{n}\infnorm{\vct{v}}\sqrt{\sum_{i=1}^n\twonorm{\phi'\left(\W_0\vct{x}_i\right)}^2\twonorm{\vct{x}_i}^2}\\
%\le& \frac{1}{\sqrt{n}}MB\sqrt{k}\infnorm{\vct{v}}
\end{align*}
For the second term note that
\begin{align*}
\mathcal{R}_2\le& \frac{1}{2n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\|\W-\W_0\|_{2,\infty}\le R}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k  \sum_{j=1}^\K\xi_{i,j}\vct{v}_{j,\ell}\phi''\left((1-t_{i\ell})\langle\vct{w}_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\vct{w}_\ell,\vct{x}_i\rangle\right)\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)^2\Bigg]\\
\le&\frac{1}{2n}\sum_{\ell=1}^k \E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\|\w_\ell-\w_\ell^0\|_{2,\infty}\le R}{\sup}\text{ }\sum_{i=1}^n \sum_{j=1}^\K|\xi_{i,j}\vb_{j,\ell}||\phi''\left((1-t_{i\ell})\langle\vct{w}_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\vct{w}_\ell,\vct{x}_i\rangle\right)|\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)^2\Bigg]\\
\le&\frac{1}{2n}\sum_{\ell=1}^k\sum_{i=1}^n  \E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}[|\sum_{j=1}^\K\xi_{i,j}\vb_{j,\ell}|]R^2B\\
\le&\frac{1}{2n}\sum_{\ell=1}^k\sum_{i=1}^n \frac{\sigma}{\sqrt{k}}BR^2\\
=&\frac{1}{2}BR^2\sigma\sqrt{k}
\end{align*}
Combining the bounds on $\mathcal{R}_1$ and $\mathcal{R}_2$ we conclude with \eqref{emp rad comp}.
\end{proof}
\begin{corollary} \label{generalize corollary}Let entries of the output layer $\Vb$ be equal to $\pm \sigma/\sqrt{kK}$. Define quadratic loss Let $\ell:\R^\K\times \R^\K\rightarrow [0,1]$ be a $1$ Lipschitz loss function satisfying $\ell(\x,\x)=0$. 
\[
\Lc(\W)=\frac{1}{n}\sum_{i=1}^n \tn{\y_i-f(\x_i,\W)}^2.
\]
Then for all $f\in \Fc$ given by \eqref{space func}, with $1-\delta$ probability, population loss for $\ell$, satisfying $\ell(\y,\y)=0$, obeys
\begin{align}
\E[\Lc(\ell,\W)]\leq \sqrt{\Lc(\W)}+ 2\sqrt{2}\sigma B(\frac{M}{\sqrt{n}}+R^2\sqrt{k})+\sqrt{\frac{5\log(2/\delta)}{n}}.\label{ell pop bound}
\end{align}
Suppose labels are one-hot encoded and thus unit Euclidian norm. Given sample $(\x,\y)\in\R^d\times \R^\K$, define the population classification error
\[
\err{\W}=\Pro(\arg\max_{1\leq i\leq K}\y_i\neq \arg\max_{1\leq i\leq K}f_i(\x,\W))
\]
We similarly have
\begin{align}
\err{\W}\leq 2\left[\sqrt{\Lc(\W)}+ 2\sqrt{2}\sigma B(\frac{M}{\sqrt{n}}+R^2\sqrt{k})+\sqrt{\frac{5\log(2/\delta)}{n}}\right].\label{err pop bound}
\end{align}
\end{corollary}
\begin{proof} Define empirical $\ell_2$ loss
\[
\Lc(\ell_2,\W)=\frac{1}{n}\sum_{i=1}^n\tn{\y_i-f(\x_i,\W)}.
\]
Using Cauchy-Schwarz, we have that $\sqrt{\Lc(\W)}\geq {\Lc(\ell_2,\W)}$.

Any 1-Lipschitz $\ell$ with $\ell(\y,\y)=0$ obeys $\ell(\y,\hat{\y})\leq \tn{\y-\hat{\y}}$ which implies 
\[
\Lc(\ell,\W)\leq \Lc(\ell_2,\W)\leq \sqrt{\Lc(\W)}.
\] Consequently, applying Lemmas \ref{standard rad} and \ref{rad rad bound} above, we find
\begin{align}
\E[\Lc(\ell,\W)]&\leq \sqrt{\Lc(\W)}+2\sqrt{2}\Rc_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}},\\
&\leq\sqrt{\Lc(\W)}+ 2\sqrt{2}\sigma B(\frac{M}{\sqrt{n}}+R^2\sqrt{k})+\sqrt{\frac{5\log(2/\delta)}{n}},
\end{align}
which yields the first statement.




To get the second statement on classification accuracy, pick the $\ell$ function to be 
\[
\ell(\y,\hat{\y})=\min(1,\tn{\y-\hat{\y}}).
\]
Note that, given a sample $(\x,\y)\in\R^d\times \R^\K$ with one-hot encoded labels, if $\arg\max_{1\leq i\leq K}y_i\neq \arg\max_{1\leq i\leq K}f_i(\x,\W)$ that implies 
\[
\ell(\y,f(\x,\W))\geq 0.5.
\] Using Markov inequality, this implies that, classification error obeys
\[
\err{\W}\leq 2\E_{(\x,\y)\sim\Dc}[\ell(\y,f(\x,\W))]=2\E[\Lc(\ell,\W)].
\]
Since $\ell$ is $1$ Lipschitz and bounded, it obeys \eqref{ell pop bound}, we find the bound on the population classification error \eqref{err pop bound}.
\end{proof}




%\begin{lemma} [Quadratic to $\ell_2$ loss] Define the quadratic loss
%\[
%\Lc(\W)=\frac{1}{2n}\sum_{i=1}^n\tn{\y_i-f(\x_i,\W)}^2.
%\]
%
%\end{lemma}
%\section{Simple}
%We shall use $\vct{w}_\ell^{0}$ to denote the rows of $\mtx{W}_0$. 
%Define
%\begin{align*}
%\mathcal{F}_{\mathcal{W}}=\big\{f(\vct{x})=\Vb\phi\left(\mtx{W}\vct{x}\right)\quad\text{such that}\quad\W\in\mathcal{W}\big\}\quad\text{with}\quad\mathcal{W}=\big\{\W: \fronorm{\W-\W_0}\le M\big\}
%\end{align*}
%Consider
%\begin{align*}
%\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right):=&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{f\in\mathcal{F}_{\mathcal{W}}}{\sup}\text{ }\sum_{i=1}^n \xi_if(\vct{x}_i)\Bigg].%\\
%%=&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{f\in\mathcal{F}_{\mathcal{W}}}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k \xi_i\vct{v}_\ell\phi(\langle\vct{w}_\ell,\vct{x}_i\rangle)\Bigg]\\
%%=&\frac{1}{n}\sum_{\ell=1}^k \vct{v}_\ell\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\twonorm{\vct{w}_\ell-\vct{w}_\ell^0}\le R_\ell}{\sup}\text{ }\sum_{i=1}^n\xi_i\phi(\langle\vct{w}_\ell,\vct{x}_i\rangle)\Bigg]
%\end{align*}
%Note that
%\begin{align*}
%\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right)=&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n \xi_i\Vb\phi\left(\W\vct{x}_i\right)\Bigg]
%%\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k \xi_i\vct{v}_\ell\phi(\langle\vct{w}_\ell,\vct{x}_i\rangle)\Bigg]
%\end{align*}
%We continue by using the identity
%\begin{align*}
%\phi\left(\langle \vct{w}_\ell,\vct{x}_i\rangle\right)=\phi\left(\langle \vct{w}_\ell^0, \vct{x}_i\rangle\right)+\left(\int_0^1\phi'((1-t_{i\ell})\langle\w_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\w_\ell,\vct{x}_i\rangle) dt\right)\left(\langle\vct{w}_\ell-\vct{w}_\ell^0,\vct{x}_i\rangle\right)
%\end{align*}
%Thus we can write
%\begin{align*}
%\phi\left(\W\vct{x}_i\right)=\phi\left(\W_0\vct{x}_i\right)+\text{diag}\left(\vct{u}_{i}\right)(\W-\W_0)\vct{x}_i\quad\text{where}\quad [\vct{u}_i]_\ell:=\int_0^1\phi'((1-t_{i\ell})\langle\w_\ell^0,\vct{x}_i\rangle+t_{i\ell}\langle\w_\ell,\vct{x}_i\rangle) dt
%\end{align*}
%We thus have
%\begin{align*}
%\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\mathcal{W}}\right)\le&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\sum_{i=1}^n\xi_i\Vb\phi\left(\W_0\vct{x}_i\right)+\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n \xi_i\Vb\text{diag}\left(\vct{u}_i\right)\left(\W-\W_0\right)\vct{x}_i\Bigg]\\
%=&\frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\W\in\mathcal{W}}{\sup}\text{ }\sum_{i=1}^n \xi_i\Vb\text{diag}\left(\vct{u}_i\right)\left(\W-\W_0\right)\vct{x}_i\Bigg]\\
%=& \frac{1}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\underset{\fronorm{\W-\W_0}\le M}{\sup}\text{ }\Big\langle\sum_{i=1}^n \xi_i\text{diag}\left(\vct{u}_i\right)\vct{v}\vct{x}_i^T,\W-\W_0\Big\rangle\Bigg]\\
%\le&\frac{M}{n}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\text{diag}\left(\vct{v}\right)\left(\sum_{i=1}^n \xi_i\vct{u}_i\vct{x}_i^T\right)}\Bigg]\\
%\le&\frac{M}{n}\infnorm{\vct{v}}\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\sum_{i=1}^n \xi_i\vct{u}_i\vct{x}_i^T}\Bigg]\\
%\le&\frac{M}{n}\infnorm{\vct{v}}\sqrt{\E_{\xi_{i,j}\overset{i.i.d.}{\sim}\pm 1}\Bigg[\fronorm{\sum_{i=1}^n \xi_i\vct{u}_i\vct{x}_i^T}^2\Bigg]}\\
%=&\frac{M}{n}\infnorm{\vct{v}}\sqrt{\sum_{i=1}^n\twonorm{\vct{u}_i}^2\twonorm{\vct{x}_i}^2}\\
%\le& \frac{1}{\sqrt{n}}MB\sqrt{k}\infnorm{\vct{v}}
%\end{align*}


==> generalize.tex <==
\section{Generalization bounds}

==> lin.tex <==



==> loss.tex <==

\section{Other losses}
Consider the loss function
\[
\Lc(\bteta)=\sum_{i=1}^n \ell(y_i,f(\x_i,\bteta)).
\]
Define 
\[
\rb(\bteta)=[\ell'(y_i,f(\x_1,\bteta))~\dots~\ell'(y_i,f(\x_n,\bteta))]
\]
We have that
\[
\grad{\bteta}=\sum_{i=1}^n \ell'(y_i,f(\x_i,\bteta))\frac{\pa f(\x_i,\bteta)}{\pa \bteta}=\Jc(\bteta)^T\rb(\bteta)
\]
We can write the next residual as
\[
\rb_{\tau+1}=\ell'(\x_i,\bteta_{\tau+1})=\ell'(f(\x_i,\bteta_{\tau}+\eta\grad{\bteta_\tau}))=\ell''_i\eta\Jc_i^T\grad{\bteta_\tau}
\]
\[
f(\x_i,\bteta_{\tau}+\eta\grad{\bteta_\tau})-f(\x_i,\bteta_{\tau})=\eta\Jc_i^T\grad{\bteta_{\tau}}=\eta\Jc_i^T\Jc\rb_\tau.
\]
\begin{align}
\rb_{\tau+1}&=\ell'(\bteta_{\tau+1})=\ell'(\bteta_{\tau}-\eta \grad{\bteta})=\ell'(\bteta_{\tau})-\eta \grad{\bteta} \int_{0}^1\ell''(\alpha\bteta_{\tau}+(1-\alpha)\bteta_{\tau+1})d\alpha\\
&=\rb_\tau-\eta\text{diag}(\ell''_\tau) \Jc(\bteta)\grad{\bteta} \\
&=\rb_\tau-\eta\text{diag}(\ell''_\tau) \Jc(\bteta) \Jc(\bteta)^T\rb_\tau\\
\end{align}


==> mixturecopy.tex <==
\section{The Jacobian of the Mixture Model is low-rank (Proofs for Section \ref{mix sec})}

The following theorem considers a simple noiseless mixture model and proves that its Jacobian is low-rank and the concatenated multiclass label vectors lie on a rank $K^2C$ information space associated with this Jacobian.
\begin{theorem} Consider a dataset consisting of $K$ classes each consisting of $C$ clusters. Let $(\bmu_{i,j})_{(i,j)=(1,1)}^{(\K, C)}$ be $K\times C$ cluster centers with unit Euclidian norm. Sample a dataset $(\x_i,\y_i)_{i=1}^n$ of size $n=KC\bar{n}$ as follows: i) Each cluster center is sampled exactly $\bar{n}$ times as input sample. ii) Suppose $\x_i=\cb_{j,k}$, then set $\y_i\in\R^\K$ to be one-hot encoding of $j$. Let $\bSi(\X)$ be the multiclass kernel matrix associated with input matrix $\X=[\x_1~\dots~\x_n]^T$. Let $\Rc$ be the range space of $\bSi(\X)$. Let $\M=[\bmu_{1,1}~\dots~\bmu_{\K,C}]^T$ be the cluster matrix. Define the single output cluster kernel matrix 
\[
\bSi'(\M)=(\M\M^T)\odot \E_{\g\distas \Nn(0,1)}[{\phi'(\M\g)}{\phi'(\M\g)^T}]\in\R^{\K C\times \K C}.
\] 
Assume $\bSi'(\M)$ is full rank. We have that
\begin{itemize}
\item $\Rc$ is a $K^2C$ dimensional space.
\item Concatenated label vector lies on $\Rc$.
\item  For $1\geq i\geq \K^2C$, we have that $\la_{i}(\bSi(\X))=\bar{n}\la_{i}(\Iden_{\K}\otimes \bSi'(\M))$. Hence, eigenvalues of information space grows with $n/\K C$.
\end{itemize}
\end{theorem}
\begin{proof} Via Lemma \ref{multi cov}, recall that multiclass covariance is given by %a block-diagonal matrix where $i$th diagonal block of size $n\times n$ is given by
\[
\bSi(\X)=k\sigma^2 \Iden_{\K}\otimes \bSi'(\X).
\]
where $\bSi'=(\X\X^T)\odot \E_{\g\distas \Nn(0,1)}[{\phi'(\X\g)}{\phi'(\X\g)^T}]$. Due to Kronecker product representation, range space of $\bSi(\X)$ is separable. In particular, we can set
\[
\Ic'=\text{range}(\bSi'(\X))
\]
and we will have $\Ic=\Iden_{\K}\otimes\Ic'$. This also implies $\text{rank}(\Ic)=\K\text{rank}(\Ic')$. Hence, we reduce the problem to single output networks. To proceed, following \eqref{concat}, we will show three things to conclude with the proof:
 \begin{itemize}
\item $\Ic'$ is of rank $\K C$.
\item Eigenvalues of $\X'$ is $\bar{n}$ times the eigenvalues of $ \bSi'(\M)$.
\item The label vector $\y_i\in\R^{\K C\bar{n}}$ associated with class $i$ lies on $\Ic'$. Hence, concatenated vector lies on $\Iden_{\K}\otimes \Ic'$.%Let $\M=[\bmu_{1,1}~\dots~\bmu_{\K,C}]$ be the cluster matrix. For $1\geq i\geq \K^2C$, we have that $\la_{i}(\bSi(\X))=\bar{n}\la_{i}(\bSi(\M))$. Hence, eigenvalues of information space grows with $n/\K C$.
\end{itemize}
We prove these statements as follows. Let $\W_0\distas\Nn(0,1)$, $\Vb$ have i.i.d.~zero-mean entries with $1/k$ variance. Let $\Jc_i(\W_0,\X),\Jc_i(\W_0,\M)$ be the Jacobian associated with the $i$th output of the neural net for data matrices $\X,\M$ respectively. Observe that columns of $\Jc_i(\W_0,\X)$ are chosen from $\Jc_i(\W_0,\M)$ and in particular each column of $\Jc_i(\W_0,\M)$ is repeated exactly $\bar{n}$ times. To mathematically relate this, define the $KC$ dimensional subspace $S$ of $\R^{\bar{n}\K C}$ where for any $\vb\in S$, entries $i,j$ of $\vb$ are equal iff $\x_i=\x_j$. Now, let $\Ub_S\in\R^{\bar{n}\K C\times \K C}$ be a 0-1 matrix with orthogonal rows that map $\R^{\K C}$ to $S$ as follows. Given $\x\in\R^{\K C}$ index its entries in $\K\times C$ in the same way columns of $\M$ are ordered. Then, all entries $1\leq i\leq \bar{n}\K C$ of $\Ub_S\x$ that correspond to $(j,k)$th cluster is equal to $\x_{(j,k)}$. The $(j,k)$th column of $\Ub_S$ is the indicator function of assignment to $(j,k)$th cluster. Since clusters have same size, $\Ub_S$ is orthogonal with singular values $\sqrt{\bar{n}}$. Then, we have that%This implies that
\[
\Ub_S\Jc_i(\W_0,\M)=\Jc_i(\W_0,\X).
\]
Let $\bar{\Ub}_S=\Ub_S/\sqrt{\bar{n}}$ which is an orthonormal matrix. This implies that
\[
\bar{n}\bar{\Ub}_S\bSi(\M)'\bar{\Ub}_S^T=\bSi(\X)'.
\]
Since $\bar{\Ub}_S$ is tall and orthonormal, range of $\bSi(\X)'$ is exactly range of $\Ub_S$ hence $\Ic'=S$ which is $\K C$ dimensional. Furthermore, $\bar{\Ub}_S$ can be subsumed into the eigenvalue decomposition of $\bSi(\M)'$ which yields that nonzero eigenvalues of $\bSi(\X)'$ are $\bar{n}$ times that of $\bSi(\M)'$ with eigenvectors lying on $S$. Finally, we will argue that label vector $\y_\ell$ lies on $S$. Observe that entries $i$ of $\y_\ell$ whose input samples $\x_i$ correspond to the same cluster $(j,k)$ is exactly same as same inputs are assigned to same labels. Specifically, if cluster is inside class $\ell$ (i.e.~$\ell=j$) then $y_{\ell,i}=1$ otherwise $y_{\ell,i}=0$.
\end{proof}
%Then $\E[\Cb(\W)]$ is a block diagonal matrix given by the Kronecker product

==> multi.tex <==
\section{Multi-class?}

==> neural_append.tex <==
\section{Proofs of Neural Network Results}

\subsection{Preliminaries}
Denote the rows of input and output weight matrices $\W,\Vb$ by $\w_\ell$ and $\vb_\ell$ respectively. Given a matrix $\M$ with $k$ rows $(\m_i)_{i=1}^k$, denote the largest Euclidian norm over rows by $\trow{\M}$. We begin by noting that for a one-hidden layer neural network of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$, the Jacobian matrix with respect to vect$(\mtx{W})\in\R^{kd}$ takes the form
\begin{align}
\mathcal{J}(\mtx{W})=
\begin{bmatrix}
\mathcal{J}_1(\W) \\ \vdots \\ \mathcal{J}_\K(\W)
\end{bmatrix}\in\R^{\K n\times kd}\label{jacob multi}
\end{align}
where $\Jc_i(\W)=\Jc(\vb_i,\W)$ is the Jacobian matrix associated with the $i$th class. $\Jc_i(\W)$ is given by
\begin{align*}
\mathcal{J}_i(\mtx{W})=
\begin{bmatrix}
\mathcal{J}_i(\vct{w}_1) & \ldots & \mathcal{J}_i(\vct{w}_k)
\end{bmatrix}\in\R^{n\times kd}\quad\text{with}\quad\mathcal{J}_i(\vct{w}_\ell):={v}_{i,\ell}\text{diag}(\phi'(\mtx{X}\vct{w}_\ell))\mtx{X}.
\end{align*}
Alternatively this can be rewritten in the form
\begin{align}
\label{KR}
\mathcal{J}_i(\mtx{W})^T=\left(\text{diag}(\vct{v}_i)\phi'\left(\mtx{W}\mtx{X}^T\right)\right)*\mtx{X}^T
\end{align}
An alternative characterization of the Jacobian is its matrix representation. Given vector $\ub\in\R^{\K n}$ partition into $\K$ size $n$ subvectors $\ub=[\ub_1~\dots~\ub_\K]$. We have
\begin{align}
\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)= \sum_{i=1}^\K\text{diag}(\vct{v}_i)\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u}_i)\mtx{X}\label{mat form}
\end{align}

\subsection{Properties}
% as depicted in Figure \ref{neuralnet}

%\subsection{Properties of Neural Net Jacobian}
%\begin{lemma}[Spectral norm of the Jacobian]\label{spectJ} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \vct{v}^T\phi\left(\W\x\right)$ where the activation $\phi$ has bounded derivatives obeying $\abs{\phi'(z)}\le B$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Then the Jacobian matrix with respect to the input-to-hidden weights obeys 
%\begin{align*}
%\opnorm{\mathcal{J}(\mtx{W})}\le \sqrt{k}B\infnorm{\vct{v}}\opnorm{\X}.
%\end{align*}
%\end{lemma}
%\begin{lemma}[Jacobian Lipschitzness]\label{JLlem} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \vct{v}^T\phi\left(\W\x\right)$ where the activation $\phi$ has bounded second order derivatives obeying $\abs{\phi''(z)}\le M$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Then the Jacobian mapping with respect to the input-to-hidden weights obeys
%\begin{align*}
%\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le M\infnorm{\vct{v}}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}\quad\text{for all}\quad \widetilde{\W},\W\in\R^{k\times d}.
%\end{align*}
%\end{lemma}
\begin{lemma}[Properties of Single Output Neural Net Jacobian]\label{props thm} Let $\K=1$ so that $\Vb^T=\vb\in\R^n$. Suppose $\phi$ is an activation satisfying $|\phi'|\leq B$. At any matrix $\W\in\R^{k\times d}$ and any unit length vector $\ub$, we have
\[
\|\Jc(\W)\|\leq B\sqrt{k}\infnorm{\vct{v}}\opnorm{\X}\quad,\quad\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}\leq B\tin{\vb}\|\X\|.
\]
Suppose $\phi$ is second order differentiable and $|\phi''|\leq M$. Furthermore, assume the rows of $\X$ have unit Euclidean norm ($\twonorm{\vct{x}_i}=1$). Then Jacobian is Lipschitz with respect to spectral norm i.e.~{for all} $\widetilde{\W},\W\in\R^{k\times d}$
\begin{align*}
\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le M\infnorm{\vct{v}}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}.
\end{align*}
\end{lemma}
\begin{proof} The result on spectral norm and Lipschitzness of $\Jc(\W)$ follows from \cite{onehidden}. To show row-wise bound, using \eqref{mat form}, given unit vector $\ub\in\R^n$, we have that
\begin{align}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}&= \trow{\text{diag}(\vct{v})\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u})\mtx{X}}\\
&= \tin{\vb}\max_{1\leq i\leq k}\tn{\phi'\left(\w_i^T\mtx{X}^T\right)\text{diag}(\vct{u})\mtx{X}}\\
&\leq \tin{\vb}\|\X\|\max_{1\leq i\leq k}\tn{\phi'\left(\w_i^T\mtx{X}^T\right)\text{diag}(\vct{u})}\\
&\leq B\tin{\vb}\|\X\|\tn{\ub}=B\tin{\vb}\|\X\|.
\end{align}
\end{proof}

\begin{theorem}[Properties of Multiclass Neural Net Jacobian]\label{props lem} Suppose $\phi$ is an activation satisfying $|\phi'|\leq B$. At any matrix $\W\in\R^{k\times d}$ and any unit length vector $\ub$, we have
\[
\|\Jc(\W)\|\leq B\sqrt{\K k}\infnorm{\Vb}\opnorm{\X}\quad,\quad\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}\leq B\sqrt{\K}\tin{\Vb}\|\X\|.
\]
Suppose $\phi$ is second order differentiable and $|\phi''|\leq M$. Furthermore, assume the rows of $\X$ have unit euclidean norm ($\twonorm{\vct{x}_i}=1$). Then Jacobian is Lipschitz with respect to spectral norm i.e.~{for all} $\widetilde{\W},\W\in\R^{k\times d}$
\begin{align*}
\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le M\sqrt{\K}\infnorm{\Vb}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}.
\end{align*}
\end{theorem}
\begin{proof} The proof will follow from Lemma \ref{props thm}. First, given $\A=[\A_1^T~\dots~\A_\K^T]^T$ and $\B=[\B_1^T~\dots~\B_\K^T]^T$, observe that
\[
\|\A\|\leq \sqrt{\K} \sup_{1\leq i\leq \K}\|\A_i\|\quad,\quad\|\A-\B\|\leq \sqrt{\K} \sup_{1\leq i\leq \K}\|\A_i-\B_i\|.
\]
These two establishes the advertised bounds on $\|\Jc(\W)\|$ and $\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}$ by writing them in terms of $\Jc_i(\W),\Jc_i(\tilde{\W})$. Similarly, to find the row bound, given unit length $\ub\in\R^{\K n}$ we split it into $\K$ vectors $\ub=[\ub_1~\dots~\ub_\K]$ and write
\begin{align}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}&=\sum_{i=1}^\K \trow{\text{mat}\left(\mathcal{J}_i^T(\mtx{W})\vct{u}_i\right)}\\
&=\sum_{i=1}^\K B\tin{\Vb}\|\X\|\tn{\ub_i}\leq B\tin{\Vb}\|\X\|\sqrt{\K},
\end{align}
concluding the proof.
\end{proof}



\begin{lemma}[Multiclass covariance] \label{multi cov}Given input and output layer weights $\Vb,\W$, consider the Jacobian described in \eqref{jacob multi}. Given an $\K n\times \K n$ matrix $\M$, let $\M[i,j]$ denote the $(i,j)$th submatrix for $1\leq i,j\leq \K$. Set $\Cb(\W)=\Jc(\W)\Jc(\W)^T$. We have that
\[
\Cb(\W)[i,j]=\sum_{\ell=1}^k(\X\X^T)\odot (v_{i,\ell}v_{j,\ell}{\phi'(\X\w_{\ell})}{\phi'(\X\w_{\ell})^T}).
\]
Suppose $\W\distas\Nn(0,1)$ and $\Vb$ has i.i.d.~zero-mean entries with $\sigma^2$ variance. Then $\E[\Cb(\W)]$ is a block diagonal matrix given by the Kronecker product%a block-diagonal matrix where $i$th diagonal block of size $n\times n$ is given by
\[
\E[\Cb(\W)]=k\sigma^2 \Iden_{\K}\otimes \bSi(\X).
\]
\end{lemma}
\begin{proof} The $(i,j)$th submatrix of $\Cb(\W)$ is given by
\begin{align}
\Cb(\W)[i,j]&=((\text{diag}(\vb_i)\phi'(\W\X^T))*\X^T)((\text{diag}(\vb_j)\phi'(\W\X^T))*\X^T)^T\\
&=\sum_{\ell=1}^k \Jc_i(\w_{\ell})\Jc_j(\w_{\ell})^T\\
&=\sum_{\ell=1}^kv_{i,\ell}v_{j,\ell}(\diag{\phi'(\X\w_{\ell})}\X)(\diag{\phi'(\X\w_{\ell})}\X)^T\\
&=\sum_{\ell=1}^kv_{i,\ell}v_{j,\ell}(\X\X^T)\odot ({\phi'(\X\w_{\ell})}{\phi'(\X\w_{\ell})^T})\\
&=\sum_{\ell=1}^k(\X\X^T)\odot (v_{i,\ell}v_{j,\ell}{\phi'(\X\w_{\ell})}{\phi'(\X\w_{\ell})^T}).
\end{align}
Setting $\W\distas\Nn(0,1)$ and $\vb$ with i.i.d. zero-mean and $\sigma^2$-variance entries, we find
\begin{align}
\E[\Cb(\W)[i,j]]&=\sum_{\ell=1}^k(\X\X^T)\odot (\E[v_{i,\ell}v_{j,\ell}]\E[{\phi'(\X\w_{\ell})}{\phi'(\X\w_{\ell})^T}])\\
&=\sum_{\ell=1}^k\sigma^2(\X\X^T)\odot (\delta(i-j)\bSi(\X))\\
&=k\delta(i-j)\sigma^2(\X\X^T)\odot (\bSi(\X)).
\end{align}
where $\delta(x)$ is the discrete $\delta$ function which is 0 for $x\neq 0$ and $1$ for $x=0$.
\end{proof}
\begin{lemma}[\cite{Schur1911}]\label{minHad} Let $\mtx{A},\mtx{B}\in\R^{n\times n}$ be two Positive Semi-Definite (PSD) matrices. Then,
\begin{align*}
\lambda_{\min}\left(\mtx{A}\odot\mtx{B}\right)\ge& \left(\min_{i} \mtx{B}_{ii}\right)\lambda_{\min}\left(\mtx{A}\right),\\
\lambda_{\max}\left(\mtx{A}\odot\mtx{B}\right)\le& \left(\max_{i} \mtx{B}_{ii}\right)\lambda_{\max}\left(\mtx{A}\right).
\end{align*}
\end{lemma}
\begin{lemma}[Minimum eigenvalue of the Jacobian at initialization]\label{minspectJ} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$ where the activation $\phi$ has bounded derivatives obeying $|\phi(0)|,\abs{\phi'(z)}\le B$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Suppose $\Vb$ has i.i.d.~$\sigma$-scaled Rademacher entries (i.e.~$\pm \sigma$ equally-likely). Then, 
%as long as
%\begin{align*}
%\frac{\twonorm{\vct{v}}}{\infnorm{\vct{v}}}\ge \sqrt{20\log n}\frac{\opnorm{\X}}{\sqrt{\lambda(\X)}}B,
%\end{align*}
the Jacobian matrix at a random point $\mtx{W}_0\in\R^{k\times d}$ with i.i.d.~$\mathcal{N}(0,1)$ entries obeys 
\begin{align*}
%&\sigma_{\min}\left(\mathcal{J}(\W_0)\right)\ge \frac{1}{\sqrt{2}}\twonorm{\vct{v}}\sqrt{\lambda(\X)},\\
&\| \Jc(\W_0)\Jc(\W_0)^T-\E[\Jc(\W_0)\Jc(\W_0)^T]\|\leq 30\K\sqrt{k}\sigma^2B^2\|\X\|^2\log(2n).
\end{align*}
with probability at least $1-1/n^{100}$. In particular, given approximation level $\delta>0$ and picking entries of $\vb$ with equal magnitude, if 
\[
k\geq \frac{1000\K^2B^4\|\X\|^4\log^2(2n)}{\delta^2},
\]
with same probability, we have that
\[
\|\frac{1}{k\sigma^2}\Jc(\W_0)\Jc(\W_0)^T- \Iden_{\K}\otimes \bSi(\X)\|\leq \delta.
\]
\end{lemma}
\begin{proof} Define the random matrix 
\[
\A_\ell=\left(\phi'\left(\X\w_\ell\right)\phi'\left(\X\w_\ell\right)^T\right)\odot\left(\X\X^T\right)
\]
Let $\Cb=\Jc(\W_0)\Jc(\W_0)^T$. Considering $n\times n$ diagonal blocks of $\Cb$ for $1\leq i\leq \K$, we have that
\[
\E[\A_\ell]=\mtx{\Sigma}(\X)\quad,\quad \Cb[i,i]=\sum_{\ell=1}^k \vb_{i,\ell}^2\A_\ell=\Cb[i,i]=\sigma^2\sum_{\ell=1}^k \A_\ell.
\]
Additionally, spectral norm of $\A_\ell$ is deterministically upper bounded by $B^2\|\X\|^2$ via Lemma \ref{minHad}. This implies
\[
\|(\A_\ell-\E[\A_\ell])^2\|= \|\A_\ell-\E[\A_\ell]\|^2\leq (2B^2\|\X\|^2)^2.
\]
To proceed, we will bound the weighted sum
\[
\Sb=\sum_{\ell=1}^k\sigma^2(\A_\ell-\E[\A_\ell])
\]
in spectral norm. The Matrix Hoeffding inequality yields
\[
\Pro(\|\Sb\|\geq t)\leq 2n\exp(-t^2/2\bar{\sigma}^2)
\]
where $\bar{\sigma}^2=\sum_{i=1}^k (2\sigma^2B^2\|\X\|^2)^2=4k\sigma^4B^4\|\X\|^4$. Setting $t=30\sqrt{k}\sigma^2B^2\|\X\|^2\log(2n)$, we find that
\[
\Pro(\| \Cb[i,i]-\E[\Cb[i,i]]\|\geq t)=\Pro(\|\Sb\|\geq t)\leq n^{-102}%\tn{\vb}^2\mtx{\Sigma}(\X)
\]
concluding the proof for diagonal blocks. For off-diagonal blocks $\Cb[i,j]$ following Lemma \ref{multi cov} we have that
\[
\Cb[i,j]=\sum_{\ell=1}^k v_{i,\ell}v_{j,\ell}\A_{\ell}.
\]
Note that by construction $(v_{i,\ell}v_{j,\ell})_{\ell=1}^k$ are i.i.d.~$\pm \sigma^2$ Rademacher variables. Hence, $\Cb[i,j]$ is sum of zero-mean i.i.d.~matrices. Consequently, using $\|\A_{\ell}^2\|\leq 4B^4\|\X\|^4$ and applying Hoeffding inequality again with same choice of $t$, we find that
\[
\Pro(\| \Cb[i,j]\|\geq t)\leq n^{-102}
\]
Union bounding over all submatrices $1\leq i,j\leq K$ and using $K\leq n$ we obtain that
\[
\Pro(\|\Cb[i,j]-\E[\Cb[i,j]]\|\geq t)\leq K^2n^{-102}\leq n^{-100}.
\]
What remains is bounding ${\bf{D}}:=\|\Cb-\E[\Cb]\|$. Let $\Db[i,:]$ denote the $i$th block row of $\Db$. Standard bounds on spectral norm in terms of submatrices yields, 
\begin{align}
&\|\Db[i,:]\|\leq \sqrt{\K}\sup_{1\leq j\leq \K} \|\Db[i,j]\|\leq \sqrt{\K}t\\
&\|\Db\|\leq \sqrt{\K}\sup_{1\leq j\leq \K} \|\Db[i,:]\|\leq \sqrt{\K}\sqrt{\K}t=\K t=30\K\sqrt{k}\sigma^2B^2\|\X\|^2\log(2n),
\end{align}
which is the advertised result. The result in terms of $\delta$ is obtained by using the population covariance Lemma \ref{multi cov}.% plugging $\tn{\vb}^2=k\sigma^2$ and 
\end{proof}
The following lemma directly follows from the proof argument of Lemma 6.12 of \cite{onehidden}.
\begin{lemma}[Upper bound on initial misfit]\label{upresz} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$ where the activation $\phi$ has bounded derivatives obeying $|\phi(0)|,\abs{\phi'(z)}\le B$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as rows of a matrix $\X\in\R^{n\times d}$ and the corresponding labels given by $\vct{y}\in\R^{\K n}$. Furthermore, assume entries of $\Vb$ are i.i.d.~Rademacher variables scaled by $\frac{\vrn\twonorm{\y}}{50B\sqrt{\K \log(2\K)kn}}$ and entries of $\mtx{W}\in\R^{k\times d}$ are i.i.d.~$\mathcal{N}(0,1)$. Then
\begin{align*}
\twonorm{\Vb\phi\left(\W\X^T\right)}\le\vrn\twonorm{\y},
\end{align*}
holds with probability at least $1-(2\K)^{-100}$.
\end{lemma}
\begin{proof}
\label{upreszpf}
The objective term can be written as
\[
\twonorm{\Vb\phi\left(\W\X^T\right)}^2=\sum_{i=1}^\K \twonorm{\vb_i^T\phi\left(\W\X^T\right)}^2.
\]
We will show that for any row $\vb$ of $\Vb$, with probability $1-(2\K)^{-101}$,
\[
 \twonorm{\vb_i^T\phi\left(\W\X^T\right)}\leq \frac{\vrn}{\sqrt{\K}}\twonorm{\y}.
\]
Union bounding will yield the desired result. To proceed, note that for any two matrices $\widetilde{\W}, \W\in\R^{k\times d}$ we have
\begin{align*}
\abs{\twonorm{\phi\left(\X\widetilde{\W}^T\right)\vct{v}}-\twonorm{\phi\left(\X\W^T\right)\vct{v}}}\le& \twonorm{\phi\left(\X\widetilde{\W}^T\right)\vct{v}-\phi\left(\X\W^T\right)\vct{v}}\\
\le&\opnorm{\phi\left(\X\widetilde{\W}^T\right)-\phi\left(\X\W^T\right)}\twonorm{\vct{v}}\\
\le& \fronorm{\phi\left(\X\widetilde{\W}^T\right)-\phi\left(\X\W^T\right)}\twonorm{\vct{v}}\\
& \hspace{-100pt}\overset{(a)}{=}\fronorm{\left(\phi'\left(\Sb\odot\X\widetilde{\W}^T+(1_{k\times n}-\Sb)\odot\X\W^T\right)\right)\odot \left(\X(\widetilde{\W}-\W)^T\right)}\twonorm{\vct{v}}\\
\le&B\fronorm{\X(\widetilde{\W}-\W)^T}\twonorm{\vct{v}}\\
\le&B\opnorm{\X}\twonorm{\vct{v}}\fronorm{\widetilde{\W}-\W},
\end{align*}
where in (a) we used the mean value theorem with $\Sb$ a matrix with entries obeying $0\le \Sb_{i,j}\le 1$ and $1_{k\times n}$ the matrix of all ones. Thus, $\twonorm{\phi\left(\X\W^T\right)\vct{v}}$ is a $B\opnorm{\X}\twonorm{\vct{v}}$-Lipschitz function of $\mtx{W}$. Thus, fixing $\vb$, for a matrix $\W$ with i.i.d.~Gaussian entries 
\begin{align}
\label{tempmyflip}
\twonorm{\phi\left(\X\W^T\right)\vct{v}}\le \E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}\big]+t,
\end{align}
holds with probability at least $1-e^{-\frac{t^2}{2B^2\twonorm{\vct{v}}^2\opnorm{\X}^2}}$. Next given $g\sim\Nn(0,1)$, we have
\begin{align}
|\E[\phi(g)]|\leq |\E[\phi(0)]|+|\E[\phi(g)-\phi(0)]|\leq B+B\E[|g|]\leq 2B\quad\text{and}\quad \text{Var}(\phi(g))\le B^2.\label{poinc stuff}
\end{align}
where the latter follows from Poincare inequality (e.g.~see \cite[p. 49]{ledoux}).
Furthermore, since $\vb$ has i.i.d.~Rademacher entries, applying Bernstein bound, event 
\begin{align}
E_{\vb}:=\{|\onebb^T\vb|^2\leq 250\log \K \tn{\vb}^2\} \label{berns v}
\end{align}
holds with probability $1-(2\K)^{-102}$. Conditioned on $E_{\vb}$, we now upper bound the expectation via
\begin{align*}
\E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}\big]\overset{(a)}{\le}& \sqrt{\E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}^2\big]}\\
=&\sqrt{\sum_{i=1}^n \E\big[\left(\vct{v}^T\phi(\W\vct{x}_i)\right)^2\big]}\\
\overset{(b)}{=}&\sqrt{n}\sqrt{\E_{\vct{g}\sim\mathcal{N}(\vct{0},\mtx{I}_k)}\big[\left(\vct{v}^T\phi(\vct{g})\right)^2\big]}\\
\overset{(c)}{=}&\sqrt{n}\sqrt{\twonorm{\vct{v}}^2\E_{g\sim\mathcal{N}(0,1)}\big[\left(\phi(g)-\E[\phi(g)]\right)^2\big]+(\vct{1}^T\vct{v})^2(\E_{g\sim\mathcal{N}(0,1)}[\phi(g)])^2}\\
\overset{(d)}{=}&\sqrt{n}\twonorm{\vct{v}}\sqrt{250\times 4B^2\log (2\K) +B^2}\\
{\le}&32\sqrt{n\log (2\K) }B\twonorm{\vct{v}}.
\end{align*}
Here, (a) follows from Jensen's inequality, (b) from linearity of expectation and the fact that for $\vct{x}_i$ with unit Euclidean norm $\mtx{W}\vct{x}_i\sim\mathcal{N}(\vct{0},\mtx{I}_k)$, (c) from simple algebraic manipulations, (d) from the inequalities \eqref{berns v} and \eqref{poinc stuff}. Thus using $t=18\sqrt{n\log (2\K) }B\twonorm{\vct{v}}$ in \eqref{tempmyflip}, conditioned on $E_{\vb}$ we conclude that
\begin{align}
\twonorm{\phi\left(\X\W^T\right)\vct{v}}\le&50\sqrt{n\log (2\K) }B\twonorm{\vct{v}},\label{fin fin eq}
\end{align}
holds with probability at least $1-\exp(-102\log (2\K)\frac{n}{\opnorm{\X}^2})\geq 1-(2\K)^{-102}$ where we used $n\geq \|\X\|^2$. Union bounding $E_{\vb}$ and conditional concentration over $\W$, the overall probability of success in \eqref{fin fin eq} is at least $1-(2\K)^{-101}$ concluding the proof after substituting the definition of $\vb$ to the right hand side
\[
50\sqrt{n\log (2\K) }B\tn{\vb}=50\sqrt{n\log (2\K) }B\sqrt{k}\frac{\vrn\twonorm{\y}}{50B\sqrt{\K\log (2\K) kn}}=\frac{\sigma \tn{\y}}{\sqrt{\K}}.
\] %Setting $\delta=9$ and $t=9\twonorm{\vct{v}}\sqrt{n} B$, our choice of $\vb$ guarantees the right hand side is at most $\vrn\tn{\y}$.
\end{proof}
%\subsection{Proofs for minimum eigenvalue of the Jacobian at initialization (Proof of Lemma \ref{minspectJ})}



==> neural_append_main_bc.tex <==
% !TEX root = JacobianGen.tex
\section{Neural Network Optimization and Generalization for Arbitrary Initialization}
%%\[
%%\bar{\alpha}=\frac{\alpha}{\vrn B\opnorm{\X}}.
%%\]
\subsection{General Optimization Result}
\begin{lemma} [Deterministic convergence guarantee] \label{nn deter}Consider a one-hidden layer neural net of the form $\vct{x}\mapsto f(\vct{x};\mtx{W}):=\Vb\phi(\mtx{W}\vct{x})$ with input weights $\W\in\R^{k\times d}$ and output weights $\Vb\in\R^{K\times k}$ and an activation $\phi$ obeying $\abs{\phi(0)}\le B$, $\abs{\phi'(z)}\le B$, and $\abs{\phi''(z)}\le B$ for all $z$. Also assume $\Vb$ is fixed with all entries bounded by $\infnorm{\Vb}\le\frac{\sigma}{\sqrt{kK}}$ and we train over $\W$ based on the loss 
\begin{align*}
\mathcal{L}(\W)=\frac{1}{2}\sum_{i=1}^n\twonorm{f(\vct{x}_i;\W)-\y_i}^2.
\end{align*}
Also, consider a point $\W_0\in\R^{k\times d}$ with $\mtx{J}$ an $(\epsilon_0,\vrn B\|\X\|)$ reference Jacobian associated with $\mathcal{J}(\W_0)$ per Definition \ref{tjac}. Furthermore, define the information $\calF$ and nuisance $\calS$ subspaces and the truncated Jacobian $\mtx{J}_{\calF}$ associated with the reference Jacobian $\mtx{J}$ based on a cut-off spectrum value of $\alpha$ per Definition \ref{tjac2}. Let the initial residual vector be $\rb_0=\y-f(\W_0)\in\R^{n\K}$. Furthermore, assume
\begin{align}
\label{epsass}
 \eps_0\leq \frac{\alpha}{5}\min\left(\delta,\sqrt{\frac{\delta\alpha}{\Gamma\beta}}\right)
 \end{align}
and
\begin{align}
k\geq 400\frac{\vrn^6B^6\opnorm{\X}^6\Gamma^2}{\delta^2\alpha^8}\left(\upp+\delta\Gamma\tn{\rb_0}\right)^2,\label{fund k bound}
%k\geq \frac{64\Gamma^2B^2\|\X\|^2R^2}{B^2\delta^2\bar{\alpha}^6}.
\end{align}
with $0\le \delta\le1$ and $\Gamma\ge 1$. We run gradient descent iterations of the form $\W_{\tau+1}=\W_{\tau}-\eta\nabla \mathcal{L}(\W_\tau)$ starting from $\W_0$ with step size $\eta$ obeying $\eta\le \frac{1}{\sigma^2B^2\opnorm{\X}^2}$. Then for all iterates $\tau$ obeying $0\le \tau\le T:=\frac{\Gamma}{\eta\alpha^2}$
\begin{align}
\tf{\W_\tau-\W_0}\le& \frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}
.\label{main res eq22}\\
\trow{\W_{\tau}-\W_0}\le& \frac{ 2\sigma B\Gamma\opnorm{\X}}{\sqrt{k}\alpha^2}\tn{\rb_0}.\label{row boundsss}
\end{align}
Furthermore, after $\tau=T$ iteration we have
\begin{align}
\tn{\rb_{T}}\le  e^{-\Gamma}\tn{\Pi_{{\Rc}}(\rb_0)}+\tn{ \Pi_{\mathcal{N}}(\rb_0)}+ \frac{\delta\alpha}{\vrn B\opnorm{\X}}\tn{\rb_0}.\label{eqqq22}
\end{align}
\end{lemma}
\begin{proof} To prove this lemma we wish to apply Theorem \ref{many step thm}. We thus need to ensure that the assumptions of this theorem are satisfied. To do this note that by Lemma \ref{props lem} Assumption \ref{ass2} holds with $\beta=\vrn B\opnorm{\X}$. Furthermore, we pick $\eps=\frac{\delta\alpha^3}{5\Gamma \vrn^2 B^2\opnorm{\X}^2}=\frac{\delta\alpha^3}{5\Gamma \beta^2}$ which together with \eqref{epsass} guarantees \eqref{cndd} holds.   We now turn our attention to verifying Assumption \ref{ass3}. To this aim note that for all $\W\in\R^{k\times d}$ obeying
\begin{align*}
\fronorm{\W-\W_0}\le R:=2\left(\frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}\right)
\end{align*}
as long as \eqref{fund k bound} holds  by Lemma \ref{props lem} we have
\begin{align*}
\|\Jc(\W)-\Jc(\W_0)\|\le&B\sqrt{\K}\infnorm{\Vb}\opnorm{\mtx{X}}R\\
\le&\frac{\vrn}{\sqrt{k}} B\opnorm{\mtx{X}}R\\
=&\frac{\delta\alpha^3}{10\Gamma\vrn^2 B^2\opnorm{\X}^2}\frac{\frac{20\Gamma\vrn^3 B^3\opnorm{\X}^3}{\delta\alpha^4}\left(\upp+\delta\Gamma\tn{\rb_0}\right)}{\sqrt{k}}\\
\le&\frac{\delta\alpha^3}{10\Gamma\vrn^2 B^2\opnorm{\X}^2}\\
=&\frac{\eps}{2}.
\end{align*}
Thus, Assumption \ref{ass3} holds with $\fronorm{\W-\W_0}\le R:=2\left(\frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}\right)$. Now that we have verified that the assumptions of Theorem \ref{many step thm} hold so do its conclusions and thus \eqref{main res eq22} and \eqref{eqqq22} hold.

We now turn our attention to proving the row-wise bound \eqref{row boundsss}. To this aim let $\w_{\ell}^{(\tau)}$ denote the $\ell$th row of $\W_\tau$. Also note that 
\[
\grad{\w_\ell}=\text{$\ell$th row of }\text{mat}(\mathcal{J}(\mtx{W})^T\rb_\tau).
\]
Hence, using Lemma \ref{props lem} equation \eqref{rowbndm} we conclude that
\[
\tn{\grad{\w_{\ell}^{(\tau)}}}\le B\sqrt{K}\infnorm{\Vb}\opnorm{\X} \le \frac{\vrn B\opnorm{\X}}{\sqrt{k}}\tn{\rb_\tau}.
\]
Consequently, for any row $1\leq \ell\leq k$, we have
\begin{align}
\twonorm{\w_{\ell}^{(\tau)}-\w_{\ell}^{(0)}}\leq \eta \frac{\vrn B\opnorm{\X}}{\sqrt{k}}\sum_{t=0}^{\tau-1}\tn{\rb_t}.\label{roww bound}
\end{align}
To bound the right-hand side we use the triangular inequality combined with \eqref{rrr bound} and \eqref{eee bound} to conclude that
\begin{align}
\label{A7}
\eta \sum_{t=0}^{\tau-1}\tn{\rb_\tau}\le&\eta\sum_{t=0}^{\tau-1}\tn{\rbb_\tau}+\eta\sum_{t=0}^{\tau-1}\tn{\rb_\tau-\rbb_\tau}\nn\\
 \le&\frac{\Gamma}{\alpha^2}\tn{\rb_0}+\frac{2\Gamma^2(\eps\beta+\eps_0^2)}{\alpha^4} \tn{\rb_0}\nn\\
 =&\frac{2\Gamma (\eps_0^2+\eps\beta)+\alpha^2}{\alpha^4}\Gamma\tn{\rb_0}\nn\\
 \le& 2\frac{\Gamma}{\alpha^2}\tn{\rb_0},
\end{align}
where in the last inequality we used the fact that $\eps_0^2\le \frac{\alpha^2}{25\Gamma}$ per \eqref{epsass} and $\epsilon\beta=\frac{\delta\alpha^3}{5\Gamma \beta}\le \frac{\alpha^2}{5\Gamma}$ per our choice of $\epsilon$. Combining \eqref{roww bound} and \eqref{A7}, we obtain
\[
\twonorm{\w_{\ell}^{(\tau)}-\w_{\ell}^{(0)}}\leq \frac{ 2\vrn B\|\X\|\Gamma}{\sqrt{k}\alpha^2}\tn{\rb_0},
\]
completing the proof of \eqref{row boundsss} and the theorem.
\end{proof}
\subsection{Main Optimization Result}
\begin{lemma} [Deterministic optimization guarantee] \label{nn deter2} Consider the setting and assumptions of Lemma \ref{nn deter}. Also assume $\tn{\Pi_{\Rc}(\rb_0)}\geq c\tn{\rb_0}$ for a constant $c>0$. Furthermore, assume
\begin{align}
\eps_0^2\le \frac{\alpha^2}{25}\min\left(c\frac{\upp\alpha}{\sigma B\Gamma^2\tn{\rb_0}\opnorm{\X}},\frac{\zeta^2\sigma^2 B^2\opnorm{\X}^2}{\alpha^2},\frac{\zeta}{\Gamma}\right),\label{ref bound eps}
\end{align}
%{{\frac{\bar{\alpha}\upp}{ \tn{\rb_0}}}\frac{\alpha^2}{25\Gamma^2}}={\frac{\alpha_0^3\upp\sigma^2}{25\Gamma^2B\K^{3/2} \|\X\|\tn{\rb_0}}}.
and
\begin{align}
k\geq 1600\left(\frac{\alpha}{\zeta\sigma B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{\sigma^6B^6\opnorm{\X}^6\Gamma^2\upp^2}{\alpha^8},\label{k bound det}
\end{align}
%with $0\le \zeta\le\frac{\alpha}{\sigma B\opnorm{\X}}$
and $\Gamma\ge 1$. We run gradient descent iterations of the form $\W_{\tau+1}=\W_{\tau}-\eta\nabla \mathcal{L}(\W_\tau)$ starting from $\W_0$ with step size $\eta$ obeying $\eta\le \frac{1}{\sigma^2B^2\opnorm{\X}^2}$. Then for all iterates $\tau$ obeying $0\le \tau\le T:=\frac{\Gamma}{\eta\alpha^2}$
\begin{align}
%\frac{\alpha_0\tn{\rb_0}}{B\sqrt{K}\|\X\|},
&\tf{\W_\tau-\W_0}\leq \frac{2\upp}{\sigma B\opnorm{\X}}.\label{main res eq23}\\
&\trow{\W_{\tau}-\W_0}\leq \frac{ 2\sigma B\Gamma\opnorm{\X}}{\sqrt{k} \alpha^2} \tn{\rb_0}.\label{row boundsss2}
\end{align}
Furthermore, after $\tau=T$ iteration we have
\begin{align}
&\twonorm{f(\W_T)-\y}\leq  e^{-\Gamma}\tn{\Pi_{{\Rc}}(\rb_0)}+\tn{ \Pi_{\mathcal{N}}(\rb_0)}+\zeta\tn{\rb_0}.\label{eqqq23}
\end{align}
\end{lemma}
\begin{proof} To prove this lemma we aim to substitute
\begin{align}
\label{delchoice}
\delta=\min\left(\frac{\zeta\sigma B\opnorm{\X}}{\alpha},\frac{\upp}{\Gamma \tn{\rb_0}}\right)\leq 1,
\end{align}
in Theorem \ref{nn deter}. To do this we need to verify the assumptions of Theorem \ref{nn deter}. To this aim note that the choice of $\delta$ from {delchoice} combined with \eqref{k bound det} ensures that
\begin{align*}
k\ge&1600\left(\frac{\alpha}{\zeta\sigma B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{\sigma^6B^6\opnorm{\X}^6\Gamma^2\upp^2}{\alpha^8}\\
\ge&\max\left(\frac{\alpha}{\zeta\sigma B\opnorm{\X}},\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{1600\sigma^6B^6\opnorm{\X}^6\Gamma^2\upp^2}{\alpha^8}\\
\ge&\frac{1}{\min\left(\frac{\zeta\sigma B\opnorm{\X}}{\alpha},\frac{\upp}{\Gamma \tn{\rb_0}}\right)^2}\frac{1600\sigma^6B^6\opnorm{\X}^6\Gamma^2\upp^2}{\alpha^8}\\
=&  \frac{1600\Gamma^2\sigma^6B^6\opnorm{\X}^6\upp^2}{\delta^2\alpha^8}\\
=&  400\frac{\Gamma^2\sigma^6B^6\opnorm{\X}^6(\upp+\upp)^2}{\delta^2\alpha^8}\\
\ge&400\frac{\Gamma^2\sigma^6B^6\opnorm{\X}^6(\upp+\delta \Gamma \tn{\rb_0})^2}{\delta^2\alpha^8},
\end{align*}
so that \eqref{fund k bound} holds. We thus turn our attention to proving \eqref{epsass}. To this aim note that based on Lemma \ref{bndearlystopval} equation \eqref{low bound} we have
\begin{align}
\upp\geq \frac{\alpha\tn{\Pi_{\Rc}(\rb_0)}}{\lambda_1}\ge \frac{\alpha\tn{\Pi_{\Rc}(\rb_0)}}{\sigma B \|\X\|}\geq \frac{c\alpha\tn{\rb_0}}{\sigma B \|\X\|}\quad\Rightarrow\quad \frac{\upp}{c \tn{\rb_0}}\geq \frac{\alpha}{\sigma B\opnorm{\X}}.\label{rhs bound}
\end{align}


Recall $\bar{\alpha}=\frac{\alpha}{\sigma B\|\X\|}=\frac{\alpha_0}{B\sqrt{K}\|\X\|}$. 

which implies that
\begin{itemize}
\item If $\delta=\frac{\zeta\sigma B\opnorm{\X}}{\alpha}$: For \eqref{epsass} to hold it suffices to have $\eps_0\le\frac{\alpha}{5} \min\left(\frac{\zeta\sigma B\opnorm{\X}}{\alpha},\sqrt{\frac{\zeta}{\Gamma}}\right)$.
\item If $\delta=\frac{\upp}{\Gamma \tn{\rb_0}}$: For \eqref{epsass} to hold it suffices to have $\eps_0\le \frac{\alpha}{5}\sqrt{c\frac{\upp\alpha}{\sigma B\Gamma^2\tn{\rb_0}\opnorm{\X}}}$ as based on \eqref{rhs bound} we have $\sqrt{\frac{c\alpha}{\beta\Gamma}}=\sqrt{\frac{c\alpha}{\sigma B\Gamma\opnorm{\X}}}\le \sqrt{\delta}$
\begin{align*}
 \eps_0\le&\frac{\alpha}{5}\sqrt{\frac{c\upp\alpha}{\sigma B\Gamma^2\tn{\rb_0}\opnorm{\X}}}\\
 =&\frac{\alpha}{5}\sqrt{\delta}\sqrt{\frac{c\alpha}{\Gamma\beta}}\\
=&\frac{\alpha}{5}\sqrt{\delta}\cdot\min\left(\sqrt{\delta},\sqrt{\frac{c\alpha}{\Gamma\beta}}\right)\\
=& \frac{\alpha}{5}\min\left(\delta,\sqrt{\frac{\delta\alpha}{\Gamma\beta}}\right)
 %\frac{\alpha}{5}\min(\frac{c\alpha}{\Gamma \sigma B \|\X\|}, \frac{\sqrt{c}\alpha}{\Gamma \sigma B \|\X\|})
\end{align*}
\end{itemize}
Combining the latter two cases as long as
\begin{align*}
\eps_0^2\le \frac{\alpha^2}{25}\min\left(c\frac{\upp\alpha}{\sigma B\Gamma^2\tn{\rb_0}\opnorm{\X}},\frac{\zeta^2\sigma^2 B^2\opnorm{\X}^2}{\alpha^2},\frac{\zeta}{\Gamma}\right)\quad\Leftrightarrow \quad\eqref{ref bound eps},
\end{align*}
then \eqref{epsass} holds. As a result when \eqref{ref bound eps} and \eqref{k bound det} hold with $\delta=\min\left(\frac{\zeta\sigma B\opnorm{\X}}{\alpha},\frac{\upp}{\Gamma \tn{\rb_0}}\right)$ both assumptions of Theorem \ref{nn deter} also hold and so do its conclusions. In particular, \eqref{main res eq23} follows from \eqref{main res eq22} by noting that based on our choice of $\delta$ we have $\delta\frac{\Gamma}{\alpha}\twonorm{\rb_0}\le \frac{\upp}{\alpha}$, \eqref{row boundsss2} follows immediately from \eqref{row boundsss}, and \eqref{eqqq23} follows from \eqref{eqqq22} by noting that based on our choice of $\delta$ we have $\frac{\delta\alpha}{\sigma B\opnorm{\X}}\le \zeta$.
\end{proof}

\subsection{Main Generalization Result}

\begin{theorem} \label{nn deter gennn}Let $(\x_i,\y_i)_{i=1}^n\distas \Dc$ be a dataset where inputs have unit Euclidian norm. Consider a neural net with $k$ hidden layers as described in \eqref{neural net func} and parameterized by $\bteta:=\text{vect}(\W)$. Let $\W_0$ be the initialization. Suppose $|\phi(0)|,|\phi'|,|\phi''|\leq B$. Let output matrix $\Vb$ be such that $\tin{\Vb}\leq \frac{\vrn}{\sqrt{\K k}}$. Let $\sigma B\|\X\|\geq \alpha>0$ be the cutoff level and $\zeta>0$ be the error tolerance. Fix fast and slow subspaces $\Rc$ and $\Rcb$ with respect to initial Jacobian $\Jc(\W_0)$ with cutoff $\alpha$. Let the initial residual vector be $\rb_0=\y-f(\W_0)\in\R^{n\K}$ and let $C_r>0$ be a number satisfying $\tn{\rb_0}\leq C_r\sqrt{n}$. Also pick the information space large enough to guarantee $ \tn{\Pi_{\Rc}(\rb_0)}\geq c\tn{\rb_0}$ for some constant $c>0$. Set $\bar{\alpha}=\frac{\alpha}{\sigma B \|\X\|}$ and assume number of hidden nodes $k$ obeys%Suppose the initial residual and the number of hidden nodes satisfy
%=\sigma \bar{\alpha}B\|\X\|
\begin{align}
 k\gtrsim\frac{C_r^2\Gamma^4n^4}{\|\X\|^4\bar{\alpha}^8\vrn^2\zeta^2}.\label{k bound det gen}
\end{align}
Set $\eta\leq \frac{1}{\vrn^2B^2\|\X\|^2}$ and fix $\Gamma\geq 1$. After $\tau_0=\frac{\Gamma}{\eta\alpha^2}$, iterations, with probability $1-\delta$, the classification error 
\begin{align}
\err{\W}=\Pro(\arg\max_{1\leq i\leq K}\y_i\neq \arg\max_{1\leq i\leq K}f_i(\x,\W))\label{class error2}
\end{align}
satisfies
\begin{align}% \frac{\tn{ \Pi_{\bar{\Rc}}(\y)}+ \exp(-\Gamma)\tn{\Pi_{{\Rc}}(\y)}+\dpz}{\sqrt{n}}+\zeta\approx  
\err{\W_{\tau_0}}&\leq \underbrace{\frac{2\tn{ \Pi_{\bar{\Rc}}(\rb_0)}}{\sqrt{n}}}_{bias~term}+\underbrace{\frac{12\vrn B \dpp}{\sqrt{n}}}_{variance~term}+5\sqrt{\frac{\log(2/\delta)}{n}}+2C_r(\exp(-\Gamma)+\zeta).
\end{align}
\end{theorem}
\begin{proof}
%First, we plug $\alpha$ in \eqref{k condition} of Theorem \ref{apply 1} to obtain
%\[
%k\geq \order{\frac{\Gamma^4 \vrn^6n^2\|\X\|^4\log^2(2n)}{\alpha^8}}.
%\]
First, using $\tn{\rb_0}\leq  C_r\sqrt{n}$ and \eqref{upp up bound} and observing $\frac{\alpha}{ \sigma B\|\X\|}\leq1\leq  \frac{\Gamma \tn{\rb_0}}{\upp}\leq C_r \frac{\Gamma\sqrt{n}}{\upp}$. We will apply Theorem \ref{nn deter2} with $\eps_0=0$. The statement of Theorem \ref{nn deter2} is implied by
\[
k\gtrsim\frac{C_r^2\Gamma^4\vrn^6B^6\|\X\|^4n^4}{\alpha^8\zeta^2}.
\]
We shall apply \eqref{err pop bound} of Lemma \ref{generalize corollary} with $M$ and $R$ dictated by Theorem \ref{nn deter2} and setting $\bar{M}=0$. Observing, $\tf{\Vb}\leq \sqrt{\K k}\tin{\Vb}\leq \vrn$, we have
\[
\err{\W}\leq 2\left[\sqrt{\Lc(\W)}+3\sigma B(\frac{M}{\sqrt{n}}+\frac{R^2}{\sqrt{k}})+\sqrt{\frac{5\log(2/\delta)}{n}}\right],
\]
where $\Lc(\W)$ is the averaged least-squares loss as in Lemma \ref{generalize corollary}. Theorem \ref{nn deter2} yields
\begin{align}
\sqrt{\Lc(\W)}=\frac{\tn{f(\W_{\tau_0})-\y}}{\sqrt{n}}&\leq \frac{ \tn{ \Pi_{\bar{\Rc}}(\rb_0)}+ (\exp(-\Gamma)+\zeta/2)\tn{\rb_0}}{\sqrt{n}}\\
&\leq \frac{ \tn{ \Pi_{\bar{\Rc}}(\rb_0)}}{\sqrt{n}}+C_r(\exp(-\Gamma)+\zeta/2).
\end{align}
Using \eqref{main res eq23} on $M$
\begin{align}
\frac{{\vrn} BM}{\sqrt{n}}\leq {\frac{2 \vrn B \upp}{\alpha\sqrt{n}}}.
\end{align}
Using \eqref{row boundsss2} on row bound $R$ and lower bound \eqref{k bound det gen} on $k$
\begin{align}
%{\vrn} BR^2\sqrt{k}\leq \order{\frac{B^3\Gamma^2\K^2 \|\X\|^2n}{\sigma\sqrt{k}\alpha_0^4}}&\leq\order{\frac{B^3\Gamma^2\K^2 \|\X\|^2n}{\sigma\alpha_0^4} C\frac{\zeta^2\alpha_0^4}{\Gamma^4n\|\X\|^2\K^2B^4\log(2n)}}\\
\frac{\sigma B R^2}{\sqrt{k}}\leq \frac{ 4C_r^2\Gamma^2 \vrn^3 B^3n\|\X\|^2}{\sqrt{k}\alpha^4}.
&\leq C_r\zeta/2% \frac{\zeta\alpha_0^2}{B}\leq \zeta.% \order{\frac{1}{\sigma} C\frac{\zeta^2}{B\log(2n)}}\leq \zeta.
\end{align}
Combining the three bounds above, we obtain the advertised population classification error of 
\[
2[\frac{ \tn{ \Pi_{\bar{\Rc}}(\rb_0)}}{\sqrt{n}}+C_r(\exp(-\Gamma)+\zeta/2)+6{\frac{2\vrn B \upp}{\alpha\sqrt{n}}}+C_r\zeta/2]
\]
To proceed, substituting $\bar{\alpha}=\frac{\alpha}{\sigma B\|\X\|}$, we find the $k$ requirement to be implied by \eqref{k bound det gen}. Secondly substituting $\dpp=\upp/\alpha$, we conclude with the main result.
\end{proof}

==> proofsApp.tex <==




==> proofs_06_06.tex <==
% !TEX root = shorter_arxiv.tex
\section{Proofs}
Before we proceed with the proof let us briefly discuss some notation used throughout. For a matrix $\mtx{W}\in\R^{k\times d}$ we use vect$(\mtx{W})\in\R^{kd}$ to denote a vector obtained by concatenating the rows $\vct{w}_1,\vct{w}_2,\ldots,\vct{w}_k\in\R^d$ of $\mtx{W}$. That is,
$\text{vect}(\W)=\begin{bmatrix}\vct{w}_1^T&\vct{w}_2^T &\ldots &\vct{w}_k^T\end{bmatrix}^T$. Similarly, we use $\mat(\vct{w})\in\R^{k\times d}$ to denote a $k\times d$ matrix obtained by reshaping the vector $\vct{w}\in\R^{kd}$ across its rows. Throughout, for a differentiable function $\phi:\R\mapsto\R$ we use $\phi'$ and $\phi''$ to denote the first and second derivative. 
\subsection{Proofs for General Theory (Proof of Theorem \ref{many step thm})}
In this section we prove our result for general nonlinearities. We begin with a few notations and definitions and preliminary lemmas in Section \ref{prelim5}. Next in Section \ref{key5} we prove some key lemmas regarding the evolution of the linearized residuals $\rbb_\tau$. In Section \ref{radam} we establish some key Rademacher complexity results used in our generalization bounds. Finally, in Section \ref{comp5} we use these results to complete the proof of Theorem \ref{many step thm}.
\subsubsection{Preliminary definitions and lemmas}
\label{prelim5}
Throughout we use 
\begin{align*}
\mtx{U}_{\mathcal{I}}=\begin{bmatrix}\vct{u}_1 & \vct{u}_2 & \ldots & \vct{u}_r\end{bmatrix}\in\R^{nK\times r}
\quad\text{and}\quad
\mtx{U}_{\mathcal{N}}=\begin{bmatrix}\vct{u}_{r+1} & \vct{u}_{r+2} & \ldots & \vct{u}_{nK}
\end{bmatrix}\in\R^{nK\times (nK-r)}. 
\end{align*}
to denote the basis matrices for the information and nuisance subspaces from Definition \ref{tjac2}. Similarly, we define the information and nuisance spectrum as 
\begin{align*}
\vct{\lambda}_{\mathcal{I}}=
\begin{bmatrix}
\lambda_1&
\lambda_2&
\ldots&
\lambda_r
\end{bmatrix}^T
\quad\text{and}\quad
\vct{\lambda}_{\mathcal{N}}=
\begin{bmatrix}
\lambda_{r+1}&
\lambda_{r+2}&
\ldots&
\lambda_{nK}
\end{bmatrix}^T.
\end{align*}
We also define the diagonal matrices 
\begin{align*}
\mtx{\Lambda}=\text{diag}(\vct{\lambda}),\quad \mtx{\Lambda}_{\calF}=\text{diag}(\vct{\lambda}_{\calF}),\quad\text{and}\quad\mtx{\Lambda}_{\calS}=\text{diag}(\vct{\lambda}_{\calS}).
\end{align*}
\begin{definition}[early stopping value and distance]\label{earlyval} Consider Definition \ref{tjac2} and let $\Gamma>0$ be a positive scalar. Associated with the initial residual $\rb_0=f(\bteta_0)-\y$ and the information/nuisance subspaces of the reference Jacobian $\mtx{J}$ (with a cut-off level $\alpha$) we define the $(\alpha,\Gamma)$ early stopping value as
%\sqrt{\twonorm{\mtx{D}_{\alpha/\vct{\lambda}_{\mathcal{F}}}\mtx{F}^T\vct{r}_0}^2+\twonorm{\mtx{D}_{\vct{\lambda}_{\mathcal{S}}/\alpha}\mtx{S}^T\vct{r}_0}^2}
\begin{align}
\upp=&\left(\sum_{s=1}^r  \frac{\alpha^2}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2+\Gamma^2\sum_{s=r+1}^{nK}\frac{\la_s^2}{\alpha^2} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}.\label{pinv def2}
\end{align}%\\=&\left(\sum_{i=1}^r  \frac{\alpha^2}{\la_i^2}a_i^2+\Gamma^2\sum_{i=r+1}^n\frac{\la_i^2}{\alpha^2} a_i^2\right)^{1/2}
We also define the early stopping distance as
\begin{align*}
\dpp=\frac{\upp}{\alpha}.
\end{align*}
\end{definition}
The goal of early stopping value/distance is understanding the behavior of the algorithm at a particular stopping time that depends on $\Gamma$ and the spectrum cutoff $\alpha$. In particular, as we will see later on the early stopping distance characterizes the distance from initialization at an appropriate early stopping time. We continue by stating and proving a few simple lemmas. The first Lemma provides upper/lower bounds on the early stopping value.
\begin{lemma}[Bounds on Early-Stopping Value]\label{bndearlystopval} The early stopping value $\upp$ from Definition \ref{earlyval} obeys
\begin{align}
&\upp\leq  \left(\tn{\Pi_{\Rc}(\rb_0)}^2+{\Gamma}^2\tn{\Pi_{\Rcb}(\rb_0)}^2\right)^{1/2}\le \Gamma\twonorm{\rb_0}\label{upp up bound}\\
&\upp\geq \frac{\alpha}{\la_1}\twonorm{\Pi_{\Rc}(\rb_0)}.\label{low bound}
\end{align}
\end{lemma}
\begin{proof}
To prove the upper bound we use the fact that $\alpha\le \la_s$ for $s\le r$ and $\alpha\geq \la_s$ for $s\geq r$ to conclude that
\begin{align*}
\upp &\le \left(\sum_{s=1}^r \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2+\Gamma^2\sum_{s=r+1}^{nK} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}\\
&= \left(\twonorm{\Pi_{\Rc}(\rb_0)}^2+{\Gamma}^2\twonorm{\Pi_{\Rcb}(\rb_0)}^2\right)^{1/2}\\
&\leq \Gamma \tn{\rb_0}.
\end{align*}
To prove the lower bound, we use the facts that $\alpha^2/\la_s^2\geq \alpha^2/\la_1^2$ to conclude that
\begin{align*}
\upp=&\left(\sum_{s=1}^r  \frac{\alpha^2}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2+\Gamma^2\sum_{s=r+1}^{nK}\frac{\la_s^2}{\alpha^2} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2},\\
\ge&\left(\sum_{s=1}^r  \frac{\alpha^2}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2},\\
\ge&\frac{\alpha}{\lambda_1}\twonorm{\Pi_{\Rc}(\rb_0)}.
\end{align*}
\end{proof}
It is of course well known that the mapping $\left(\mtx{I}-\eta\A\A^T\right)$ is a contraction for sufficiently small values of $\eta$. The next lemma shows that if we replace one of the $\A$ matrices with a matrix $\B$ which is close to $\A$ the resulting matrix $\left(\mtx{I}-\eta\A\B^T\right)$, while may not be contractive, is not too expansive.
\begin{lemma} [Asymmetric PSD increase]\label{asym pert} Let $\A,\B\in\R^{n\times p}$ be matrices obeying 
\begin{align*}
\opnorm{\A}\le \beta,\quad\opnorm{\B}\le \beta,\quad\text{and}\quad\opnorm{\B-\A}\leq \eps.
\end{align*}
Then, for all $\rb\in\R^n$ and $\eta\leq 1/\beta^2$ we have
\[
\twonorm{\left(\Iden-\eta \A\B^T\right)\rb}\le \left(1+\eta\eps^2\right)\twonorm{\rb}.%2\eps\tn{\Jb^T\rb}\tn{\rb}+\eps^2\tn{\rb}^2.
\]
\end{lemma}
\begin{proof} Note that using $\eta\leq 1/\beta^2$ and $\opnorm{\B-\A}\leq \eps$ we conclude that
\begin{align*}
\twonorm{\left(\Iden-\eta \A\B^T\right)\rb}^2=&\twonorm{\left(\Iden-\eta \B\B^T-\eta(\A-\B)\B^T\right)\rb}^2\\
=&\twonorm{\rb-\eta(\A-\B+\B)\B^T\rb}^2\\
=&\twonorm{\rb}^2-2\eta\rb^T(\A-\B+\B)\B^T\rb+\eta^2\twonorm{\A\B^T\rb}^2\\
\le& \twonorm{\rb}^2-2\eta\tn{\B^T\rb}^2+2\eta \twonorm{(\A-\B)^T\rb}\tn{\B^T\rb}+\eta^2\|\A\|^2\tn{\B^T\rb}^2\\
=& \twonorm{\rb}^2-\eta\tn{\B^T\rb}^2+2\eta \twonorm{(\A-\B)^T\rb}\tn{\B^T\rb}+\left(\eta^2\|\A\|^2\tn{\B^T\rb}^2-\eta\tn{\B^T\rb}^2\right)\\
\overset{\eta\le 1/\beta^2}{\leq}&\twonorm{\rb}^2-\eta\tn{\B^T\rb}^2+2\eta \twonorm{(\A-\B)^T\rb}\tn{\B^T\rb}\\
\overset{\opnorm{\A-\B}\le \epsilon}{\le} & \twonorm{\rb}^2-\eta\tn{\B^T\rb}^2+2\eta \eps\tn{\B^T\rb}\tn{\rb}\\
=&(1+\eta\eps^2)\twonorm{\rb}^2-\eta\left(\eps\twonorm{\rb}-\twonorm{\B^T\rb}\right)^2\\
\le&(1+\eta\eps^2)\twonorm{\rb}^2,
%&\leq \tn{\rb}^2-2\eta\tn{\B^T\rb}^2+\eta^2\tn{\B\B^T\rb}^2+2\eta \tn{(\A-\B)^T\rb}\tn{\B^T\rb}+2\eta^2\|\A-\B\|\|\B\|\tn{\B^T\rb}^2+\eta^2\|\A-\B\|^2\tn{\B^T\rb}^2%\tn{\rb}^2-2\eta \rb^T \A\B^T\rb+\eta^2\tn{ \A\B^T\rb}^2.
\end{align*}
completing the proof.
\end{proof}
The next lemma shows that if two PSD matrices are close to each other then an appropriate square root of these matrices will also be close.
\begin{lemma}\label{psd pert} Let $\A$ and $\B$ be $n\times n$ positive semi-definite matrices satisfying $\|\A-\B\|\leq \alpha^2$ for a scalar $\alpha\ge 0$. Then for any $\X\in\R^{n\times p}$ with $p\geq n$ obeying $\A=\X\X^T$, there exists a matrix $\Y\in\R^{n\times p}$ obeying $\B=\Y\Y^T$ such that
\[
\|\Y-\X\|\leq 2\alpha
\]
\end{lemma}
\begin{proof}
%\[
%\Jb^T\sum_{t=1}^{\tau-1}(\Iden-\Jb\Jb^T)^t \rb
%\]
First we note that for any two PSD matrices $\A_+, \B_+\in\R^{n\times n}$ obeying $\A_+,\B_+\succeq \frac{\alpha^2}{4}\Iden_n$, Lemma 2.2 of \cite{schmitt1992perturbation} guarantees that
\[
\opnorm{\A_+^{1/2}-\B_+^{1/2}}\leq \frac{\|\A_+-\B_+\|}{\alpha}.
\]
In the above for a PSD matrix $\A\in\R^{n\times n}$ with an eigenvalue decomposition $\A=\mtx{U}\mtx{\Lambda}\mtx{U}^T$ we use $\A^{1/2}$ to denote the square root of the matrix given by $\A=\mtx{U}\mtx{\Lambda}^{1/2}\mtx{U}^T$. We shall use this result with $\A_+=\A+\frac{\alpha^2}{4}\Iden_n$ and $\B_+=\B+\frac{\alpha^2}{4}\Iden_n$ to conclude that
\[
\opnorm{\A_+^{1/2}-\B_+^{1/2}}\leq \frac{\opnorm{\A_+-\B_+}}{\alpha}=\frac{\opnorm{\A-\B}}{\alpha}.
\]
Furthermore, using the fact that the eigenvalues of $\A_+$ and $\B_+$ are just shifted versions of the eigenvalues of $\A$ and $\B$ by $\alpha^2/4$ we can conclude that
\[
\opnorm{\A_+^{1/2}-\A^{1/2}}\le \frac{\alpha}{2}\quad\text{and}\quad\opnorm{\B_+^{1/2}-\B^{1/2}}\leq\frac{\alpha}{2}.
\]
Combining the latter two inequalities with the assumption that $\opnorm{\A-\B}\le \alpha^2$ we conclude that
\begin{align}
\label{tempkey1}
\opnorm{\A^{1/2}-\B^{1/2}}\le& \opnorm{\A_+^{1/2}-\B_+^{1/2}}+\opnorm{\A_+^{1/2}-\A^{1/2}}+\opnorm{\B_+^{1/2}-\B^{1/2}}\nn\\
\le&\frac{\opnorm{\A-\B}}{\alpha}+\frac{\alpha}{2}+\frac{\alpha}{2}\nn\\
\le&2\alpha.
\end{align}
Suppose $p\geq n$ and assume the matrices $\A$ and $\B$ have eigenvalue decompositions given by $\A=\Ub_{\A}\La_{\A}\Ub_{\A}^T$ and $\B=\Ub_{\B}\La_{\B}\Ub_{\B}^T$. Then, any $\X\in\R^{n\times p}$ with $p\ge n$ has the form $\X=\mtx{U}_{\A}\La_{\A}^{1/2}\mtx{V}_{\A}^T$ with $\mtx{V}_{\A}\in\R^{p\times n}$ an orthonormal matrix. Now pick
\begin{align*}
\Y= \Ub_{\B}\La_{\B}^{1/2}\Ub_{\B}^T\mtx{U}_{\A}\mtx{V}_{\A}^T.
\end{align*}
Then clearly $\Y\Y^T=\B$. Furthermore, we have
\begin{align*}
\opnorm{\X-\Y}=&\opnorm{\mtx{U}_{\A}\La_{\A}^{1/2}\mtx{V}_{\A}^T-\Ub_{\B}\La_{\B}^{1/2}\Ub_{\B}^T\mtx{U}_{\A}\mtx{V}_{\A}^T}\\
=&\opnorm{\mtx{U}_{\A}\La_{\A}^{1/2}\mtx{U}_{\A}^T\mtx{U}_{\A}\mtx{V}_{\A}^T-\Ub_{\B}\La_{\B}^{1/2}\Ub_{\B}^T\mtx{U}_{\A}\mtx{V}_{\A}^T}\\
=&\opnorm{\left(\mtx{U}_{\A}\La_{\A}^{1/2}\mtx{U}_{\A}^T-\Ub_{\B}\La_{\B}^{1/2}\Ub_{\B}^T\right)\mtx{U}_{\A}\mtx{V}_{\A}^T}\\
=&\opnorm{\left(\A^{1/2}-\B^{1/2}\right)\mtx{U}_{\A}\mtx{V}_{\A}^T}\\
=&\opnorm{\A^{1/2}-\B^{1/2}}.
\end{align*}
Combining the latter with \eqref{tempkey1} completes the proof. 
%Next, assume $p<n$. Let $\B_p$ be the rank-$p$ approximation of $\B$. Using Weyl's eigenvalue inequality, $\text{rank}(\A)=p$, and the fact that $\|\A-\B\|\leq \alpha^2$, we find that $\|\B_p-\B\|\leq\alpha^2\implies \|\A-\B_p\|\leq 2\alpha^2$. Now, let $\A=\Ub_{\A}\La_{\A}\Ub_{\A}^T$ and $\B_p=\Ub_{\B}\La_{\B}\Ub_{\B}^T$ with $n\times p$ matrices $\Ub_\A,\Ub_\B$ and $\X=\mtx{U}_{\A}\La_{\A}^{1/2}\mtx{V}_{\A}^T$ with $\mtx{V}_{\A}\in\R^{p\times p}$. Define the matrix
%\[
%\Y= \Ub_{\B}\La_{\B}^{1/2}\Ub_{\B}^T\mtx{U}_{\A}\mtx{V}_{\A}^T.
%\]
\end{proof}

\subsubsection{Key lemmas for general nonlinearities}
\label{key5}
Throughout this section we assume $\Jb$ is the reference Jacobian per Definition \ref{tjac} with eigenvalue decomposition $\Jb=\Ub\mtx{\Lambda}\Vb^T=\sum_{s=1}^{\K n} \la_s\ub_s\vb_s^T$ with $\mtx{\Lambda}=\text{diag}(\vct{\la})$. We also define $\vct{a}=\mtx{U}^T\rb_0=\mtx{U}^T\widetilde{\rb}_0\in\R^{nK}$ be the coefficients of the initial residual in the span of the column space of this reference Jacobian. 

We shall first characterize the evolution of the linearized parameter $\bbteta_\tau$ and residual $\rbb_{\tau}$ vectors from \eqref{lin res eq} in the following lemma.
\begin{lemma} \label{lem linear} The linearized residual vector $\rbb_{\tau}$ can be written in the form
\begin{align}
\rbb_\tau=\mtx{U}\left(\Iden-\eta\mtx{\Lambda}^2\right)^\tau\vct{a}=\sum_{s=1}^{nK} (1-\eta \la_s^2)^{\tau} a_s\ub_s.\label{res result}
\end{align}
Furthermore, assuming $\eta\leq 1/\la_1^2$ the linear updates $\bbteta_\tau$ obey% let $\bbteta$ be the linearized pseudo-inverse given by $\bbteta=\brteta_\infty$ satisfying
\begin{align}
\label{tetaresult}
\tn{\bbteta_\tau-\bbteta_0}^2\leq\sum_{s=1}^r  \frac{a_s^2}{\la_s^2}+\tau^2\eta^2\sum_{s=r+1}^{nK} \la_s^2 a_s^2.
% \sum_{i=1}^r  \frac{a_i^2}{\la_i^2}+\sum_{i=r+1}^n\tau^2\eta^2 \la_i^2 a_i^2\leq  \sum_{i=1}^r  \frac{a_i^2}{\la_i^2}+\tau^2\eta^2 \alpha^2\tn{\Pi_{\Rcp}(\rb_0)}^2.\label{pinv def}%\Jb^\dagger \Pi_{\Rc}(\rb_0).
\end{align}%=\sqrt{\rb_0^T(\Jb\Jb^T)^{-1}\rb_0}
\end{lemma}
\begin{proof}
Using the fact that $\Jb\Jb^T=\mtx{U}\mtx{\Lambda}^2\mtx{U}^T$ we have
\begin{align*}
(\Iden-\eta\Jb\Jb^T)^\tau=\mtx{U}\left(\Iden-\eta\mtx{\Lambda}^2\right)^\tau\mtx{U}^T
\end{align*}
Using the latter combined with \eqref{lin res eq} we thus have
\begin{align*}
\rbb_{\tau}=&(\Iden-\eta\Jb\Jb^T)^\tau\rb_0,\\
=&\mtx{U}\left(\Iden-\eta\mtx{\Lambda}^2\right)^\tau\mtx{U}^T\rb_0,\\
=&\mtx{U}\left(\Iden-\eta\mtx{\Lambda}^2\right)^\tau\vct{a},\\
=&\sum_{s=1}^{nK} (1-\eta \la_s^2)^{\tau} a_s\ub_s,
\end{align*}
completing the proof of \eqref{res result}.

We now turn our attention to proving \eqref{tetaresult} by tracking the representation of $\bbteta_\tau$ in terms of the right singular vectors of $\Jb$. To do this note that using \eqref{res result} we have
\begin{align*}
\Jb^T\rbb_t=\mtx{V}\mtx{\Lambda}\mtx{U}^T\rbb_t=\mtx{V}\mtx{\Lambda}\left(\Iden-\eta\mtx{\Lambda}^2\right)^t\vct{a}.
\end{align*}
Using the latter together with the gradient update on the linearized problem we have
\begin{align*}
\bbteta_\tau-\bbteta_0=&-\eta\left(\sum_{t=0}^{\tau-1}\nabla \mathcal{L}_{lin}(\bbteta_t)\right)=-\eta\left(\sum_{t=0}^{\tau-1}\Jb^T\rbb_t\right)=-\eta\mtx{V}\left(\sum_{t=0}^{\tau-1}\mtx{\Lambda}\left(\Iden-\eta\mtx{\Lambda}^2\right)^t\right)\vct{a}.
\end{align*}
Thus for any $s\in\{1,2,\ldots,nK\}$
\begin{align*}
\vct{v}_s^T\left(\bbteta_\tau-\bbteta_0\right)=-\eta\lambda_s\vct{a}_s\left(\sum_{t=0}^{\tau-1}\left(1-\eta\lambda_s^2\right)^t\right)=-\eta\lambda_s\vct{a}_s\frac{1-\left(1-\eta\lambda_s^2\right)^\tau}{\eta\lambda_s^2}=-\vct{a}_s\frac{1-\left(1-\eta\lambda_s^2\right)^\tau}{\lambda_s}.
\end{align*}
Noting that for $\eta\le 1/\lambda_1^2\le 1/\lambda_s^2$ we have $1-\eta\lambda_s^2\ge 0$, the latter identity implies that
\begin{align}
\label{vproj1}
\abs{\vct{v}_s^T\left(\bbteta_\tau-\bbteta_0\right)}\le \frac{\abs{\vct{a}_s}}{\lambda_s}.
\end{align}
Furthermore, using the fact that $1-\eta\lambda_s^2\le 1$ we have
\begin{align}
\label{vproj2}
\abs{\vct{v}_s^T\left(\bbteta_\tau-\bbteta_0\right)}=\eta\lambda_s\abs{\vct{a}_s}\left(\sum_{t=0}^{\tau-1}\left(1-\eta\lambda_s^2\right)^t\right)\le \eta\lambda_s\abs{\vct{a}_s}\tau
\end{align}
Combining \eqref{vproj1} for $1\le s\le r$ and \eqref{vproj2} for $s>r$ we have
\[
\twonorm{\bbteta_\tau-\bbteta_0}^2=\sum_{s=1}^{nK} \abs{\vct{v}_s^T\left(\bbteta_\tau-\bbteta_0\right)}^2\leq \sum_{s=1}^r  \frac{a_s^2}{\la_s^2}+\tau^2\eta^2\sum_{s=r+1}^{nK} \la_s^2 a_s^2,%\leq  \sum_{i=1}^r  \frac{a_i^2}{\la_i^2}+\tau^2 \alpha^2\sum_{i=r+1}^n a_i^2.
\]
completing the proof of \eqref{tetaresult}.
\end{proof}
%\begin{itemize}
%\item For $i\leq r$, we find that
%\item For $i> r$
%\end{itemize}
%Since $\vb_i$'s are orthonormal, we find $\tn{\bbteta_\tau-\bteta_0}\leq B_{\Jb}$.
% \textcolor{red}{CLARIFY}
For future use we also state a simple corollary of the above Lemma below.
\begin{corollary}\label{cor simp} Consider the setting and assumptions of Lemma \ref{lem linear}. Then, after $\tau$ iterations we have
\begin{align}
\label{cor76conc1}
\twonorm{\rbb_\tau}\le \left(1-\eta\alpha^2\right)^\tau\tn{\Pi_{\Rc}(\rb_0)}+\tn{\Pi_{\Rcb}(\rb_0)}.
\end{align}
Furthermore, after $T=\frac{\Gamma}{\eta\alpha^2}$ iterations we have
\begin{align}
\label{cor76conc2}
\tn{\rbb_T}\le e^{-\Gamma}\tn{\Pi_{\Rc}(\rb_0)}+\tn{\Pi_{\Rcb}(\rb_0)}.
\end{align}
and
\begin{align*}
&\twonorm{\bbteta_T-\bbteta_0}^2\leq \sum_{s=1}^r  \frac{\vct{a}_s^2}{\la_s^2}+\Gamma^2\sum_{s=r+1}^{nK}\frac{\la_s^2 \vct{a}_s^2}{\alpha^4}=\frac{\upp^2}{\alpha^2}.
%&\tn{\bbteta_\tau-\bteta_0}\leq \frac{\upp}{\alpha}.
\end{align*}
with $\upp$ given by \eqref{pinv def2} per Definition \ref{bndearlystopval}.
\end{corollary}
\begin{proof} 
To prove the first bound on the residual (\eqref{cor76conc1})note that using \eqref{res result} we have
\begin{align*}
\mtx{U}_{\mathcal{I}}^T\rbb_\tau=\left(\mtx{I}-\eta\Lambda_{\calF}^2\right)^\tau\mtx{U}_{\mathcal{I}}^T\rbb_0\quad \text{and}\quad\mtx{U}_{\mathcal{N}}^T\rbb_\tau=\left(\mtx{I}-\eta\Lambda_{\calS}^2\right)^\tau\mtx{U}_{\calS}^T\rbb_0
\end{align*}
Thus, using the fact that for $s\leq r$ we have $\lambda_s\ge \alpha$ we have $(1-\eta\la_s^2)^{\tau}\leq(1-\eta\alpha^2)^{\tau}$ and for $s>r$ we have $(1-\eta\la_s^2)^{\tau}\le 1$, we can conclude that
\begin{align*}
\twonorm{\mtx{U}_{\mathcal{I}}^T\rbb_\tau}\le \left(1-\eta\alpha^2\right)^\tau\twonorm{\mtx{U}_{\mathcal{I}}^T\rb_0}\quad\text{and}\quad\twonorm{\mtx{U}_{\mathcal{N}}^T\rbb_\tau}\le \twonorm{\mtx{U}_{\mathcal{N}}^T\rb_0}.
\end{align*}
Combining these with the triangular inequality we have
\begin{align*}
\twonorm{\rbb_\tau}=\twonorm{\begin{bmatrix}\mtx{U}_{\mathcal{I}}^T\rbb_\tau\\\mtx{U}_{\mathcal{N}}^T\rbb_\tau\end{bmatrix}}\le\twonorm{\mtx{U}_{\mathcal{I}}^T\rbb_\tau}+\twonorm{\mtx{U}_{\mathcal{N}}^T\rbb_\tau}\le\left(1-\eta\alpha^2\right)^\tau\twonorm{\mtx{U}_{\mathcal{I}}^T\rb_0}+\twonorm{\mtx{U}_{\mathcal{N}}^T\rb_0},
\end{align*}
concluding the proof of \eqref{cor76conc1}. The second bound on the residual simply follows from the fact that $(1-\eta\alpha^2)^{T}\leq e^{-\Gamma}$. The bound on $\twonorm{\bbteta_T-\bbteta_0}^2$ is trivially obtained by using $T^2=\frac{\Gamma^2}{\eta^2\alpha^4}$ in \eqref{tetaresult}.
\end{proof}
The lemma above shows that with enough iterations, gradient descent on the linearized problem fits the residual over the information space and the residual is (in the worst case) unchanged over the nuisance subspace $\Rcb$. Our hypothesis is that, when the model is generalizable the residual mostly lies on the information space $\Rc$ which contains the directions aligned with the top singular vectors. Hence, the smaller term $\tn{\Pi_{\mathcal{N}}(\rb_0)}$ over the nuisance space will not affect generalization significantly. To make this intuition precise however we need to connect the residual of the original problem to that of the linearized problem. The following lemma sheds light on the evolution of the original problem \eqref{nonlin gd} by characterizing the evolution of the difference between the residuals of the original and linearized problems from one iteration to the next.
\begin{lemma}[Keeping track of perturbation - one step]\label{grwth} Assume Assumptions \ref{ass2} and \ref{ass3} hold and $\bteta_{\tau}$ and $\bteta_{\tau+1}$ are within an $R$ neighborhood of $\bteta_0$, that is,
\begin{align*}
\twonorm{\bteta_{\tau}-\bteta_0}\le R\quad\text{and}\quad\twonorm{\bteta_{\tau+1}-\bteta_0}\le R.
\end{align*}
Then with a learning rate obeying $\eta\leq 1/\beta^2$, the deviation in the residuals of the original and linearized problems $\eb_{\tau+1}=\rb_{\tau+1}-\rbb_{\tau+1}$ obey
\begin{align}
\tn{\eb_{\tau+1}}&\leq \eta(\eps_0^2+\eps\beta)\tn{\rbb_{\tau}}+(1+\eta\eps^2)\tn{\eb_{\tau}}.\label{etau repeat}
\end{align}
%Given vectors $\rb,\rbb,\eb=\rb-\rbb$ and matrices $\A,\B,\Jb$ satisfying $\|\B-\Jb\|,\|\A-\Jb\|\leq \eps/2$ and $\|\A\|,\|\B\|,\|\Jb\|\leq \beta$, for $\eta\leq 1/\beta^2$, we have that
%\begin{align}
%\tn{(\Iden-\eta\B\A^T)\rb-(\Iden-\eta\Jb\Jb^T)\rbb}&\leq \eta\eps\beta\tn{\rbb}+(1+\eta\eps^2)\tn{\eb}.\label{first statement}
%\end{align}
 %Let $\Jb$ be same as in Definition \ref{tjac}. 
%Given $\rb,\rbb,\eb=\rb-\rbb$ and matrices $\A,\B,\Jb$ satisfying $\|\B-\Jb\|,\|\A-\Jb\|\leq \eps/2$ and $\|\A\|,\|\B\|,\|\Jb\|\leq \beta$ and $\smn{\Jb},\smn{\B},\smn{\A}\geq 2\bn$ where $\eps\leq \bn$. 
\end{lemma}
%we can apply \eqref{first statement} with and $\rbb_\tau=\rbb$, $\rb_\tau=\rb$, $\eb_\tau=\eb$ to control the evolution of $\eb_{\tau+1}$ to get \eqref{etau repeat}. W
\begin{proof} For simplicity, denote $\B_1=\Jc(\bteta_{\tau+1},\bteta_\tau)$, $\B_2=\Jc(\bteta_\tau)$, $\A=\Jc(\bteta_0)$ where
\[
\Jc(\bb,\ab)=\int_{0}^1 \Jc(t \bb+(1-t)\ab)dt.
\]
We can write the predictions due to $\bteta_{\tau+1}$ as
\begin{align*}
f(\bteta_{\tau+1})&=f(\bteta_{\tau}-\eta\grad{\bteta_\tau})=f(\bteta_{\tau})+\eta \Jc(\bteta_{\tau+1},\bteta_\tau) \grad{\bteta_\tau}\\
&=f(\bteta_{\tau})+\eta \Jc(\bteta_{\tau+1},\bteta_\tau)\Jc^T(\bteta_\tau)(f(\bteta_{\tau})-\y).
\end{align*}
This implies that
\[
\rb_{\tau+1}=f(\bteta_{\tau+1})-\y=(\Iden-\eta\B_1\B_2^T)\rb_\tau.
\]
Similarly, for linearized problem we have $\rbb_{\tau+1}=(\Iden-\eta\Jb\Jb^T)\rbb_\tau$. Thus,%
\begin{align}
\label{tkey2}
\tn{\eb_{\tau+1}}&=\twonorm{(\Iden-\eta\B_1\B_2^T)\rb_\tau-(\Iden-\eta\Jb\Jb^T)\rbb_\tau}\nn\\
&=\twonorm{(\Iden-\eta\B_1\B_2^T)\eb_\tau-\eta(\B_1\B_2^T-\Jb\Jb^T)\rbb_\tau}\nn\\
&\leq \tn{(\Iden-\eta\B_1\B_2^T)\eb_\tau}+\eta\tn{(\B_1\B_2^T-\Jb\Jb^T)\rbb_\tau}\nn\\
&\leq \tn{(\Iden-\eta\B_1\B_2^T)\eb_\tau}+\eta\opnorm{(\B_1\B_2^T-\Jb\Jb^T)}\tn{\rbb_\tau}.
\end{align}
%Under Assumptions \ref{ass2} and \ref{ass3}, we write
We proceed by bounding each of these two terms. For the first term, we apply Lemma \ref{asym pert} with $\A=\B_1$ and $\B=\B_2$ and use $\|\B_1-\B_2\|\leq \eps$ to conclude that
\begin{align}
\label{fstkey2}
\tn{(\Iden-\eta\B_1\B_2^T)\eb_\tau}\leq (1+\eta\eps^2)\tn{\eb_\tau}.
\end{align}
Next we turn our attention to bounding the second term. To this aim note that
\begin{align}
\label{sstkey2}
\|\B_1\B_2^T-\Jb\Jb^T\|&=\|\B_1\B_2^T-\A\A^T+\A\A^T-\Jb\Jb^T\|\nn\\
&\leq \|\B_1\B_2^T-\A\A^T\|+\|\A\A^T-\Jb\Jb^T\|\nn\\
&\leq \|(\B_1-\A)\B_2^T\|+\|\A(\B_2-\A)^T\|+\|\A\A^T-\Jb\Jb^T\|\nn\\
&\le \|\B_1-\A\|\|\B_2\|+\|\B_2-\A\|\|\A\|+\|\A\A^T-\Jb\Jb^T\|\nn\\
&\leq \beta\frac{\eps}{2}+\beta\frac{\eps}{2}+ \eps_0^2\nn\\
&=\eps_0^2+\eps\beta.
\end{align}
In the last inequality we use the fact that per Assumption \ref{ass3} we have $\|\B_1-\A\|\le \eps/2$ and $\|\B_2-\A\|\le \eps/2$ as well as the fact that per Definition \ref{tjac} $\|\A\A^T-\Jb\Jb^T\|\le \eps_0^2$. Plugging \eqref{fstkey2} and \eqref{sstkey2} in \eqref{tkey2} completes the proof.
%$\eb^T\B\A^T\eb\geq (2\bn-\eps)2\bn\geq \bn^2$. We can write
%\[
%\tn{(\Iden-\eta\B\A^T)\eb}^2=\tn{\eb}^2-\eta \eb^T\B\A^T\eb+\eta^2\tn{\B\A^T\eb}^2
%\]
\end{proof}
Next we prove a result about the growth of sequences obeying certain assumptions. As we will see later on in the proofs this lemma allows us to control the growth of the perturbation between the original and linearized residuals ($e_\tau=\twonorm{\eb_\tau}$).  
\begin{lemma}[Bounding residual perturbation growth for general nonlinearities] \label{lem growth} Consider positive scalars $\Gamma,\alpha,\eps,\eta>0$. Also assume $\eta\leq 1/\alpha^2$ and $\alpha\ge \sqrt{2\Gamma}\eps$ and set $T=\frac{\Gamma}{\eta\alpha^2}$. Assume the scalar sequences $e_\tau$ (with $e_0=0$) and $\widetilde{r}_\tau$ obey the following identities 
\begin{align}
{\widetilde{r}}_{\tau}\le& (1-\eta\alpha^2)^\tau \rho_++\rho_-,\nn\\
e_{\tau}\le& (1+\eta\eps^2)e_{\tau-1}+ \eta \Theta{\widetilde{r}}_{\tau-1},\label{lem78ass}
\end{align}
for all $0\le \tau\le T$ and non-negative values $\rho_-,\rho_+\ge 0$. Then, for all $0\leq \tau\leq T$, 
\begin{align}
e_{\tau}\leq \Theta \Lambda\quad\text{holds with}\quad\Lambda=\frac{2(\Gamma\rho_-+\rho_+)}{\alpha^2}.\label{e control}
\end{align}
\end{lemma}
\begin{proof} We shall prove the result inductively. Suppose \eqref{e control} holds for all $t\leq \tau-1$. Consequently, we have
\begin{align*}
e_{t+1}\le&(1+\eta\eps^2)e_t+ \eta\Theta {\widetilde{r}}_t\\
\le&e_t+\eta\eps^2e_t+\eta\Theta\left((1-\eta\alpha^2)^t \rho_++\rho_-\right)\\
\le&e_t+\eta \Theta\left(\eps^2 \Lambda+(1-\eta\alpha^2)^{t} \rho_++\rho_-\right).
\end{align*}
Thus
\begin{align}
\frac{e_{t+1}-e_{t}}{\Theta}\le \eta \left(\eps^2 \Lambda+(1-\eta\alpha^2)^{t} \rho_++\rho_-\right).\label{diff eq}
\end{align}
Summing up both sides of \eqref{diff eq} for $0\leq t\leq \tau-1$ we conclude that
\begin{align*}
\frac{e_{\tau}}{\Theta}&=\sum_{t=0}^{\tau-1} \frac{e_{t+1}-e_t}{\Theta}\\
&\leq \eta\tau\left(\eps^2\Lambda+\rho_-\right)+\eta\rho_+\sum_{t=0}^{\tau-1}(1-\eta\alpha^2)^{t} \\
&= \eta\tau\left(\eps^2\Lambda+\rho_-\right)+\eta\rho_+\frac{1-\left(1-\eta\alpha^2\right)^\tau}{\eta\alpha^2} \\
&\le \eta\left( \tau\eps^2 \Lambda+\frac{\rho_+}{\eta\alpha^2} +\tau\rho_-\right)\\
&= \eta\tau(\eps^2 \Lambda+\rho_-)+\frac{\rho_+}{\alpha^2}\\
&\leq \eta T(\eps^2 \Lambda+\rho_-)+\frac{\rho_+}{\alpha^2}\\
%&=\frac{\Gamma}{\alpha^2}(\eps^2 \Lambda+\rho_-)+\frac{\rho_+}{\alpha^2}\\
&=\frac{\Gamma\eps^2\Lambda +\Gamma\rho_-+\rho_+}{\alpha^2}\\
&=\frac{\Gamma\eps^2\Lambda}{\alpha^2}+\frac{\Lambda}{2}\\
&\leq \Lambda,
\end{align*}
where in the last inequality we used the fact that $\alpha^2\geq 2\Gamma\eps^2$. This completes the proof of the induction step and the proof of the lemma.
%We know that $\Lambda$ needs to upper bound this, hence
%\[
%\Lambda = \frac{2(\Gamma\rho_-+\rho_+)}{\alpha}\geq  \frac{\Gamma\rho_-+\rho_+}{\alpha-{\Gamma\eps}}\implies \Lambda(1-\frac{\Gamma\eps}{\alpha})\geq \frac{\Gamma\rho_-+\rho_+}{\alpha}\iff \Lambda\geq \frac{\Gamma\eps\Lambda +\Gamma\rho_-+\rho_+}{\alpha}.
%\]
%Hence, induction holds.
\end{proof}


\subsubsection{Completing the proof of Theorem \ref{many step thm}}
\label{comp5}%\eqref{eqqq2}
With the key lemmas in place in this section we wish to complete the proof of Theorem \ref{many step thm}.
We will use induction to prove the result. Suppose the statement is true for some $\tau-1\leq T-1$. In particular, we assume the identities \eqref{main res eq1} and \eqref{main res eq2} hold for all $0\leq t\leq\tau-1$. We aim to prove these identities continue to hold for iteration $\tau$. We will prove this result in multiple steps.

%\begin{itemize}
%\item \eqref{main res eq1} holds for $. %For all $0\leq t\leq\tau$, $\tn{\bteta_{t}-\bteta_0}\leq R$.
%\item \eqref{main res eq2} holds.
%\end{itemize} 

\noindent{\bf{Step I: Next iterate obeys $\twonorm{\bteta_\tau-\bteta_0}\le R$.}}\\ 
We first argue that $\bteta_{\tau}$ lies in the domain of interest as dictated by \eqref{assumpgen}, i.e.~$\tn{\bteta_\tau-\bteta_0}\leq R$. To do this note that per the induction assumption \eqref{main res eq2} holds for iteration $\tau-1$ and thus $\tn{\bteta_{\tau-1}-\bteta_0}\leq R/2$. As a result using the triangular inequality to show $\twonorm{\bteta_\tau-\bteta_0}\le R$ holds it suffices to show that $\tn{\bteta_{\tau}-\bteta_{\tau-1}}\leq R/2$ holds. To do this note that
\begin{align}
\tn{\bteta_\tau-\bteta_{\tau-1}}=&\eta\tn{ \grad{\bteta_{\tau-1}}}\nn\\
=&\eta\twonorm{\Jc^T(\bteta_{\tau-1})\rb_{\tau-1}}\nn\\
=&\eta\twonorm{\Jcb^T(\bteta_{\tau-1})\rb_{\tau-1}}\nn\\
\overset{(a)}{\le}& \eta \tn{\Jc^T(\bteta_{\tau-1})\rbb_{\tau-1}}+\eta \tn{\Jc^T(\bteta_{\tau-1})(\rb_{\tau-1}-\rbb_{\tau-1})}\nn\\
\overset{(b)}{\le}& \eta \twonorm{\Jb^T\rbb_{\tau-1}}+\eta \opnorm{\Jc(\bteta_{\tau-1})-\Jb}\twonorm{\rbb_{\tau-1}}+\eta \opnorm{\Jc(\bteta_{\tau-1})}\twonorm{\rb_{\tau-1}-\rbb_{\tau-1}}\nn\\
\overset{(c)}{\le}& \eta \twonorm{\Jb\rbb_{\tau-1}}+\frac{\eps_0+\eps}{\beta^2}\twonorm{\rbb_{\tau-1}}+\frac{1}{\beta}\tn{\rb_{\tau-1}-\rbb_{\tau-1}}\nn\\
\overset{(d)}{\le}& \eta \tn{\Jb^T\rbb_{\tau-1}}+\frac{2\delta\alpha}{5\beta^2}\tn{{\rb}_0}+\frac{1}{\beta}\twonorm{\rb_{\tau-1}-\rbb_{\tau-1}}\nn\\
\overset{(e)}{\le}& \eta \tn{\Jb^T\rbb_{\tau-1}}+\frac{2\delta\alpha}{5\beta^2}\tn{{\rb}_0}+\frac{3\delta\alpha}{5\beta^2}\tn{\rb_0}\nn\\
\overset{(f)}{\le}& \eta \left(\twonorm{\Jb^T\Pi_{\Rc}(\rbb_{\tau-1})}+\twonorm{\Jb^T\Pi_{\Rcb}(\rbb_{\tau-1})}\right)+\frac{\delta\alpha}{\beta^2}\twonorm{{\rb}_0}\nn\\
\overset{(g)}{\le}& \frac{1}{\beta}\twonorm{\Pi_{\Rc}(\rbb_{\tau-1})}+\frac{\alpha}{\beta^2}\tn{\Pi_{\Rcb}(\rbb_{\tau-1})}+\frac{\delta\alpha}{\beta^2}\twonorm{{\rb}_0}\nn\\
\overset{(h)}{\le}& \frac{1}{\beta}\twonorm{\Pi_{\Rc}({\rb}_0)}+\frac{\alpha}{\beta^2}\twonorm{\Pi_{\Rcb}({\rb}_0)}+\frac{\delta\alpha}{\beta^2}\twonorm{{\rb}_0}\nn\\
\leq& \twonorm{\mtx{J}_{\calF}^{\dagger}\vct{r}_0}+\frac{1}{\alpha}\tn{\Pi_{\Rcb}({\rb}_0)}+\frac{\delta\alpha}{\beta^2}\twonorm{{\rb}_0}\nn\\
\leq&\frac{R}{2}.\nn
\end{align}
%%\le& \eta \|\Jc(\bteta_{\tau-1})\|\tn{\rb_{\tau-1}}\nn\\
%\overset{(a)}{\le}&\frac{\tn{\rb_{\tau-1}}}{\beta}\nn\\
%\le&\frac{\tn{\rbb_{\tau-1}}+\tn{\rbb_{\tau-1}-\rb_{\tau-1}}}{\beta}\nn\\
%\overset{(b)}{\le}&\frac{\tn{\rbb_{\tau-1}}}{\beta}+\frac{\delta\alpha}{\beta^2}\twonorm{\rb_0}\nn\\
%\overset{(c)}{\le}&\frac{\tn{\rb_{0}}}{\beta}+\frac{\delta\alpha}{\beta^2}\twonorm{\rb_0}\nn\\
%\overset{(d)}{\le}&\frac{\tn{\rb_{0}}}{\beta}+\frac{\delta\Gamma}{\alpha}\twonorm{\rb_0}\nn\\
%\overset{(e)}{\le}&\frac{\upp+\delta\Gamma\tn{\rb_0}}{\alpha}\nn\\
%\overset{(f)}{\le}&\frac{R}{2}.
%\\&= \eta (\Jc(\bteta_{\tau-1}-\Jb)\rb_{\tau-1}+\Jb\eb_{\tau-1}+\Jb\rbb_{\tau-1})
Here, (a) and (b) follow from a simple application of the triangular inequality, (c) from the fact that $\opnorm{\Jc(\bteta_{\tau-1})-\mtx{J}}\le\opnorm{\Jc(\bteta_{\tau-1})-\Jc(\bteta_0)}+\opnorm{\Jc(\bteta_0)-\mtx{J}}\le \eps+\eps_0$, (d) from combining the bounds in \eqref{cndd}, (e) from the induction hypothesis that postulates \eqref{main res eq1} holds for iteration $\tau-1$, (f) from the triangular inequality, (g) from the fact that $\opnorm{\mtx{J}}\le \beta$ and $\opnorm{\mtx{J}^T\vct{z}}\le \alpha\twonorm{\vct{z}}$ for all $\vct{z}\in\mathcal{N}$, (h) from the fact that $\rbb_{\tau-1}=\left(\mtx{I}-\eta\Jb\Jb^T\right)^{\tau-1}\rb_0$ which implies that $\Pi_{\mathcal{I}}(\rbb_{\tau-1})=\left(\mtx{I}-\eta\Jb\Jb^T\right)^{\tau-1}\Pi_{\mathcal{I}}(\rb_0)$ and $\Pi_{\mathcal{N}}(\rbb_{\tau-1})=\left(\mtx{I}-\eta\Jb\Jb^T\right)^{\tau-1}\Pi_{\mathcal{N}}(\rb_0)$ and $\opnorm{\left(\mtx{I}-\eta\Jb\Jb^T\right)}\le 1$ for $\eta\le 1/\beta^2$ which implies that $\twonorm{\Pi_{\mathcal{I}}(\rbb_{\tau-1})}\le \twonorm{\Pi_{\mathcal{I}}(\rb_0)}$ and $\twonorm{\Pi_{\mathcal{N}}(\rbb_{\tau-1})}\le \twonorm{\Pi_{\mathcal{N}}(\rb_0)}$ 


(d) from the fact that $\alpha\le \beta$, (e) from the fact that $\tn{\rb_0}\le \frac{\beta}{\alpha}\upp$, and (f) from the fact that
\begin{align*}
\frac{\upp}{\alpha}=&\left(\sum_{s=1}^r  \frac{1}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2+\Gamma^2\sum_{s=r+1}^{nK}\frac{\la_s^2}{\alpha^4} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}\\
\le&\left(\sum_{s=1}^r  \frac{1}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}+\left(\Gamma^2\sum_{s=r+1}^{nK}\frac{\la_s^2}{\alpha^4} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}\\
\le&\left(\sum_{s=1}^r  \frac{1}{\la_s^2}\left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}+\frac{\Gamma}{\alpha}\left(\sum_{s=r+1}^{nK} \left(\langle\vct{u}_s,\vct{r}_0\rangle\right)^2\right)^{1/2}\\
=&\twonorm{\mtx{J}_{\mathcal{I}}^\dagger\rb_0}+\frac{\Gamma}{\alpha}\twonorm{\Pi_{\mathcal{N}}(\rb_0)}.
\end{align*}

\noindent{\bf{Step II: Original and linearized residuals are close (first part of \eqref{main res eq1}).}}\\
In this step we wish to show that the first part of \eqref{main res eq1} holds for iteration $\tau$. Since we established in the previous step that $\tn{\bteta_{\tau}-\bteta_0}\leq R$ the assumption of Lemma \ref{grwth} holds for iterations $\tau-1$ and $\tau$. Hence, using Lemma \ref{grwth} equation \eqref{etau repeat} we conclude that
\begin{align*}
\tn{\eb_{\tau}}&\leq \eta(\eps_0^2+\eps\beta)\tn{\rbb_{\tau-1}}+(1+\eta\eps^2)\tn{\eb_{\tau}}.
\end{align*}
This combined with the induction assumption implies that
\begin{align}
\label{pf53t1}
\tn{\eb_{t}}&\leq \eta(\eps_0^2+\eps\beta)\tn{\rbb_{t-1}}+(1+\eta\eps^2)\tn{\eb_{t}},
\end{align}
holds for all $t\le \tau\le T$. Furthermore, using Lemma \ref{lem linear} equation \eqref{cor76conc1} for all $t\le \tau\le T$ we have
\begin{align}
\label{pf53t2}
\twonorm{\rbb_t}\le \left(1-\eta\alpha^2\right)^t\tn{\Pi_{\Rc}(\rb_0)}+\tn{\Pi_{\Rcb}(\rb_0)},
\end{align}
To proceed, we shall apply Lemma \ref{lem growth} with the following variable substitutions
\begin{align}
\Theta:=\eps_0^2+\eps\beta,\quad\rho_+=\tn{\Pi_{\Rc}(\rb_0)},\quad\rho_-=\tn{\Pi_{\Rcb}(\rb_0)},\quad e_\tau:=\tn{\eb_\tau},\quad {\widetilde{r}}_\tau:= \tn{\rbb_\tau}.
\end{align}
%Set $\Gamma=\log(1/\delta)$. Note that $\alpha/\eps=\frac{1}{\delta}\beta^2/\alpha^2>\tau_0$. 
%\noindent {\bf{Showing small error:}
We note that Lemma \ref{lem growth} is applicable since (i) $\eta\le 1/\beta^2\le 1/\alpha^2$, (ii) based on \eqref{cndd} we have $\frac{\alpha}{\eps}\ge \frac{5\Gamma}{\delta}\frac{\beta^2}{\alpha^2}\ge \sqrt{2\Gamma}$, (iii) $\tau$ obeys $\tau\leq T= \frac{\Gamma}{\eta\bn^2}$, and (iv) \eqref{lem78ass} holds based on \eqref{pf53t1} and \eqref{pf53t2}. Thus using Lemma \ref{lem growth} we can conclude that
\begin{align}
\tn{\eb_{\tau}}\le& 2(\eps_0^2+\eps\beta)\frac{\left(\tn{\Pi_{\Rc}(\rb_0)}+\Gamma\tn{\Pi_{\Rcb}(\rb_0)}\right)}{\bn^2}\nn\\
\le&\frac{2\Gamma(\eps_0^2+\eps\beta)\tn{\rb_0}}{\alpha^2}\label{etau termm}\\
\le&( \frac{2}{25}+\frac{2}{5})\frac{\delta\alpha}{\beta} \tn{\rb_0}\leq\frac{3}{5} \frac{\delta\alpha}{\beta} \tn{\rb_0},\label{etau term}
\end{align}
where in the last inequality we used \eqref{cndd}. This completes the first part of \eqref{main res eq1} via induction.

%If $\tau\geq \frac{\Gamma}{\eta\bn^2}$, we also have that
%\[
%\tn{\Pi_{\Rc}(\rbb_\tau)}^2=\sum_{i=1}^r ((1-\eta \la_i^2)^{\tau} a_i)^2\leq r(1-\eta \bn^2)^{\tau}a_i^2\leq \exp(-\Gamma)\tn{\rb_0}^2\leq \delta^2\tn{\Pi_{\Rc}(\rb_0)}^2.
%\]
%Adding these two, and using $\tn{\rb_\tau}\leq \tn{\rbb_\tau-\rb_\tau}+\tn{\rbb_\tau}$, we find
%\begin{align}
%\tn{\rb_\tau}&\leq \exp(-\Gamma)\tn{\Pi_{\Rc}(\rb_0)}+\tn{\Pi_{\bar{\Rc}}(\rb_0)}+\eps\beta\frac{2(\Gamma \tn{\Pi_{\bar{\Rc}}(\rb_0)}+\tn{\Pi_{\Rc}(\rb_0)})}{\bn^2}\\
%&\leq \tn{\Pi_{\bar{\Rc}}(\rb_0)}+\delta\tn{\rb_0}.
%\end{align}
\noindent{\bf{Step III: Original and linearized parameters are close (second part of \eqref{main res eq1}).}}\\
 In this step we wish to show that the second part of \eqref{main res eq1} holds for iteration $\tau$. To do this we begin by noting that by the fact that $\Jb$ is a reference Jacobian we have $\|\Jcb(\bteta_0)-\Jb\|\leq \eps_0$ where $\Jcb$ augments $\Jc(\bteta_0)$ by padding zero columns to match size of $\Jb$. Also by Assumption \ref{ass3} we have $\|\Jc(\bteta)-\Jc(\bteta_0)\|\leq \frac{\eps}{2}$. Combining the latter two via the  triangular inequality we conclude that
\begin{align}
\label{53temp3}
\|\Jcb(\bteta_\tau)-\Jb\|\leq \eps_0+\eps.
\end{align}
Let $\brteta$ and $\nabla \bar{\Lc}(\bteta)$ be vectors augmented by zero padding $\bteta,\grad{\bteta}$ so that they have dimension $\max(\K n, p)$. Now, we track the difference between $\brteta$ and linearized $\tilde{\bteta}$ as follows
\begin{align}
\frac{\tn{\brteta_{\tau}-\widetilde{\bteta}_{\tau}}}{\eta}&=\twonorm{\sum_{t=0}^{\tau-1}\nabla\bar{\Lc}(\bteta_t)-\nabla\mathcal{L}_{lin}(\bbteta_t)}\nn\\
&=\twonorm{\sum_{t=0}^{\tau-1}\Jcb(\bteta_t)^T\rb_t- \Jb^T\rbb_t}\nn\\
&\leq \sum_{t=0}^{\tau-1} \tn{\Jcb(\bteta_t)^T\rb_t- \Jb^T\rbb_t}\nn\\
&\leq \sum_{t=0}^{\tau-1} \tn{(\Jcb(\bteta_t)-\Jb)^T\rbb_t}+\tn{\Jcb(\bteta_t)^T(\rb_t-\rbb_t)}\nn\\
&= \sum_{t=0}^{\tau-1} \tn{(\Jcb(\bteta_t)-\Jb)^T\rbb_t}+\tn{\Jcb(\bteta_t)^T\eb_t}\nn\\
&\leq  \sum_{t=0}^{\tau-1}(\eps+\eps_0)\tn{\rbb_t}+\beta\tn{\eb_t}.\label{combined eq}
\end{align}
In the last inequality we used the fact that $\|\Jcb(\bteta_t)-\Jb\|\leq \eps+\eps_0$ and $\|\Jb\|\leq \beta$. We proceed by bounding each of the two terms in \eqref{combined eq} above. For the first term we use the fact that $\tn{\rbb_\tau}\leq \tn{\rb_0}$ to conclude
\begin{align}
\sum_{t=0}^{\tau-1} \tn{\rbb_t}\leq\tau \tn{\rb_0}\leq T \tn{\rb_0}= \frac{\Gamma\tn{\rb_0}}{\eta\alpha^2}.\label{rrr bound}%(1-\bn^2\eta/4)^\tau \tn{\rb_0}\leq \frac{4}{\eta\bn^2}\tn{\rb_0}.
\end{align}
%\begin{align}
%\sum_{t=0}^{\tau-1} \tn{\rbb_t}\leq \frac{1}{\eta\alpha^2}\tn{\Pi_{\Rc}(\rb_0)}+\tau\tn{\Pi_{\Rcb}(\rb_0)}\leq \frac{1}{\eta\alpha^2}\tn{\Pi_{\Rc}(\rb_0)}+\tau\tn{\Pi_{\Rcb}(\rb_0)}\leq  \frac{\tn{\Pi_{\Rc}(\rb_0)}+\Gamma\tn{\Pi_{\Rcb}(\rb_0)}}{\eta\alpha^2}.\label{rrr bound}%(1-\bn^2\eta/4)^\tau \tn{\rb_0}\leq \frac{4}{\eta\bn^2}\tn{\rb_0}.
%\end{align}
To bound the second term in \eqref{combined eq} we use \eqref{etau termm} together with $\tau\le T\le \frac{\Gamma}{\eta\alpha^2}$ to conclude that
\begin{align}
\sum_{t=0}^{\tau-1} \tn{\eb_t}\leq \tau  \frac{2(\eps\beta+\eps_0^2)}{\alpha^2} \Gamma\tn{\rb_0}\leq   \frac{2\Gamma^2(\eps\beta+\eps_0^2)}{\eta \alpha^4} \tn{\rb_0}.\label{eee bound}%4\tau\eps\beta\Gamma\frac{\tn{\rb_0}}{\bn^2}.
\end{align}
Combining \eqref{rrr bound} and \eqref{eee bound} in \eqref{combined eq}, we conclude that
%\[
%\tn{\bteta_{\tau}-\brteta_{\tau}}\leq 4\eta\eps \beta^2\alpha^{-2}\Gamma\tau\tn{\rb_0}
%\]
\begin{align*}
\tn{\brteta_{\tau}-\widetilde{\bteta}_{\tau}}\le& \left(  \frac{2\Gamma(\eps\beta^2+\eps_0^2\beta)}{\alpha^3}+\frac{\eps+\eps_0}{\alpha}\right) \frac{\Gamma}{\alpha}\tn{\rb_0}\\
=&\left(\epsilon\frac{2\Gamma\beta^2}{\alpha^3}+\eps_0^2\frac{2\Gamma\beta}{\alpha^3}+\frac{\eps+\eps_0}{\alpha}\right)\frac{\Gamma}{\alpha}\tn{\rb_0}\\
\overset{(a)}{\le}&\left(\frac{\delta}{5}+\eps_0^2\frac{2\Gamma\beta}{\alpha^3}+\frac{\eps+\eps_0}{\alpha}\right)\frac{\Gamma}{\alpha}\tn{\rb_0}\\
\overset{(b)}{\le}&\left(\frac{1}{5}\delta+\frac{2}{25}\delta+\frac{\eps+\eps_0}{\alpha}\right)\frac{\Gamma}{\alpha}\tn{\rb_0}\\
\overset{(c)}{\le}&\left(\frac{1}{5}\delta+\frac{2}{25}\delta+\frac{1}{5}\delta+\frac{\eps_0}{\alpha}\right)\frac{\Gamma}{\alpha}\tn{\rb_0}\\
\overset{(d)}{\le}&\left(\frac{1}{5}\delta+\frac{2}{25}\delta+\frac{1}{5}\delta+\frac{1}{5}\delta\right)\frac{\Gamma}{\alpha}\tn{\rb_0}\\
=&\frac{17}{25}\frac{\delta}{\alpha}\Gamma\tn{\rb_0}.
\end{align*}
Here, (a) follows from $\eps\leq \frac{\delta\alpha^3}{5\Gamma\beta^2}$ per Assumption \eqref{cndd}, (b) from $\eps_0\le \frac{1}{5}\sqrt{\frac{\delta\alpha^3}{\Gamma\beta}}$ per Assumption \eqref{cndd}, (c) from $\eps\leq \frac{\delta\alpha^3}{5\Gamma\beta^2}\le \frac{\delta\alpha}{5\Gamma}\le \frac{\delta\alpha}{5}$ per Assumption \eqref{cndd}, and (d) from $\eps_0\le \frac{\delta\alpha}{5}$ per Assumption \eqref{cndd}. Thus,
\begin{align*}
\tn{\brteta_{\tau}-\widetilde{\bteta}_{\tau}}\le\frac{\delta}{\alpha}\Gamma\tn{\rb_0}.
\end{align*}
Combining the latter with the fact that $\tn{\bbteta_\tau-\brteta_0}\leq \frac{\upp}{\alpha}$ based on Corollary \ref{cor simp} we conclude that
\begin{align*}
\twonorm{\bteta_\tau-\bteta_0}=\twonorm{\brteta_\tau-\brteta_0}\le \twonorm{\bbteta_\tau-\brteta_0}+\twonorm{\brteta_\tau-\bbteta_\tau}\le \frac{\upp}{\alpha}+\frac{\delta}{\alpha}\Gamma\tn{\rb_0}\le \twonorm{\mtx{J}_{\calF}^{\dagger}\vct{r}_0}+\frac{\Gamma}{\alpha}\twonorm{\Pi_{\calS}\left(\vct{r}_0\right)}+\frac{\delta}{\alpha}\Gamma\tn{\rb_0}
\end{align*}
The completes the proof of the bound \eqref{main res eq2}. 
  
\noindent\textbf{Step V: Bound on residual with early stopping.}\\
In this step we wish to prove \eqref{eqqq2}. To this aim note that
\begin{align*}
\twonorm{\rb_T}\overset{(a)}{\le}& \twonorm{\rbb_T}+\twonorm{\rbb_T-\rb_T}\\
\overset{(b)}{\le}&\twonorm{\rbb_T}+\frac{\delta\alpha}{\beta}\tn{\rb_0}\\
\overset{(b)}{\le}&e^{-\Gamma}\tn{\Pi_{\Rc}(\rb_0)}+\tn{\Pi_{\Rcb}(\rb_0)}+\frac{\delta\alpha}{\beta}\tn{\rb_0}
\end{align*}
where (a) follows from the triangular inequality, (b) from the conclusion of Step II (first part of \eqref{main res eq1}), and (c) from Corollary \ref{cor simp} equation \eqref{cor76conc2}. This completes the proof of \eqref{eqqq2}.

\subsection{Key lemmas and identities for neural networks}
In this section we prove some key lemmas and identities regarding the Jacobian of one-hidden layer networks as well as the size of the initial residual that when combined with Theorem \ref{many step thm} allows us to prove theorems involving neural networks. We begin with some preliminary identities and calculations in Section \ref{prelimiden}. Next, in Section \ref{fundet} we prove a few key properties of the Jacobian mapping of a one-hidden layer neural network. Section \ref{Jacrandinit} focuses on a few further properties of the Jacobian at a random initialization. Finally, in Section \ref{initmisfit} we provide bounds on the initial misfit.

For two matrices
\begin{align*}
\mtx{A}=\begin{bmatrix}\mtx{A}_1\\\mtx{A}_2\\\vdots\\\mtx{A}_p\end{bmatrix}\in\R^{p\times m}\quad\text{and}\quad \mtx{B}=\begin{bmatrix}\mtx{B}_1\\\mtx{B}_2\\\vdots\\\mtx{B}_p\end{bmatrix}\in\R^{p\times n},
\end{align*}
we define their Khatri-Rao product as $\mtx{A} * \mtx{B}  = [\mtx{A}_1\otimes \mtx{B}_1,\dotsc, \mtx{A}_p\otimes \mtx{B}_p]\in\R^{p\times mn}$, where $\otimes$ denotes the Kronecher product.
\subsubsection{Preliminary identities and calculations}
\label{prelimiden}
We begin by discussing a few notations. Throughout we use $\w_\ell$ and $\vb_\ell$ to denote the $\ell$th row of input and output weight matrices $\W$ and $\Vb$. Given a matrix $\M$ we use $\trow{\M}$ to denote the largest Euclidean norm of the rows of $\M$. We begin by noting that for a one-hidden layer neural network of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$, the Jacobian matrix with respect to vect$(\mtx{W})\in\R^{kd}$ takes the form
\begin{align}
\mathcal{J}(\mtx{W})=
\begin{bmatrix}
\mathcal{J}_1(\W) \\ \vdots \\ \mathcal{J}_\K(\W)
\end{bmatrix}\in\R^{\K n\times kd}\label{jacob multi}
\end{align}
where $\Jc_\ell(\W)$ is the Jacobian matrix associated with the $\ell$th class. In particular, $\Jc_\ell(\W)$ is given by
\begin{align*}
\mathcal{J}_\ell(\mtx{W})=
\begin{bmatrix}
\mathcal{J}_\ell(\vct{w}_1) & \ldots & \mathcal{J}_\ell(\vct{w}_k)
\end{bmatrix}\in\R^{n\times kd}\quad\text{with}\quad\mathcal{J}_\ell(\vct{w}_s):=\mtx{V}_{\ell,s}\text{diag}(\phi'(\mtx{X}\vct{w}_s)\mtx{X}.
\end{align*}
Alternatively using Khatri-Rao products this can be rewritten in the more compact form
\begin{align}
\label{KR}
\mathcal{J}_\ell(\mtx{W})=\left(\text{diag}(\vct{v}_\ell)\phi'\left(\mtx{X}\mtx{W}^T\right)\right)*\mtx{X}.
\end{align}
An alternative characterization of the Jacobian is via its matrix representation. Given a vector $\ub\in\R^{\K n}$ let us partition it into $\K$ size $n$ subvectors so that $\ub=[\ub_1^T~\dots~\ub_\K^T]^T$. We have
\begin{align}
\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)= \sum_{\ell=1}^\K\text{diag}(\vct{v}_\ell)\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u}_\ell)\mtx{X}.\label{mat form}
\end{align}

\subsubsection{Fundamental properties of the Jacobian of the neural network}
\label{fundet}
In this section we prove a few key properties of the Jacobian mapping of a one-hidden layer neural network.
% as depicted in Figure \ref{neuralnet}

%\subsection{Properties of Neural Net Jacobian}
%\begin{lemma}[Spectral norm of the Jacobian]\label{spectJ} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \vct{v}^T\phi\left(\W\x\right)$ where the activation $\phi$ has bounded derivatives obeying $\abs{\phi'(z)}\le B$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Then the Jacobian matrix with respect to the input-to-hidden weights obeys 
%\begin{align*}
%\opnorm{\mathcal{J}(\mtx{W})}\le \sqrt{k}B\infnorm{\vct{v}}\opnorm{\X}.
%\end{align*}
%\end{lemma}
%\begin{lemma}[Jacobian Lipschitzness]\label{JLlem} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \vct{v}^T\phi\left(\W\x\right)$ where the activation $\phi$ has bounded second order derivatives obeying $\abs{\phi''(z)}\le M$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Then the Jacobian mapping with respect to the input-to-hidden weights obeys
%\begin{align*}
%\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le M\infnorm{\vct{v}}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}\quad\text{for all}\quad \widetilde{\W},\W\in\R^{k\times d}.
%\end{align*}
%\end{lemma}
\begin{lemma}[Properties of Single Output Neural Net Jacobian]\label{props thm} Let $\K=1$ so that $\Vb^T=\vb\in\R^n$. Suppose $\phi$ is an activation obeying $|\phi'(z)|\leq B$ for all $z$. Then, for any $\W\in\R^{k\times d}$ and any unit length vector $\ub$, we have
\begin{align*}
\|\Jc(\W)\|\le& B\sqrt{k}\infnorm{\vct{v}}\opnorm{\X}
\end{align*}
and
\begin{align}
\label{rowwisebnd}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}\le& B\tin{\vb}\|\X\|
\end{align}
Furthermore, suppose $\phi$ is twice differentiable and $|\phi''(z)|\leq B$ for all $z$. Also assume all data points have unit Euclidean norm ($\twonorm{\vct{x}_i}=1$). Then the Jacobian mapping is Lipschitz with respect to spectral norm i.e.~{for all} $\widetilde{\W},\W\in\R^{k\times d}$ we have
\begin{align*}
\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le B\infnorm{\vct{v}}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}.
\end{align*}
\end{lemma}
\begin{proof} The result on spectral norm and Lipschitzness of $\Jc(\W)$ have been proven in \cite{onehidden}. To show the row-wise bound \eqref{rowwisebnd}, we use \eqref{mat form} to conclude that
\begin{align*}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}&= \trow{\text{diag}(\vct{v})\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u})\mtx{X}}\\
&= \tin{\vb}\max_{1\leq \ell\leq k}\tn{\phi'\left(\w_\ell^T\mtx{X}^T\right)\text{diag}(\vct{u})\mtx{X}}\\
&\leq \tin{\vb}\|\X\|\max_{1\leq \ell\leq k}\tn{\phi'\left(\w_\ell^T\mtx{X}^T\right)\text{diag}(\vct{u})}\\
&\leq B\tin{\vb}\|\X\|\tn{\ub}\\
&=B\tin{\vb}\|\X\|.
\end{align*}
\end{proof}
Next we extend the lemma above to the multi-class setting.
\begin{lemma}[Properties of Multiclass Neural Net Jacobian]\label{props lem} Suppose $\phi$ is an activation obeying $|\phi'(z)|\le B$ for all $z$. Then, for any $\W\in\R^{k\times d}$ and any unit length vector $\ub$, we have
\[
\|\Jc(\W)\|\leq B\sqrt{\K k}\infnorm{\Vb}\opnorm{\X}
\]
and
\begin{align}
\label{rowbndm}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}\leq B\sqrt{\K}\tin{\Vb}\|\X\|.
\end{align}
Furthermore, suppose $\phi$ is twice differentiable and $|\phi''(z)|\leq B$ for all $z$. Also assume all data points have unit Euclidean norm ($\twonorm{\vct{x}_i}=1$). Then the Jacobian mapping is Lipschitz with respect to spectral norm i.e.~{for all} $\widetilde{\W},\W\in\R^{k\times d}$ we have
\begin{align*}
\opnorm{\mathcal{J}(\widetilde{\mtx{W}})-\mathcal{J}(\mtx{W})}\le B\sqrt{\K}\infnorm{\Vb}\opnorm{\mtx{X}}\fronorm{\widetilde{\mtx{W}}-\mtx{W}}.
\end{align*}
\end{lemma}
\begin{proof} The proof will follow from Lemma \ref{props thm}. First, given $\A=[\A_1^T~\dots~\A_\K^T]^T$ and $\B=[\B_1^T~\dots~\B_\K^T]^T$, observe that
\[
\|\A\|\leq \sqrt{\K} \sup_{1\leq \ell\leq \K}\|\A_\ell\|\quad\text{and}\quad\|\A-\B\|\leq \sqrt{\K} \sup_{1\leq \ell\leq \K}\|\A_\ell-\B_\ell\|.
\]
These two identities applied to the components $\Jc_\ell(\W)$ and $\Jc_\ell(\widetilde{\W})-\Jc_\ell(\W)$ completes the proof of the bound on the spectral norm and the perturbation. To prove the bound in \eqref{rowbndm} we use the identity \eqref{mat form} to conclude that
\begin{align*}
\trow{\text{mat}\left(\mathcal{J}^T(\mtx{W})\vct{u}\right)}&=\trow{\sum_{\ell=1}^\K\text{diag}(\vct{v}_\ell)\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u}_\ell)\mtx{X}}\\
&\le\sum_{\ell=1}^\K \trow{\text{diag}(\vct{v}_\ell)\phi'\left(\mtx{W}\mtx{X}^T\right)\text{diag}(\vct{u}_\ell)\mtx{X}}\\
&\le\sum_{\ell=1}^\K B\tin{\Vb}\|\X\|\tn{\ub_\ell}\\
&= B\tin{\Vb}\|\X\|\left(\sum_{\ell=1}^\K\tn{\ub_\ell}\right)\\
&\le B\tin{\Vb}\|\X\|\sqrt{K}\left(\sum_{\ell=1}^\K\tn{\ub_\ell}^2\right)^{1/2}\\
&= B\tin{\Vb}\|\X\|\sqrt{\K},
\end{align*}
where the penultimate inequality follows from Cauchy Schwarz, completing the proof.
\end{proof}
\subsubsection{Properties of the Jacobian at random initialization}
\label{Jacrandinit}
In this section we prove a few lemmas characterizing the properties of the Jacobian at the random initialization.
\begin{lemma}[Multiclass covariance] \label{multi cov}Given input and output layer weights $\Vb$ and $\W$, consider the Jacobian described in \eqref{jacob multi}. Given an $\K n\times \K n$ matrix $\M$, for $1\leq \ell,\widetilde{\ell}\leq \K$, let $\M[\ell,\widetilde{\ell}]$ denote the $(\ell,\widetilde{\ell})$th submatrix. For $\Cb(\W)=\Jc(\W)\Jc(\W)^T$ we have
\[
\Cb(\W)[\ell,\widetilde{\ell}]=\sum_{s=1}^k(\X\X^T)\odot (\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}{\phi'(\X\w_{s})}{\phi'(\X\w_{s})^T}).
\]
Suppose $\W\distas\Nn(0,1)$ and $\Vb$ has i.i.d.~zero-mean entries with $\vrn^2$ variance. Then $\E[\Cb(\W)]$ is a block diagonal matrix given by the Kronecker product%a block-diagonal matrix where $i$th diagonal block of size $n\times n$ is given by
\[
\E[\Cb(\W)]=k\vrn^2 \Iden_{\K}\otimes \bSi(\X).
\]
where $\bSi(\X)$ is equal to $(\X\X^T)\odot \E[{\phi'(\X\w_s)}{\phi'(\X\w_s)^T}]$.
\end{lemma}
\begin{proof} The $(\ell,\widetilde{\ell} )$th submatrix of $\Cb(\W)$ is given by
\begin{align}
\label{Celll}
\Cb(\W)[\ell,\widetilde{\ell}]&=((\text{diag}(\vb_\ell)\phi'(\W\X^T))*\X^T)((\text{diag}(\vb_{\widetilde{\ell}})\phi'(\W\X^T))*\X^T)^T\nn\\
&=\sum_{s=1}^k \Jc_\ell(\w_s)\Jc_{\widetilde{\ell}}(\w_s)^T\nn\\
&=\sum_{s=1}^k\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}(\diag{\phi'(\X\w_s)}\X)(\diag{\phi'(\X\w_s)}\X)^T\nn\\
&=\sum_{s=1}^k\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}(\X\X^T)\odot ({\phi'(\X\w_s)}{\phi'(\X\w_s)^T})\nn\\
&=\sum_{s=1}^k\left(\X\X^T\right)\odot \left(\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}{\phi'(\X\w_s)}{\phi'(\X\w_s)^T}\right).
\end{align}
Setting $\W\distas\Nn(0,1)$ and $\mtx{V}$ with i.i.d. zero-mean and $\vrn^2$-variance entries, we conclude that
\begin{align*}
\E[\Cb(\W)[\ell,\widetilde{\ell}]]&=\sum_{s=1}^k(\X\X^T)\odot (\E[\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}]\E[{\phi'(\X\w_s)}{\phi'(\X\w_s)^T}])\\
&=\sum_{s=1}^k\vrn^2(\X\X^T)\odot (\delta(\ell-\widetilde{\ell})\bSi(\X))\\
&=k\delta(\ell-\widetilde{\ell})\vrn^2(\X\X^T)\odot (\bSi(\X)),
\end{align*}
where $\delta(x)$ is the discrete $\delta$ function which is 0 for $x\neq 0$ and $1$ for $x=0$.
\end{proof}
Next we state a useful lemma from \cite{Schur1911} which allows us to bound the eigenvalues of the Hadamard product of the two PSD matrices.
\begin{lemma}[\cite{Schur1911}]\label{minHad} Let $\mtx{A},\mtx{B}\in\R^{n\times n}$ be two Positive Semi-Definite (PSD) matrices. Then,
\begin{align*}
\lambda_{\min}\left(\mtx{A}\odot\mtx{B}\right)\ge& \left(\min_{i} \mtx{B}_{ii}\right)\lambda_{\min}\left(\mtx{A}\right),\\
\lambda_{\max}\left(\mtx{A}\odot\mtx{B}\right)\le& \left(\max_{i} \mtx{B}_{ii}\right)\lambda_{\max}\left(\mtx{A}\right).
\end{align*}
\end{lemma}
Next we state a lemma regarding concentration of the Jacobian matrix at initialization.
\begin{lemma}[Concentration of the Jacobian at initialization]\label{minspectJ} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$ where the activation $\phi$ obeys $|\phi(0)|\le B$ and $\abs{\phi'(z)}\le B$ for all $z$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as the rows of a matrix $\X\in\R^{n\times d}$. Furthermore, suppose $\Vb$ has i.i.d.~$\vrn$-scaled Rademacher entries (i.e.~$\pm \vrn$ equally-likely). Then, 
%as long as
%\begin{align*}
%\frac{\twonorm{\vct{v}}}{\infnorm{\vct{v}}}\ge \sqrt{20\log n}\frac{\opnorm{\X}}{\sqrt{\lambda(\X)}}B,
%\end{align*}
the Jacobian matrix at a random point $\mtx{W}_0\in\R^{k\times d}$ with i.i.d.~$\mathcal{N}(0,1)$ entries obeys 
\begin{align*}
%&\sigma_{\min}\left(\mathcal{J}(\W_0)\right)\ge \frac{1}{\sqrt{2}}\twonorm{\vct{v}}\sqrt{\lambda(\X)},\\
&\opnorm{\Jc(\W_0)\Jc(\W_0)^T-\E[\Jc(\W_0)\Jc(\W_0)^T]}\leq 30\K\sqrt{k}\vrn^2B^2\|\X\|^2\log(2n).
\end{align*}
with probability at least $1-1/n^{100}$. In particular, as long as
\[
k\geq \frac{1000\K^2B^4\|\X\|^4\log^2(2n)}{\delta^2},
\]
with the same probability, we have that
\[
\opnorm{\frac{1}{k\vrn^2}\Jc(\W_0)\Jc(\W_0)^T- \Iden_{\K}\otimes \bSi(\X)}\leq \delta.
\]
\end{lemma}
\begin{proof} 
Define $\Cb=\Jc(\W_0)\Jc(\W_0)^T$. We begin by showing that the diagonal blocks of $\Cb$. To do this first
for $1\le s\le k$ define the random matrices
\[
\A_s=\left(\phi'\left(\X\w_s\right)\phi'\left(\X\w_s\right)^T\right)\odot\left(\X\X^T\right).
\]
Now consider $n\times n$ diagonal blocks of $\Cb$ (denoted by $\Cb[\ell,\ell]$) and note that we have
\begin{align*}
 \Cb[\ell,\ell]=&\left(\phi'\left(\X\W^T\right)\text{diag}(\vct{v}_\ell)\text{diag}(\vct{v}_\ell)\phi'\left(\W\X^T\right)\right)\odot\left(\X\X^T\right)\\
 =&\sum_{s=1}^k \mtx{V}_{\ell,s}^2\A_s\\
 =&\vrn^2\sum_{s=1}^k \A_s.
\end{align*}
%\E[\A_\ell]=\mtx{\Sigma}(\X)\quad,\quad
Furthermore, using Lemma \ref{minHad}
\begin{align*}
\opnorm{\A_s}\le \left(\underset{i}{\max}\text{ }\left(\phi'(\vct{x}_i^T\w_s)\right)^2\right)\opnorm{\X}^2\le B^2\opnorm{\X}^2.
\end{align*}
Also, using Jensen's inequality 
\begin{align*}
\opnorm{\E[\A_s]}\le \E\opnorm{\A_s}\le B^2\opnorm{\X}^2.
\end{align*}
Combining the latter two identities via the triangular inequality we conclude that
\begin{align}
\label{randjtemp}
\opnorm{(\A_s-\E[\A_s])^2}=\opnorm{\A_s-\E[\A_s]}^2\le \left(\opnorm{\A_s}+\opnorm{\E[\A_s]}\right)^2\leq \left(2B^2\|\X\|^2\right)^2.
\end{align}
To proceed, we will bound the weighted sum
\[
\Sb=\sum_{s=1}^k\vrn^2(\A_s-\E[\A_s])
\]
in spectral norm. To this aim we utilize the Matrix Hoeffding inequality which states that
\[
\Pro(\|\Sb\|\geq t)\leq 2ne^{-\frac{t^2}{2\Delta^2}},
\]
where $\Delta^2$ is an upper bound on $\opnorm{\sum_{s=1}^k\vrn^4(\A_s-\E[\A_s])^2}$. Using \eqref{randjtemp} we can pick $\Delta^2=\sum_{s=1}^k (2\vrn^2B^2\|\X\|^2)^2=4k\vrn^4B^4\|\X\|^4$. Setting $t=30\sqrt{k}\vrn^2B^2\|\X\|^2\log(2n)$, we conclude that
\[
\Pro\Big\{\opnorm{\Cb[\ell,\ell]-\E[\Cb[\ell,\ell]]}\geq t\Big\}=\Pro(\|\Sb\|\geq t)\leq n^{-102}%\tn{\vb}^2\mtx{\Sigma}(\X)
\]
concluding the proof of concentration of the diagonal blocks of $\Cb$. 

For the off-diagonal blocks $\Cb[\ell,\widetilde{\ell}]$ using \eqref{Celll} from the proof of Lemma \ref{multi cov} we have that
\[
\Cb[\ell,\widetilde{\ell}]=\sum_{s=1}^k \mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}\A_{s}.
\]
Note that by construction $\{\mtx{V}_{\ell,s}\mtx{V}_{\widetilde{\ell},s}\}_{s=1}^k$ are i.i.d.~$\pm \vrn^2$ Rademacher variables and thus $\Cb[\ell,\widetilde{\ell}]$ is sum of zero-mean i.i.d.~matrices and we are again in the position to apply Hoeffding's inequality. To this aim note that 
\begin{align*}
\opnorm{\sum_{s=1}^k\mtx{V}_{\ell,s}^2\mtx{V}_{\widetilde{\ell},s}^2\A_{s}^2}=\vrn^4\opnorm{\sum_{s=1}^k\A_{s}^2}\le \vrn^4\sum_{s=1}^k\opnorm{\A_s}^2\le \vrn^4kB^4\opnorm{\X}^4,
\end{align*}
so that we can take $\Delta^2=\vrn^4kB^4\opnorm{\X}^4$ and again conclude that for $t=30\sqrt{k}\vrn^2B^2\|\X\|^2\log(2n)$ we have
\[
\Pro\Big\{\opnorm{\Cb[\ell,\widetilde{\ell}]}\geq t\Big\}\leq n^{-102}
\]
Using the fact that $\E[\Cb[\ell,\widetilde{\ell}]]=0$ and $K\le n$, combined with a union bound over all sub-matrices $1\leq \ell,\widetilde{\ell}\leq K$ we conclude thatt
\[
\Pro\Big\{\opnorm{\Cb[\ell,\widetilde{\ell}]-\E\big[\Cb[\ell,\widetilde{\ell}]\big]}\geq t\Big\}\leq K^2n^{-102}\leq n^{-100}.
\]
All that remains is to combine the concentration results for the sub-matrices to arrive at the complete bound. In mathematical terms we need to bound ${\bf{D}}:=\|\Cb-\E[\Cb]\|$.To this aim define $\Db[\ell,:]$ to denote the $\ell$th block row of $\Db$. Standard bounds on spectral norm in terms of sub-matrices yields allows us to conclude that 
\begin{align*}
\|\Db[\ell,:]\|\leq& \sqrt{\K}\sup_{1\leq \widetilde{\ell}\leq \K} \opnorm{\Db[\ell,\widetilde{\ell}]}\leq \sqrt{\K}t\quad\Rightarrow\\
\|\Db\|\leq& \sqrt{\K}\sup_{1\leq \ell\leq \K} \|\Db[\ell,:]\|\leq \sqrt{\K}\sqrt{\K}t=\K t=30\K\sqrt{k}\vrn^2B^2\|\X\|^2\log(2n),
\end{align*}
concluding the proof. The result in terms of $\delta$ is obtained by using the population covariance Lemma \ref{multi cov}.% plugging $\tn{\vb}^2=k\sigma^2$ and 
\end{proof}

%\subsubsection{Proof of Lemma \ref{multi cov}}
%\begin{proof} $\Jc(\W_0)$ can be written as $\Jc(\W_0)=[\Jc_1(\W_0)^T~\dots~\Jc_\K(\W_0)^T]^T$ where $\Jc_i(\W_0)$ is the Jacobian corresponding to the $i$th output node of the network. Consequently, the diagonal blocks of $\E[\Jc(\W_0)\Jc(\W_0)^T]$ are equal to $\E[\Jc_i(\W_0)\Jc_i(\W_0)^T]\in\R^{n\times n}$ which is equal to the matrix $\E\Big[\left(\phi'\left(\X\w\right)\phi'\left(\X\w\right)^T\right)\odot\left(\X\X^T\right)\Big]$ \cite{du2018gradient,oymak2019towards}. What remains is proving that the off-diagonal blocks are zero. Observe that, conditioned on $\W$, $\Jc_i(\W_0)^T$ is a zero-mean random variable which is a a linear function of the $i$th row of $\Vb$, hence $\Jc_i(\W_0)$ and $\Jc_j(\W_0)$ are independent for $i\neq j$ which yields $\E[\Jc_i(\W_0)\Jc_j(\W_0)^T]=\E[\Jc_i(\W_0)]\E[\Jc_j(\W_0)^T]=0$.
%\end{proof}
\subsubsection{Upper bound on initial residual}
\label{initmisfit}
In this section we prove a lemma concerning the size of the initial misfit. The proof of this lemma (stated below) follows from a similar argument in the proof of \cite[Lemma 6.12]{onehidden}.
\begin{lemma}[Upper bound on initial residual]\label{upresz} Consider a one-hidden layer neural network model of the form $\vct{x}\mapsto \Vb\phi\left(\W\x\right)$ where the activation $\phi$ has bounded derivatives obeying $|\phi(0)|,\abs{\phi'(z)}\le B$. Also assume we have $n$ data points $\vct{x}_1, \vct{x}_2,\ldots,\vct{x}_n\in\R^d$ with unit euclidean norm ($\twonorm{\vct{x}_i}=1$) aggregated as rows of a matrix $\X\in\R^{n\times d}$ and the corresponding labels given by $\vct{y}\in\R^{\K n}$. Furthermore, assume the entries of $\Vb$ are i.i.d.~Rademacher variables scaled by $\frac{\vrn\twonorm{\y}}{50B\sqrt{\K \log(2\K)kn}}$ and the entries of $\mtx{W}\in\R^{k\times d}$ are i.i.d.~$\mathcal{N}(0,1)$. Then,
\begin{align*}
\fronorm{\Vb\phi\left(\W\X^T\right)}\le\vrn\twonorm{\y},
\end{align*}
holds with probability at least $1-(2\K)^{-100}$.
\end{lemma}
\begin{proof}
\label{upreszpf}
We begin the proof by noting that
\[
\fronorm{\Vb\phi\left(\W\X^T\right)}^2=\sum_{\ell=1}^\K \twonorm{\vb_\ell^T\phi\left(\W\X^T\right)}^2.
\]
We will show that for any row $\vb$ of $\Vb$, with probability at least $1-(2\K)^{-101}$,
\begin{align}
\label{singr}
 \twonorm{\vb_\ell^T\phi\left(\W\X^T\right)}\leq \frac{\vrn}{\sqrt{\K}}\twonorm{\y}.
\end{align}
so that a simple union bound can conclude the proof. Therefore, all that remains is to show \eqref{singr} holds. To prove the latter, note that for any two matrices $\widetilde{\W}, \W\in\R^{k\times d}$ we have
\begin{align*}
\abs{\twonorm{\phi\left(\X\widetilde{\W}^T\right)\vct{v}}-\twonorm{\phi\left(\X\W^T\right)\vct{v}}}\le& \twonorm{\phi\left(\X\widetilde{\W}^T\right)\vct{v}-\phi\left(\X\W^T\right)\vct{v}}\\
\le&\opnorm{\phi\left(\X\widetilde{\W}^T\right)-\phi\left(\X\W^T\right)}\twonorm{\vct{v}}\\
\le& \fronorm{\phi\left(\X\widetilde{\W}^T\right)-\phi\left(\X\W^T\right)}\twonorm{\vct{v}}\\
& \hspace{-100pt}\overset{(a)}{=}\fronorm{\left(\phi'\left(\Sb\odot\X\widetilde{\W}^T+(1_{k\times n}-\Sb)\odot\X\W^T\right)\right)\odot \left(\X(\widetilde{\W}-\W)^T\right)}\twonorm{\vct{v}}\\
\le&B\fronorm{\X(\widetilde{\W}-\W)^T}\twonorm{\vct{v}}\\
\le&B\opnorm{\X}\twonorm{\vct{v}}\fronorm{\widetilde{\W}-\W},
\end{align*}
where in (a) we used the mean value theorem with $\Sb$ a matrix with entries obeying $0\le \Sb_{i,j}\le 1$ and $1_{k\times n}$ the matrix of all ones. Thus, $\twonorm{\phi\left(\X\W^T\right)\vct{v}}$ is a $B\opnorm{\X}\twonorm{\vct{v}}$-Lipschitz function of $\mtx{W}$. Thus, fixing $\vb$, for a matrix $\W$ with i.i.d.~Gaussian entries 
\begin{align}
\label{tempmyflip}
\twonorm{\phi\left(\X\W^T\right)\vct{v}}\le \E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}\big]+t,
\end{align}
holds with probability at least $1-e^{-\frac{t^2}{2B^2\twonorm{\vct{v}}^2\opnorm{\X}^2}}$. Next given $g\sim\Nn(0,1)$, we have
\begin{align}
|\E[\phi(g)]|\leq |\E[\phi(0)]|+|\E[\phi(g)-\phi(0)]|\leq B+B\E[|g|]\leq 2B\quad\text{and}\quad \text{Var}(\phi(g))\le B^2.\label{poinc stuff}
\end{align}
where the latter follows from Poincare inequality (e.g.~see \cite[p. 49]{ledoux}).
Furthermore, since $\vb$ has i.i.d.~Rademacher entries, applying Bernstein bound, event 
\begin{align}
E_{\vb}:=\{|\onebb^T\vb|^2\leq 250\log \K \tn{\vb}^2\} \label{berns v}
\end{align}
holds with probability $1-(2\K)^{-102}$. Conditioned on $E_{\vb}$, we now upper bound the expectation via
\begin{align*}
\E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}\big]\overset{(a)}{\le}& \sqrt{\E\big[\twonorm{\phi\left(\X\W^T\right)\vct{v}}^2\big]}\\
=&\sqrt{\sum_{i=1}^n \E\big[\left(\vct{v}^T\phi(\W\vct{x}_i)\right)^2\big]}\\
\overset{(b)}{=}&\sqrt{n}\sqrt{\E_{\vct{g}\sim\mathcal{N}(\vct{0},\mtx{I}_k)}\big[\left(\vct{v}^T\phi(\vct{g})\right)^2\big]}\\
\overset{(c)}{=}&\sqrt{n}\sqrt{\twonorm{\vct{v}}^2\E_{g\sim\mathcal{N}(0,1)}\big[\left(\phi(g)-\E[\phi(g)]\right)^2\big]+(\vct{1}^T\vct{v})^2(\E_{g\sim\mathcal{N}(0,1)}[\phi(g)])^2}\\
\overset{(d)}{=}&\sqrt{n}\twonorm{\vct{v}}\sqrt{250\times 4B^2\log (2\K) +B^2}\\
{\le}&32\sqrt{n\log (2\K) }B\twonorm{\vct{v}}.
\end{align*}
Here, (a) follows from Jensen's inequality, (b) from linearity of expectation and the fact that for $\vct{x}_i$ with unit Euclidean norm $\mtx{W}\vct{x}_i\sim\mathcal{N}(\vct{0},\mtx{I}_k)$, (c) from simple algebraic manipulations, (d) from the inequalities \eqref{berns v} and \eqref{poinc stuff}. Thus using $t=18\sqrt{n\log (2\K) }B\twonorm{\vct{v}}$ in \eqref{tempmyflip}, conditioned on $E_{\vb}$ we conclude that
\begin{align}
\twonorm{\phi\left(\X\W^T\right)\vct{v}}\le&50\sqrt{n\log (2\K) }B\twonorm{\vct{v}}=50\sqrt{n\log (2\K) }B\sqrt{k}\frac{\vrn\twonorm{\y}}{50B\sqrt{\K\log (2\K) kn}}=\frac{\vrn \tn{\y}}{\sqrt{\K}}.,\label{fin fin eq}
\end{align}
holds with probability at least $1-\exp(-102\log (2\K)\frac{n}{\opnorm{\X}^2})\geq 1-(2\K)^{-102}$ where we used $n\geq \|\X\|^2$. Using a union bound over $E_{\vb}$ and the conditional concentration over $\W$, the overall probability of success in \eqref{fin fin eq} is at least $1-(2\K)^{-101}$ concluding the proof of \eqref{singr} and the Lemma.
\end{proof}

\subsection{Rademacher complexity and generalization bounds}
\label{radam}
In this section we state and prove some Rademacher complexity results that will be used in our generalization bounds. We begin with some basic notation regarding Rademacher complexity.
%Population error can be upper bounded as
%\[
%\Lc_P(h)\leq \Lc_S(h)+2\Rc(
%\]
% parameterized by weights $\W$.
Let $\Fc$ be a function class. Suppose $f\in\Fc$ maps $\R^d$ to $\R^K$. Let $\{\vct{\eps}_i\}_{i=1}^n$ be i.i.d.~vectors in $\R^K$ with  i.i.d.~Rademacher variables. Given i.i.d.~samples $\Sc=\{(\x_i,\y_i)\}_{i=1}^n\sim \Dc$, we define the empirical Rademacher complexity to be
\[
\mathcal{R}_{\Sc}(\Fc)=\frac{1}{n}\E\bigg[\sup_{f\in\Fc}\text{ }\sum_{i=1}^n \vct{\eps}_{i}^T f(\x_i)\bigg].
\]
We begin by stating a vector contraction inequality by Maurer \cite{maurer2016vector}. This is obtained by setting $h_i(f(\x_i))=h(\y_i,f(\x_i))$ in Corollary 4 of \cite{maurer2016vector}.
\begin{lemma} \label{lem multi}Let $f(\cdot):\R^d\rightarrow \R^\K$ and let $\ell:\R^\K\times \R^K\rightarrow\R$ be a $1$ Lipschitz loss function with respect to second variable. Let $\{\eps_i\}_{i=1}^n$ be i.i.d.~Rademacher variables. Given i.i.d.~samples $\{(\x_i,\y_i)\}_{i=1}^n$, define
\[
\mathcal{R}_{\Sc}(\ell,\Fc)=\E\bigg[\sup_{f\in \Fc}\sum_{i=1}^n\eps_i \ell(\y_i,f(\x_i))\bigg].
\]
We have that
\[
\mathcal{R}_{\Sc}(\ell,\Fc)\leq \sqrt{2}\mathcal{R}_{\Sc}(\Fc).
\]
\end{lemma}

%\begin{lemma} Let $f(\cdot):\R\rightarrow \R$ and let $\ell_i:\R\rightarrow[0,1]$ be $1$ Lipschitz loss functions. Given i.i.d.~samples $(\x_i)_{i=1}^n$, consider the empirical loss
%\[
%\Lc(\ell,\W)=\frac{1}{n}\sum_{i=1}^n \ell_i(f(\x_i,\W)).
%\]
%With probability $1-\delta$ over samples, for all $f\in \Fc$, we have that
%\[
%\E[\Lc(\ell,\W)]\leq \Lc(\ell,\W)+2\Rc_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
%\]
%\end{lemma}
Combining the above result with standard generalization bounds based on Rademacher complexity \cite{bartlett2002rademacher} allows us to prove the following result.
\begin{lemma} \label{standard rad}Let $\ell(\cdot,\cdot):\R^\K\times \R^\K\rightarrow [0,1]$ be a $1$ Lipschitz loss function. Given i.i.d.~samples $\{(\x_i,\y_i)\}_{i=1}^n$, consider the empirical loss
\[
\Lc(f,\ell)=\frac{1}{n}\sum_{i=1}^n \ell(\y_i,f(\x_i)).
\]
With probability $1-\delta$ over the samples, for all $f\in \Fc$, we have that
\[
\E[\Lc(f,\ell)]\leq \Lc(f,\ell)+2\sqrt{2}\mathcal{R}_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
\]
\end{lemma}
\begin{proof} Based on \cite{bartlett2002rademacher}, 
\[
\E[\Lc(f,\ell)]\leq \Lc(f,\ell)+2\mathcal{R}_{\Sc}(\ell,\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}}
\]
holds with $1-\delta$ probability. Combining the latter with Lemma \ref{lem multi} completes the proof.
\end{proof}

\begin{lemma} \label{rad rad bound} Consider a neural network model of the form $\x\mapsto f(\x;\Vb,\W)=\Vb\phi\left(\W\x\right)$ with $\W\in\R^{k\times d}$ and $\Vb\in\R^{\K\times k}$ denoting the input and output weight matrices. Suppose $\mtx{V}_0\in\R^{K\times k}$ is a matrix obeying $\tin{\Vb_0}\leq \vrn/\sqrt{k\K}$. Also let $\W_0\in\R^{k\times d}$ be a reference input weight matrix. Furthermore, we define the neural network function  space parameterized by the weights as follows
\begin{align}
&\mathcal{F}_{\Vc,\Wc}=\Big\{f(\x;\Vb,\W)\quad\text{such that}\quad\Vb\in\Vc\quad\text{and}\quad\W\in\Wc\Big\}\quad\text{with}\quad\Vc=\bigg\{\Vb: \fronorm{\Vb-\Vb_0}\le \frac{\vrn M_{\mathcal{V}}}{\sqrt{\K k}}\bigg\}\nn\\
&\quad\quad\text{and}\quad\Wc=\bigg\{\W: \fronorm{\W-\W_0}\le M_{\mathcal{W}}\quad\text{and}\quad \|\W-\W_0\|_{2,\infty}\le \frac{R}{\sqrt{k}}\Big\}.\label{space func}
\end{align}
Additionally, assume the training data $\{(\vct{x}_i,\y_i)\}_{i=1}^n$are generated i.i.d. with the input data points of unit Euclidean norm (i.e.~$\tn{\x_i}=1$). Also, define the average energy at $\W_0$ as
\[
E=\left(\frac{1}{kn}\sum_{i=1}^n\tn{\phi(\W_0\x_i)}^2\right)^{1/2}.
\]
Also let $\{\vct{\xi}_i\}_{i=1}^n\in\R^\K$ be i.i.d.~vectors with i.i.d.~Rademacher entries and define the empirical Rademacher complexity
\begin{align*}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\Vc,\Wc}\right):=&\frac{1}{n}\E\Bigg[\underset{f\in\mathcal{F}_{\Vc,\Wc}}{\sup}\text{ }\sum_{i=1}^n \vct{\xi}_i^Tf(\x_i)\Bigg].
\end{align*}
Then,%{\textcolor{red}{MOVE TO multiclass starting here!}} 
\begin{align}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\Vc,\Wc}\right)\le  \vrn B\left(\frac{M_{\mathcal{W}}+EM_{\mathcal{V}}}{\sqrt{n}}+\frac{R^2+M_{\mathcal{W}}M_{\mathcal{V}}}{\sqrt{k}}\right).\label{emp rad comp}
\end{align} 
\end{lemma}
\begin{proof}
We shall use $\w_\ell$ to denote the rows of $\W$ (same for $\W_0,\Vb,\Vb_0$). We will approximate $\phi\left(\langle \w_\ell,\x_i\rangle\right)$ by its linear approximation $\phi\left(\langle \w_\ell^0, \x_i\rangle\right)+\phi'(\langle\w_\ell^0,\x_i\rangle)\left(\langle\w_\ell-\w_\ell^0,\x_i\rangle\right)$ via the second order Taylor's mean value theorem. We thus have
\begin{align*}
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\Vc,\Wc}\right)\le&\frac{1}{n}\E\Bigg[\sum_{i=1}^n\vct{\xi}^T_i\Vb_0\phi\left(\W_0\x_i\right)\Bigg]\\
&+\underbrace{\frac{1}{n}\E\Bigg[\underset{\W\in\Wc}{\sup}\text{ }\sum_{i=1}^n \vct{\xi}^T_i\Vb_0\text{diag}\left(\phi'\left(\W_0\x_i\right)\right)\left(\W-\W_0\right)\x_i\Bigg]}_{\mathcal{R}_1}\\
&+\underbrace{\frac{1}{2n}\E_{\xi_{i,j}\distas\pm 1}\Bigg[\underset{\W\in\Wc}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k  \sum_{j=1}^\K\xi^T_{i,j}\vb_{0,j,\ell}\phi''\left((1-t_{i\ell})\langle\w_\ell^0,\x_i\rangle+t_{i\ell}\langle\w_\ell,\x_i\rangle\right)\left(\langle\w_\ell-\w_\ell^0,\x_i\rangle\right)^2\Bigg]}_{\mathcal{R}_2}\\
&+\underbrace{\frac{1}{n}\E\bigg[\sup_{\Vb\in\Vc,\W\in\Wc}\sum_{i=1}^n\vct{\xi}_i^T(\Vb-\Vb_0)(\phi(\W\x_i)-\phi(\W_0\x_i))\bigg]}_{\mathcal{R}_3}\\
&+\underbrace{\frac{1}{n}\E\bigg[\sup_{\Vb\in\Vc}\sum_{i=1}^n\vct{\xi}_i^T(\Vb-\Vb_0)\phi(\W_0\x_i)\bigg]}_{\mathcal{Rc}_4}
\end{align*}
We proceed by bounding each of these four terms. For the first term note that
\begin{align*}
\mathcal{R}_1\le& \frac{1}{n}\E\Bigg[\underset{\fronorm{\W-\W_0}\le M_{\mathcal{W}}}{\sup}\text{ }\sum_{i=1}^n \vct{\xi}^T_i\Vb_0\text{diag}\left(\phi'\left(\W_0\x_i\right)\right)\left(\W-\W_0\right)\x_i\Bigg]\\
\le& \frac{1}{n}\E\Bigg[\underset{\fronorm{\W-\W_0}\le M_{\mathcal{W}}}{\sup}\text{ }\Big\langle\sum_{i=1}^n \text{diag}\left(\phi'\left(\W_0\x_i\right)\right)\Vb_0^T\vct{\xi}_i\x_i^T,\W-\W_0\Big\rangle\Bigg]\\
\le&\frac{M_{\mathcal{W}}}{n}\E\Bigg[\fronorm{\left(\sum_{i=1}^n \text{diag}\left(\Vb_0^T\vct{\xi}_i\right)\phi'\left(\W_0\x_i\right)\x_i^T\right)}\Bigg]\\
\le&\frac{M_{\mathcal{W}}}{n}\E\Bigg[\fronorm{\left(\sum_{i=1}^n \text{diag}\left(\Vb_0^T\vct{\xi}_i\right)\phi'\left(\W_0\x_i\right)\x_i^T\right)}^2\Bigg]^{1/2}\\
=&\frac{M_{\mathcal{W}}}{n}\Bigg[\sum_{i=1}^n\E\fronorm{ \text{diag}\left(\Vb_0^T\vct{\xi}_i\right)\phi'\left(\W_0\x_i\right)\x_i^T}^2\Bigg]^{1/2}\\
=&\frac{M_{\mathcal{W}}}{n}\Bigg[\sum_{i=1}^n\E\tn{ \text{diag}\left(\Vb_0^T\vct{\xi}_i\right)\phi'\left(\W_0\x_i\right)}^2\Bigg]^{1/2}\\
\le&\frac{BM_{\mathcal{W}}}{n}\Bigg[\sum_{i=1}^n\E\tn{ \Vb_0^T\vct{\xi}_i}^2\Bigg]^{1/2}\\
\le&\frac{BM_{\mathcal{W}}}{n}\tf{\Vb_0}\\
\le& \frac{BM_{\mathcal{W}}\vrn}{\sqrt{n}},
\end{align*}
where in the last inequality we used the fact that $\tf{\Vb_0}\leq \vrn$. For the second term note that
\begin{align*}
\mathcal{R}_2\le& \frac{1}{2n}\E\Bigg[\underset{\|\W-\W_0\|_{2,\infty}\le R}{\sup}\text{ }\sum_{i=1}^n\sum_{\ell=1}^k  \sum_{j=1}^\K\xi_{i,j}\vb_{0,j,\ell}\phi''\left((1-t_{i\ell})\langle\w_\ell^0,\x_i\rangle+t_{i\ell}\langle\w_\ell,\x_i\rangle\right)\left(\langle\w_\ell-\w_\ell^0,\x_i\rangle\right)^2\Bigg]\\
\le&\frac{1}{2n}\sum_{\ell=1}^k \E\Bigg[\underset{\tn{\w_\ell-\w_\ell^0}\le R}{\sup}\text{ }\sum_{i=1}^n\abs{ \sum_{j=1}^\K\xi_{i,j}\vb_{0,j,\ell}}\abs{\phi''\left((1-t_{i\ell})\langle\w_\ell^0,\x_i\rangle+t_{i\ell}\langle\w_\ell,\x_i\rangle\right)}\left(\langle\w_\ell-\w_\ell^0,\x_i\rangle\right)^2\Bigg]\\
\le&\frac{1}{2kn}\sum_{\ell=1}^k\sum_{i=1}^n  \E\Bigg[\abs{\sum_{j=1}^\K\xi_{i,j}\vb_{0,j,\ell}}\Bigg]R^2B\\
\le &\frac{BR^2}{2k} \|\Vb_0^T\|_{2,1}\\
\le& \frac{BR^2\vrn}{2\sqrt{k}}.
%\le&\frac{1}{2n}\sum_{\ell=1}^k\sum_{i=1}^n \frac{\sigma}{\sqrt{k}}BR^2\\
%=&\frac{1}{2}BR^2\sigma\sqrt{k}
\end{align*} %Let $\tilde{M}=\sigma\bar{M}/\sqrt{k\K}$. 
In the above we used $\|\mtx{M}\|_{2,1}$ for a matrix $\mtx{M}$ to denote the sum of the Euclidean norm of the rows of $\mtx{M}$. We also used the fact that $ \|\Vb_0^T\|_{2,1}\leq \vrn\sqrt{k}$. To bound the third term note that
\begin{align*}
\mathcal{R}_3&=\frac{1}{n}\E\bigg[\sup_{\Vb\in\Vc,\W\in\Wc}\sum_{i=1}^n\vct{\xi}_i^T(\Vb-\Vb_0)(\phi(\W\x_i)-\phi(\W_0\x_i))\bigg]\\
&\le\frac{1}{n}\E\bigg[\sup_{\Vb\in\Vc,\W\in\Wc}\sum_{i=1}^n\fronorm{\Vb-\Vb_0}\twonorm{\vct{\xi}_i}\twonorm{(\phi(\W\x_i)-\phi(\W_0\x_i))}\bigg]\\
&\le\frac{\vrn M_{\mathcal{V}}}{n\sqrt{kK}}\E\Big[\sup_{\W\in\Wc}\sum_{i=1}^n\tn{\vct{\xi}_i}\tn{\phi(\W\x_i)-\phi(\W_0\x_i)}\Big]\\
&\le\frac{\vrn M_{\mathcal{V}}}{n\sqrt{k}}\cdot\sup_{\W\in\Wc}\sum_{i=1}^n\tn{\phi(\W\x_i)-\phi(\W_0\x_i)}\\ 
&\le\frac{\vrn B M_{\mathcal{V}}}{n\sqrt{k}}\cdot\sup_{\W\in\Wc}\sum_{i=1}^n\tn{(\W-\W_0)\x_i}\\ 
&\le\frac{\vrn B M_{\mathcal{V}}}{n\sqrt{k}}\cdot\sup_{\W\in\Wc}\sum_{i=1}^n\fronorm{(\W-\W_0)}\\ 
&=\frac{\vrn B M_{\mathcal{V}}}{\sqrt{k}}\cdot\sup_{\W\in\Wc}\fronorm{(\W-\W_0)}\\ 
&=\frac{\vrn BM_{\mathcal{V}}M_{\mathcal{W}}}{\sqrt{k}}.
\end{align*}
Finally, to bound the fourth term note that we have
\begin{align*}
\mathcal{R}_4&=\frac{1}{n}\E\bigg[\sup_{\Vb\in\Vc}\sum_{i=1}^n\vct{\xi}_i^T(\Vb-\Vb_0)\phi(\W_0\x_i)\bigg]\\
&=\frac{1}{n}\E\bigg[\sup_{\fronorm{\Vb-\Vb_0}\le \frac{\vrn M_{\mathcal{V}}}{\sqrt{kK}}}\Big\langle\sum_{i=1}^n\vct{\xi}_i\phi(\W_0\x_i)^T,(\Vb-\Vb_0)\Big\rangle\bigg]\\
&=\frac{\vrn M_{\mathcal{V}}}{n\sqrt{kK}}\E\bigg[\fronorm{\sum_{i=1}^n\phi(\W_0\x_i)\vct{\xi}_i^T}\bigg]\\
&\le\frac{\vrn M_{\mathcal{V}}}{n\sqrt{kK}}\left(\E\bigg[\fronorm{\sum_{i=1}^n\phi(\W_0\x_i)\vct{\xi}_i^T}^2\bigg]\right)^{1/2}\\
&=\frac{\vrn M_{\mathcal{V}}}{n\sqrt{kK}}\left(\sum_{i=1}^n\E\bigg[\fronorm{\phi(\W_0\x_i)\vct{\xi}_i^T}^2\bigg]\right)^{1/2}\\
&=\frac{\vrn M_{\mathcal{V}}}{\sqrt{n}}\left(\frac{1}{kn}\sum_{i=1}^n\E\bigg[\fronorm{\phi(\W_0\x_i)}^2\bigg]\right)^{1/2}\\
&=\frac{\vrn EM_{\mathcal{V}}}{\sqrt{n}}\\
&\le\frac{\vrn BEM_{\mathcal{V}}}{\sqrt{n}}
\end{align*}
Combining these four bounds we conclude that
\[
\mathcal{R}_{\mathcal{S}}\left(\mathcal{F}_{\Vc,\Wc}\right)\leq \vrn B\left(\frac{M_{\mathcal{W}}}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}+\frac{\vrn BM_{\mathcal{V}}M_{\mathcal{W}}}{\sqrt{k}}+\frac{EM_{\mathcal{V}}}{\sqrt{n}}\right),
\]
concluding the proof of \eqref{emp rad comp}.
\end{proof}
Next we state a crucial lemma that connects the test error measured by any Lipschitz loss to that of the quadratic loss on the training data. 
\begin{lemma} \label{generalize corollary} Consider a one-hidden layer neural network with input to output mapping of the form $\vct{x}\in\R^d\mapsto f(\vct{x};\Vb,\mtx{W})=\mtx{V}\phi\left(\W\vct{x}\right)\in\R^K$ with $\W\in\R^{k\times d}$ denoting the input-to-hidden weights and $\V\in\R^{k\times K}$ the hidden-to-output weights. Suppose $\mtx{V}_0\in\R^{K\times k}$ is a matrix obeying $\tin{\Vb_0}\leq \vrn/\sqrt{k\K}$. Also let $\W_0\in\R^{k\times d}$ be a reference input weight matrix. Also define the empirical losses
\begin{align*}
\mathcal{L}(\V,\W)=\frac{1}{n}\sum_{i=1}^n \tn{\y_i-f(\x_i;\Vb,\W)}^2,
\end{align*}
and
\begin{align*}
\mathcal{L}(f,\ell)=\frac{1}{n}\sum_{i=1}^n \ell(f(\x_i;\Vb,\W),\y_i),
\end{align*}
with $\ell:\R^\K\times \R^\K\rightarrow [0,1]$ a one Lipschitz loss function obeying $\ell(\y,\y)=0$. Additionally, assume the training data $\{(\vct{x}_i,\y_i)\}_{i=1}^n$are generated i.i.d. according to a distribution $\mathcal{D}$ with the input data points of unit Euclidean norm (i.e.~$\tn{\x_i}=1$). Also, define the average energy at $\W_0$ as
\[
E=\left(\frac{1}{kn}\sum_{i=1}^n\tn{\phi(\W_0\x_i)}^2\right)^{1/2}.
\]
Then for all $f$ in the function class $\mathcal{F}_{\Wc}$ given by \eqref{space func}
\begin{align}
\E[\Lc(f,\ell)]\leq \sqrt{\Lc(\Vb,\W)}+ 2\sqrt{2}\vrn B\left(\frac{M_{\mathcal{W}}}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}+\frac{\vrn BM_{\mathcal{V}}M_{\mathcal{W}}}{\sqrt{k}}+\frac{EM_{\mathcal{V}}}{\sqrt{n}}\right)+\sqrt{\frac{5\log(2/\delta)}{n}},\label{ell pop bound}
\end{align}
holds with probability at least $1-\delta$. Furthermore, Suppose labels are one-hot encoded and thus unit Euclidian norm. Given a sample $(\x,\y)\in\R^d\times \R^\K$ generated according to the distribution $\mathcal{D}$, define the population classification error
\[
\err{\W}=\Pro(\arg\max_{1\leq \ell\leq K}\y_i\neq \arg\max_{1\leq \ell\leq K}f_i(\x,\W)).
\]
Then, we also have
\begin{align}
\err{\W}\leq 2\left[\sqrt{\Lc(\Vb,\W)}+ 2\sqrt{2}\vrn B\left(\frac{M_{\mathcal{W}}}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}+\frac{\vrn BM_{\mathcal{V}}M_{\mathcal{W}}}{\sqrt{k}}+\frac{EM_{\mathcal{V}}}{\sqrt{n}}\right)+\sqrt{\frac{5\log(2/\delta)}{n}}\right].\label{err pop bound}
\end{align}
\end{lemma}
\begin{proof} 
%Define empirical $\ell_2$ loss
%\[
%\Lc(\ell_2,\W)=\frac{1}{n}\sum_{i=1}^n\tn{\y_i-f(\x_i,\W)}.
%\]
%Using Cauchy-Schwarz, we have that $\sqrt{\Lc(\W)}\geq {\Lc(\ell_2,\W)}$.
To begin first note that any 1-Lipschitz $\ell$ with $\ell(\y,\y)=0$ obeys $\ell(\y,\hat{\y})\leq \tn{\y-\hat{\y}}$. Thus, we have
\[
\Lc(f,\ell)\leq \frac{1}{n}\sum_{i=1}^n\tn{\y_i-f(\x_i;\Vb,\W)}\leq \sqrt{\Lc(\Vb,\W)},
\] 
where the last inequality follows from Cauchy-Schwarz. Consequently, applying Lemmas \ref{standard rad} and \ref{rad rad bound} we conclude that
\begin{align*}
\E[\Lc(\ell,\W)]&\leq \Lc(f,\ell)+2\sqrt{2}\cdot\mathcal{R}_{\Sc}(\Fc)+\sqrt{\frac{5\log(2/\delta)}{n}},\\
&\leq\sqrt{\Lc(\W)}+ 2\sqrt{2}\vrn B\left(\frac{M_{\mathcal{W}}}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}+\frac{\vrn BM_{\mathcal{V}}M_{\mathcal{W}}}{\sqrt{k}}+\frac{EM_{\mathcal{V}}}{\sqrt{n}}\right)+\sqrt{\frac{5\log(2/\delta)}{n}},
\end{align*}
which yields the first statement.

To prove the second statement on classification accuracy, we pick the $\ell$ function as follows
\[
\ell(\y,\hat{\y})=\min(1,\tn{\y-\hat{\y}}).
\]
Note that, given a sample $(\x,\y)\in\R^d\times \R^\K$ with one-hot encoded labels, if 
\begin{align*}
\arg\max_{1\leq \ell\leq K}\y_\ell\neq \arg\max_{1\leq \ell\leq K}f_\ell(\x;\Vb,\W),
\end{align*} 
this implies 
\[
\ell\left(\y,f(\x;\Vb,\W)\right)\geq 0.5.
\] 
Combining the latter with Markov inequality we arrive at
\[
\err{\W}\leq 2\E_{(\x,\y)\sim\Dc}[\ell(\y,f(\x;\Vb,\W))]=2\E[\Lc(\ell,\W)].
\]
Now since $\ell$ is $1$ Lipschitz and bounded, it obeys \eqref{ell pop bound}, which combined with the above identity yields \eqref{err pop bound}, completing the proof.
\end{proof}
%a fixed
\subsection{Proofs for neural nets with arbitrary initialization (Proof of Theorem \ref{nn deter gen})}
In this section we prove Theorem \ref{nn deter gen}. We first discuss a preliminary optimization result in Section \ref{prelimopt}. Next, in Section \ref{mainopt} we build upon this result to prove our main optimization result. Finally, in Section \ref{maingen} we use these optimization results to prove our main generalization result, completing the proof of Theorem \ref{nn deter gen}.
%Optimization and Generalization for
%%\[
%%\bar{\alpha}=\frac{\alpha}{\vrn B\opnorm{\X}}.
%%\]
\subsubsection{Preliminary Optimization Result}
\label{prelimopt}
\begin{lemma} [Deterministic convergence guarantee] \label{nn deter}Consider a one-hidden layer neural net of the form $\vct{x}\mapsto f(\vct{x};\mtx{W}):=\Vb\phi(\mtx{W}\vct{x})$ with input weights $\W\in\R^{k\times d}$ and output weights $\Vb\in\R^{K\times k}$ and an activation $\phi$ obeying $\abs{\phi(0)}\le B$, $\abs{\phi'(z)}\le B$, and $\abs{\phi''(z)}\le B$ for all $z$. Also assume $\Vb$ is fixed with all entries bounded by $\infnorm{\Vb}\le\frac{\vrn}{\sqrt{kK}}$ and we train over $\W$ based on the loss 
\begin{align*}
\mathcal{L}(\W)=\frac{1}{2}\sum_{i=1}^n\twonorm{f(\vct{x}_i;\W)-\y_i}^2.
\end{align*}
Also, consider a point $\W_0\in\R^{k\times d}$ with $\mtx{J}$ an $(\epsilon_0,\vrn B\|\X\|)$ reference Jacobian associated with $\mathcal{J}(\W_0)$ per Definition \ref{tjac}. Furthermore, define the information $\calF$ and nuisance $\calS$ subspaces and the truncated Jacobian $\mtx{J}_{\calF}$ associated with the reference Jacobian $\mtx{J}$ based on a cut-off spectrum value of $\alpha$ per Definition \ref{tjac2}. Let the initial residual vector be $\rb_0=\y-f(\W_0)\in\R^{n\K}$. Furthermore, assume
\begin{align}
\label{epsass}
 \eps_0\leq \frac{\alpha}{5}\min\left(\delta,\sqrt{\frac{\delta\alpha}{\Gamma\vrn B\|\X\|}}\right)
 \end{align}
and
\begin{align}
k\geq 400\frac{\vrn^6B^6\opnorm{\X}^6\Gamma^2}{\delta^2\alpha^8}\left(\upp+\delta\Gamma\tn{\rb_0}\right)^2,\label{fund k bound}
%k\geq \frac{64\Gamma^2B^2\|\X\|^2R^2}{B^2\delta^2\bar{\alpha}^6}.
\end{align}
with $0\le \delta\le1$ and $\Gamma\ge 1$. We run gradient descent iterations of the form $\W_{\tau+1}=\W_{\tau}-\eta\nabla \mathcal{L}(\W_\tau)$ starting from $\W_0$ with step size $\eta$ obeying $\eta\le \frac{1}{\vrn^2B^2\opnorm{\X}^2}$. Then for all iterates $\tau$ obeying $0\le \tau\le T:=\frac{\Gamma}{\eta\alpha^2}$
\begin{align}
\tf{\W_\tau-\W_0}\le& \frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}
.\label{main res eq22}\\
\trow{\W_{\tau}-\W_0}\le& \frac{ 2\vrn B\Gamma\opnorm{\X}}{\sqrt{k}\alpha^2}\tn{\rb_0}.\label{row boundsss}
\end{align}
Furthermore, after $\tau=T$ iteration we have
\begin{align}
\tn{\rb_{T}}\le  e^{-\Gamma}\tn{\Pi_{{\Rc}}(\rb_0)}+\tn{ \Pi_{\mathcal{N}}(\rb_0)}+ \frac{\delta\alpha}{\vrn B\opnorm{\X}}\tn{\rb_0}.\label{eqqq22}
\end{align}
\end{lemma}
\begin{proof} To prove this lemma we wish to apply Theorem \ref{many step thm}. We thus need to ensure that the assumptions of this theorem are satisfied. To do this note that by Lemma \ref{props lem} Assumption \ref{ass2} holds with $\beta=\vrn B\opnorm{\X}$. Furthermore, we pick $\eps=\frac{\delta\alpha^3}{5\Gamma \vrn^2 B^2\opnorm{\X}^2}=\frac{\delta\alpha^3}{5\Gamma \beta^2}$ which together with \eqref{epsass} guarantees \eqref{cndd} holds.   We now turn our attention to verifying Assumption \ref{ass3}. To this aim note that for all $\W\in\R^{k\times d}$ obeying
\begin{align*}
\fronorm{\W-\W_0}\le R:=2\left(\frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}\right)
\end{align*}
as long as \eqref{fund k bound} holds  by Lemma \ref{props lem} we have
\begin{align*}
\|\Jc(\W)-\Jc(\W_0)\|\le&B\sqrt{\K}\infnorm{\Vb}\opnorm{\mtx{X}}R\\
\le&\frac{\vrn}{\sqrt{k}} B\opnorm{\mtx{X}}R\\
=&\frac{\delta\alpha^3}{10\Gamma\vrn^2 B^2\opnorm{\X}^2}\frac{\frac{20\Gamma\vrn^3 B^3\opnorm{\X}^3}{\delta\alpha^4}\left(\upp+\delta\Gamma\tn{\rb_0}\right)}{\sqrt{k}}\\
\le&\frac{\delta\alpha^3}{10\Gamma\vrn^2 B^2\opnorm{\X}^2}\\
=&\frac{\eps}{2}.
\end{align*}
Thus, Assumption \ref{ass3} holds with $\fronorm{\W-\W_0}\le R:=2\left(\frac{\upp}{\alpha}+\delta\frac{\Gamma}{\alpha}\tn{\rb_0}\right)$. Now that we have verified that the assumptions of Theorem \ref{many step thm} hold so do its conclusions and thus \eqref{main res eq22} and \eqref{eqqq22} hold.

We now turn our attention to proving the row-wise bound \eqref{row boundsss}. To this aim let $\w_{\ell}^{(\tau)}$ denote the $\ell$th row of $\W_\tau$. Also note that 
\[
\grad{\w_\ell}=\text{$\ell$th row of }\text{mat}(\mathcal{J}(\mtx{W})^T\rb_\tau).
\]
Hence, using Lemma \ref{props lem} equation \eqref{rowbndm} we conclude that
\[
\tn{\grad{\w_{\ell}^{(\tau)}}}\le B\sqrt{K}\infnorm{\Vb}\opnorm{\X} \le \frac{\vrn B\opnorm{\X}}{\sqrt{k}}\tn{\rb_\tau}.
\]
Consequently, for any row $1\leq \ell\leq k$, we have
\begin{align}
\twonorm{\w_{\ell}^{(\tau)}-\w_{\ell}^{(0)}}\leq \eta \frac{\vrn B\opnorm{\X}}{\sqrt{k}}\sum_{t=0}^{\tau-1}\tn{\rb_t}.\label{roww bound}
\end{align}
To bound the right-hand side we use the triangular inequality combined with \eqref{rrr bound} and \eqref{eee bound} to conclude that
\begin{align}
\label{A7}
\eta \sum_{t=0}^{\tau-1}\tn{\rb_\tau}\le&\eta\sum_{t=0}^{\tau-1}\tn{\rbb_\tau}+\eta\sum_{t=0}^{\tau-1}\tn{\rb_\tau-\rbb_\tau}\nn\\
 \le&\frac{\Gamma}{\alpha^2}\tn{\rb_0}+\frac{2\Gamma^2(\eps\beta+\eps_0^2)}{\alpha^4} \tn{\rb_0}\nn\\
 =&\frac{2\Gamma (\eps_0^2+\eps\beta)+\alpha^2}{\alpha^4}\Gamma\tn{\rb_0}\nn\\
 \le& 2\frac{\Gamma}{\alpha^2}\tn{\rb_0},
\end{align}
where in the last inequality we used the fact that $\eps_0^2\le \frac{\alpha^2}{25\Gamma}$ per \eqref{epsass} and $\epsilon\beta=\frac{\delta\alpha^3}{5\Gamma \beta}\le \frac{\alpha^2}{5\Gamma}$ per our choice of $\epsilon$. Combining \eqref{roww bound} and \eqref{A7}, we obtain
\[
\twonorm{\w_{\ell}^{(\tau)}-\w_{\ell}^{(0)}}\leq \frac{ 2\vrn B\|\X\|\Gamma}{\sqrt{k}\alpha^2}\tn{\rb_0},
\]
completing the proof of \eqref{row boundsss} and the theorem.
\end{proof}
\subsubsection{Main Optimization Result}
\label{mainopt}
\begin{lemma} [Deterministic optimization guarantee] \label{nn deter3} Consider the setting and assumptions of Lemma \ref{nn deter}. Suppose $\tn{\rb_0}\leq C_r\sqrt{n}$ for some $C_r\geq 1$. Setting $\bar{\alpha}=\frac{\alpha}{\vrn B\|\X\|}$ and $\delta=\frac{\zeta}{C_r\bar{\alpha}\sqrt{n}}$, we have that if
\begin{align}
\label{epsassss}
 \eps_0\leq \frac{\alpha}{5}\min\left(\frac{\zeta}{C_r\bar{\alpha}\sqrt{n}},\sqrt{\frac{\zeta}{\Gamma C_r\sqrt{n}}}\right)
 \end{align}
and
\begin{align}
k\geq 800\frac{C_r^2\Gamma^4}{\delta^2\nu^2\bar{\alpha}^8\|\X\|^2}\left(n+\frac{\zeta^2}{\bar{\alpha}^2}\right),\label{fund k boundss}
%k\geq \frac{64\Gamma^2B^2\|\X\|^2R^2}{B^2\delta^2\bar{\alpha}^6}.
\end{align}
all gradient iterations obey
\begin{align}
\tf{\W_\tau-\W_0}\le& \dpp+\frac{\Gamma \zeta}{\alpha\bar{\alpha}}
.\label{main res eq22ss}\\
\trow{\W_{\tau}-\W_0}\le& \frac{ 2\Gamma}{\sqrt{k}\alpha\bar{\alpha}}\tn{\rb_0}.\label{row boundsssss}
\end{align}
Furthermore, after $\tau=T$ iteration we have
\begin{align}
\tn{\rb_{T}}\le  e^{-\Gamma}\tn{\Pi_{{\Rc}}(\rb_0)}+\tn{ \Pi_{\mathcal{N}}(\rb_0)}+ \zeta.\label{eqqq22ss}
\end{align}
\end{lemma}
\begin{proof} Observe that $\delta\tn{\rb_0}\leq\zeta/\bar{\alpha}$ and $\upp\leq \Gamma \tn{\rb_0}\leq \Gamma C_r\sqrt{n}$. Substituting the proposed $\zeta$ choice we find
\[
\frac{\alpha}{5}\min\left(\delta,\sqrt{\frac{\delta\alpha}{\Gamma\nu B\|\X\|}}\right)=\frac{\alpha}{5}\min\left(\frac{\zeta}{C_r\bar{\alpha}\sqrt{n}},\sqrt{\frac{\zeta}{\Gamma C_r\sqrt{n}}}\right).
\]
and
\begin{align}
\frac{\vrn^6B^6\opnorm{\X}^6\Gamma^2}{\delta^2\alpha^8}\left(\upp+\delta\Gamma\tn{\rb_0}\right)^2&\leq \frac{\Gamma^2}{\delta^2\bar{\alpha}^6\alpha^2}\left(\upp+\delta\Gamma\tn{\rb_0}\right)^2\\
&\leq \frac{2\Gamma^4}{\delta^2\bar{\alpha}^6\alpha^2}\left(C_r^2n+\frac{\zeta^2}{\bar{\alpha}^2}\right)\\
&\leq \frac{2C_r^2\Gamma^4}{\delta^2\nu^2\bar{\alpha}^8\|\X\|^2}\left(n+\frac{\zeta^2}{\bar{\alpha}^2}\right)
\end{align}
and
\[
\delta\frac{\Gamma}{\alpha}\tn{\rb_0}\leq \frac{\Gamma \zeta}{\alpha\bar{\alpha}}
\]
and
\[
\frac{\delta\alpha}{\vrn B\opnorm{\X}}\tn{\rb_0}\leq \zeta.
\]
\end{proof}

\subsubsection{Main generalization result (completing the proof of Theorem \ref{nn deter gen})}\label{maingen}
Theorem \ref{nn deter gen} immediately follows from Theorem \ref{nn deter gennn} below by upper bounding $\dpp$ (see Definition \ref{earlyval}) using Lemma \ref{bndearlystopval} equation \eqref{upp up bound}.
\begin{theorem}\label{nn deter gennn}
Consider a training data set $\{(\x_i,\y_i)\}_{i=1}^n\in\R^d\times \R^K$ generated i.i.d.~according to a distribution $\Dc$ where the input samples have unit Euclidean norm. Also consider a neural net with $k$ hidden layers as described in \eqref{neural net func} parameterized by $\W$ where the activation function $\phi$ obeys $\abs{\phi'(z)}, \abs{\phi''(z)}\le B$. Let $\W_0$ be the initial weight matrix with i.i.d.~$\Nn(0,1)$ entries. Also assume the output matrix has bounded entries obeying $\infnorm{\mtx{V}}\le \frac{\vrn}{\sqrt{kK}}$. Furthermore, set $\mtx{J}:=\mathcal{J}(\W_0)$ and define the information $\calF$ and nuisance $\calS$ subspaces and the truncated Jacobian $\mtx{J}_{\calF}$ associated with the reference/initial Jacobian $\mtx{J}$ based on a cut-off spectrum value $\alpha=\vrn B \bar{\alpha} \sqrt[4]{n}\sqrt{\opnorm{\X}}$. Also define the initial residual $\rb_0=f(\W_0)-\y\in\R^{nK}$ and pick $C_r>0$ so that $\frac{\tn{\rb_0}}{\sqrt{n}}\le C_r$. Also assume the cut-off level $\alpha$ is selected so that the information space is large enough to guarantee $ \tn{\Pi_{\Rc}(\rb_0)}\geq c\tn{\rb_0}$ for some constant $c>0$. Also assume, the number of hidden nodes $k$ obeys%Suppose the initial residual and the number of hidden nodes satisfy
%=\sigma \bar{\alpha}B\|\X\|
\begin{align}
 k\ge25600 \frac{C_r^2\Gamma^4}{\bar{\alpha}^8\vrn^2B^2\zeta^2},\label{k bound det gen}
\end{align}
with $\Gamma\ge 1$ and tolerance level $\zeta\le 2$.
%%
%%
%%
%%Let the initial residual vector be $\rb_0=\y-f(\W_0)\in\R^{n\K}$ and let $C_r>0$ be a number satisfying $\tn{\rb_0}\leq C_r\sqrt{n}$. Also pick the information space large enough to guarantee $ \tn{\Pi_{\Rc}(\rb_0)}\geq c\tn{\rb_0}$ for some constant $c>0$. Set $\bar{\alpha}=\frac{\alpha}{\sigma B \sqrt[4]{n}\sqrt{\opnorm{\X}}\|\X\|}$ and assume number of hidden nodes $k$ obeys%Suppose the initial residual and the number of hidden nodes satisfy
%%%=\sigma \bar{\alpha}B\|\X\|
%%\begin{align}
%% k\gtrsim\frac{C_r^2\Gamma^4}{\bar{\alpha}^8\vrn^2\zeta^2}.\label{k bound det gen}
%%\end{align}
%Set $\eta\leq \frac{1}{\vrn^2B^2\|\X\|^2}$ and fix $\Gamma\geq 1$. 
Run gradient descent updates \eqref{grad dec me} with learning rate $\eta\le \frac{1}{\vrn^2B^2\opnorm{\X}^2}$. Then, after $T=\frac{\Gamma }{\eta\alpha^2}$ iterations, with probability at least $1-\delta$, the generalization error obeys
\begin{align}% \frac{\tn{ \Pi_{\bar{\Rc}}(\y)}+ \exp(-\Gamma)\tn{\Pi_{{\Rc}}(\y)}+\dpz}{\sqrt{n}}+\zeta\approx  
\err{\W_{T}}&\leq \underbrace{\frac{2\tn{ \Pi_{\mathcal{N}}(\rb_0)}}{\sqrt{n}}}_{bias~term}+\underbrace{\frac{12\vrn B \dpp}{\sqrt{n}}}_{variance~term}+5\sqrt{\frac{\log(2/\delta)}{n}}+2C_r(e^{-\Gamma}+\zeta),
\end{align}
where $\dpp$ is the early stopping distance as in Def. \eqref{earlyval}.
\end{theorem}
%%%\begin{theorem} \label{nn deter gennn}Let $(\x_i,\y_i)_{i=1}^n\distas \Dc$ be a dataset where inputs have unit Euclidian norm. Consider a neural net with $k$ hidden layers as described in \eqref{neural net func} and parameterized by $\bteta:=\text{vect}(\W)$. Let $\W_0$ be the initialization. Suppose $|\phi(0)|,|\phi'|,|\phi''|\leq B$. Let output matrix $\Vb$ be such that $\tin{\Vb}\leq \frac{\vrn}{\sqrt{\K k}}$. Let $\sigma B\|\X\|\geq \alpha>0$ be the cutoff level and $\zeta>0$ be the error tolerance. Fix fast and slow subspaces $\Rc$ and $\Rcb$ with respect to initial Jacobian $\Jc(\W_0)$ with cutoff $\alpha$. Let the initial residual vector be $\rb_0=\y-f(\W_0)\in\R^{n\K}$ and let $C_r>0$ be a number satisfying $\tn{\rb_0}\leq C_r\sqrt{n}$. Also pick the information space large enough to guarantee $ \tn{\Pi_{\Rc}(\rb_0)}\geq c\tn{\rb_0}$ for some constant $c>0$. Set $\bar{\alpha}=\frac{\alpha}{\sigma B \|\X\|}$ and assume number of hidden nodes $k$ obeys%Suppose the initial residual and the number of hidden nodes satisfy
%%%%=\sigma \bar{\alpha}B\|\X\|
%%%\begin{align}
%%% k\gtrsim\frac{C_r^2\Gamma^4n^2}{\|\X\|^4\bar{\alpha}^8\vrn^2\zeta^2}.\label{k bound det gen}
%%%\end{align}
%%%Set $\eta\leq \frac{1}{\vrn^2B^2\|\X\|^2}$ and fix $\Gamma\geq 1$. After $\tau_0=\frac{\Gamma}{\eta\alpha^2}$, iterations, with probability $1-\delta$, the classification error 
%%%\begin{align}
%%%\err{\W}=\Pro(\arg\max_{1\leq i\leq K}\y_i\neq \arg\max_{1\leq i\leq K}f_i(\x,\W))\label{class error2}
%%%\end{align}
%%%satisfies
%%%\begin{align}% \frac{\tn{ \Pi_{\bar{\Rc}}(\y)}+ \exp(-\Gamma)\tn{\Pi_{{\Rc}}(\y)}+\dpz}{\sqrt{n}}+\zeta\approx  
%%%\err{\W_{\tau_0}}&\leq \underbrace{\frac{2\tn{ \Pi_{\bar{\Rc}}(\rb_0)}}{\sqrt{n}}}_{bias~term}+\underbrace{\frac{12\vrn B \dpp}{\sqrt{n}}}_{variance~term}+5\sqrt{\frac{\log(2/\delta)}{n}}+2C_r(\exp(-\Gamma)+\zeta),
%%%\end{align}
%%%where $\dpp$ is the early stopping distance as in Def. \eqref{earlyval}.
%%%\end{theorem}
\begin{proof}
%First, we plug $\alpha$ in \eqref{k condition} of Theorem \ref{apply 1} to obtain
%\[
%k\geq \order{\frac{\Gamma^4 \vrn^6n^2\|\X\|^4\log^2(2n)}{\alpha^8}}.
%\]
First, note that using $\alpha\le \beta=\vrn B\opnorm{\X}$, $\frac{\upp}{\Gamma}\le \twonorm{\rb_0}$ per \eqref{upp up bound}, and $\tn{\rb_0}\leq  C_r\sqrt{n}$ we have
\begin{align*}
\frac{\alpha}{ \vrn B\|\X\|}\leq1\leq  \frac{\Gamma \tn{\rb_0}}{\upp}\leq C_r \frac{\Gamma\sqrt{n}}{\upp}. 
\end{align*}
This together with $\zeta\le 2$ implies that 
\begin{align}\label{temp521}
\frac{\alpha}{\frac{\zeta}{2}\vrn B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\le&\frac{\alpha}{\frac{\zeta}{2}\vrn B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\frac{\zeta}{2}\upp}\nn\\
\le&2\frac{\Gamma \tn{\rb_0}}{\frac{\zeta}{2}\upp}\nn\\
\le&2\frac{C_r}{\frac{\zeta}{2}}\frac{\Gamma}{\upp}\sqrt{n}.
\end{align}
Thus when
\begin{align*}
k\ge&25600 \frac{C_r^2\Gamma^4}{\bar{\alpha}^8\vrn^2B^2\zeta^2}\\\
=&6400 \left(\frac{C_r\Gamma}{\frac{\zeta}{2}}\right)^2\frac{n^2\Gamma^2\vrn^6B^6\opnorm{\X}^4}{\alpha^8}\\
\overset{\sqrt{n}\ge\|\X\|}{\ge}&6400 \left(\frac{C_r\Gamma}{\frac{\zeta}{2}}\right)^2\frac{n\vrn^6B^6\opnorm{\X}^6}{\alpha^8}\\
=& 1600 \left(2\frac{C_r}{\frac{\zeta}{2}}\frac{\Gamma}{\upp}\sqrt{n}\right)^2\frac{\upp^2\vrn^6B^6\opnorm{\X}^6}{\alpha^8}\\
\overset{\eqref{temp521}}{\ge}&1600\left(\frac{\alpha}{\frac{\zeta}{2}\vrn B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{\upp^2\vrn^6B^6\opnorm{\X}^6}{\alpha^8}
\end{align*}
Thus, \eqref{k bound det} holds. Also \eqref{ref bound eps} trivially holds for $\eps_0$. Thus applying Theorem \ref{nn deter2} with $\eps_0=0$ the following three conclusions hold
\begin{align}
%\frac{\alpha_0\tn{\rb_0}}{B\sqrt{K}\|\X\|},
&\tf{\W_\tau-\W_0}\leq \frac{2\upp}{\alpha}=2\dpp.\label{frott51}
\end{align}
and
\begin{align}
\trow{\W_{\tau}-\W_0}\le& \frac{ 2\vrn B\Gamma\opnorm{\X}}{\sqrt{k} \alpha^2} \tn{\rb_0}\nn\\
\overset{\tn{\rb_0}\le C_r\sqrt{n}}{\le}&\frac{ 2\sqrt{n}C_r\vrn B\Gamma\opnorm{\X}}{\sqrt{k} \alpha^2}.
%\le& \frac{ 2\sqrt{n}C_r\sigma B\Gamma\opnorm{\X}}{\sqrt[4]{k} \alpha^2}
\label{rowtt521}
\end{align}
and 
\begin{align}
\label{tt521}
\twonorm{f(\W_T)-\y}\le&  e^{-\Gamma}\tn{\Pi_{{\Rc}}(\rb_0)}+\tn{ \Pi_{\mathcal{N}}(\rb_0)}+\frac{\zeta}{2}\tn{\rb_0}\nn\\
\le&  \tn{ \Pi_{\mathcal{N}}(\rb_0)}+\left(e^{-\Gamma}+\frac{\zeta}{2}\right)\tn{\rb_0}\nn\\
\overset{\tn{\rb_0}\le C_r\sqrt{n}}{\le}&  \tn{ \Pi_{\mathcal{N}}(\rb_0)}+C_r\left(e^{-\Gamma}+\frac{\zeta}{2}\right)\sqrt{n}.
\end{align}
Furthermore, using the assumption that $\infnorm{\Vb}\le \frac{\vrn}{\sqrt{kK}}$ Lemma \ref{generalize corollary} applies and hence equation \eqref{err pop bound} with $\W=\W_T$, $\sqrt{\mathcal{L}(\W_T)}=\frac{\twonorm{f(\W_T)-\y}}{\sqrt{n}}$, $M_{\mathcal{W}}=2\dpp$, $M_{\mathcal{V}}=0$, and $R=\frac{2\sqrt{n}C_r\vrn B\Gamma\opnorm{\X}}{\alpha^2}$ implies that
\begin{align}
\label{temperr}
\err{\W_T}\leq 2\left[\frac{\twonorm{f(\W_T)-\y}}{\sqrt{n}}+3\vrn B\left(\frac{2\dpp}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}\right)+\sqrt{\frac{5\log(2/\delta)}{n}}\right]
\end{align}
Also note that using \eqref{k bound det gen} we have
\begin{align}
\label{R2k}
\frac{3\vrn B R^2}{\sqrt{k}}\leq \frac{ 12C_r^2\Gamma^2 \vrn^3 B^3n\|\X\|^2}{\sqrt{k}\alpha^4}\leq C_r\frac{\zeta}{2}% \frac{\zeta\alpha_0^2}{B}\leq \zeta.% \order{\frac{1}{\sigma} C\frac{\zeta^2}{B\log(2n)}}\leq \zeta.
\end{align}
Plugging \eqref{tt521} and \eqref{R2k} into \eqref{temperr} completes the proof.
\end{proof}
\subsection{Proofs for neural network with random initialization (proof of Theorem \ref{gen main})}
In this section we prove Theorem \ref{gen main}. We first discuss and prove an optimization result in Section \ref{mainopt22}. Next, in Section \ref{comp22} we build upon this result to complete the proof of Theorem \ref{gen main}.

\subsubsection{Optimization result}
\label{mainopt22}
%Suppose label vector $\y$ has $\ell_2$ norm $\sqrt{n}$. This is without loss of generality. In particular, under one-hot encoding each label would have unit Euclidian norm.
\begin{theorem} [Optimization guarantee for random initialization]\label{apply 1} Consider a training data set $\{(\x_i,\y_i)\}_{i=1}^n\in\R^d\times \R^K$ generated i.i.d.~according to a distribution $\Dc$ where the input samples have unit Euclidean norm and the concatenated label vector obeys $\tn{\y}=\sqrt{n}$ (e.g.~one-hot encoding). Consider a neural net with $k$ hidden layers as described in \eqref{neural net func} parameterized by $\W$ where the activation function $\phi$ obeys $\abs{\phi'(z)}, \abs{\phi''(z)}\le B$. Let $\W_0$ be the initial weight matrix with i.i.d.~$\Nn(0,1)$ entries. Fix a precision level $\zeta$ and set 
\begin{align}
\vrn=\frac{\zeta}{50B\sqrt{\log(2\K)}}.\label{simplified cond}
\end{align}
Also assume the output layer $\Vb$ has i.i.d.~Rademacher entries scaled by $\frac{\vrn}{\sqrt{k\K}}$. Furthermore, set $\mtx{J}:=(\Iden_\K \otimes \bSi(\X))^{1/2}$ and define the information $\calF$ and nuisance $\calS$ spaces and the truncated Jacobian $\mtx{J}_{\calF}$ associated with the reference Jacobian $\mtx{J}$ based on a cut-off spectrum value of $\alpha_0=\bar{\alpha}\sqrt[4]{n}\sqrt{K\opnorm{\X}}B\le B\sqrt{K}\opnorm{\X}$ per Definition \ref{tjac neural} so as to ensure $\twonorm{\Pi_{\calF}(\y)}\ge c\twonorm{\y}$ for some constant $c$. Assume\vspace{-6pt}
\begin{align}
\label{k condition}
k\ge 12\times 10^7\frac{\Gamma^4\K^4B^8\|\X\|^6n\log^2(2n)}{c^4\zeta^4\alpha_0^8}
\end{align}
with $\Gamma\ge 1$ and $\zeta\le \frac{c}{2}$. We run gradient descent iterations of the form \eqref{grad dec me} with a learning rate $\eta\le \frac{1}{\vrn^2B^2\opnorm{\X}^2}$. Then, after $T=\frac{\Gamma K}{\eta\vrn^2\alpha_0^2}$ iterations, the following identities 
\begin{align}
&\tn{f(\W_{\tau_0})-\y}\leq  \tn{ \Pi_{\Rcb}(\y)}+ \e^{-\Gamma}\tn{\Pi_{{\Rc}}(\y)}+4\zeta\sqrt{n},\label{eqqq24}\\%\frac{4\sqrt{n}\alpha_0}{B\sqrt{K}\|\X\|},
&\tn{\W_\tau-\W_0}\leq \frac{2\sqrt{\K}(\upz(\y)+\Gamma\zeta \sqrt{n})}{\vrn\alpha_0},\label{main res eq24}\\
&\trow{\W_{\tau}-\W_0}\leq \frac{4\Gamma B\K \|\X\|}{\vrn\alpha_0^2}\sqrt{\frac{n}{k}},\label{row boundsss3}
\end{align}
hold with probability at least $1-(2\K)^{-100}$.
\end{theorem}
\begin{proof} To prove this result we wish to apply Theorem \ref{nn deter2}. To do this we need to verify the assumptions of this theorem. To start with, using Lemma \ref{upresz} with probability at least $1-(2\K)^{-100}$, the initial prediction vector $f(\W_0)$ obeys
\begin{align}
\tn{f(\W_0)}\leq \zeta\tn{\y}=\zeta\sqrt{n}\leq \frac{\sqrt{n}}{2}.\label{y diff diff}%50B\sqrt{\log(2\K)}\vrn
\end{align}
Hence the initial residual obeys $\tn{\rb_0}\leq 2\sqrt{n}$. Furthermore, using $\zeta\leq c/2$
\begin{align}
\tn{\rb_0-\y}\le& \zeta \tn{\y}\implies \tn{\Pi_{\Rc}(\rb_0-\y)}\le \zeta \tn{\y}.
\end{align}
Thus,
\begin{align}
\tn{\Pi_{\Rc}(\rb_0)}\ge&\tn{\Pi_{\Rc}(\y)}-\tn{\Pi_{\Rc}(\rb_0-\y)}\nn\\
\ge&\tn{\Pi_{\Rc}(\y)}-\zeta\tn{\y}\nn\\
\ge&\left(c-\zeta\right)\tn{\y}\nn\\
\ge&\frac{c}{2}\tn{\y}\label{penult}\\
\ge&\frac{c}{4}\tn{\rb_0}.\label{lastbri}
 %\tn{\Pi_{\Rc}(\y)}/2\geq (c/4)  \tn{\rb_0}.\label{r y perturb}%\tn{\Pi_{\Rcb}(\rb_0-\y)}\leq \zeta \tn{\y}.
\end{align}
Thus the assumption on the ratio of information to totally energy of residual holds and we can replace $c$ with $\frac{c}{4}$ in Theorem \ref{nn deter2}. Furthermore, since $\upz(\cdot)$ is $\Gamma$-Lipschitz function of its input vector in $\ell_2$ norm hence we also have
\begin{align}
\upz(\rb_0)\leq \upz(\y) +\Gamma\tn{\rb_0-y}\leq \upz(\y) +\Gamma \zeta\tn{\y}.\label{upp lip}
\end{align}
%Since $\zeta\leq \frac{\upz(\y)}{\Gamma\tn{\y}}\leq 1$, we have $\upz(\rb_0)\leq 2\upz(\y)$.
%To proceed we will plug $\zeta=\frac{\sigma}{50B\sqrt{\log(2\K)}}$ in Theorem \ref{nn deter2}.
Next we wish to show that \eqref{ref bound eps} holds. In particular we will show that there exists an $\eps_0$-reference Jacobian $\Jb$ for $\Jc(\W_0)$ satisfying $\Jb\Jb^T=\E[\Jc(\W_0)\Jc(\W_0)^T]$. Note that, such a $\Jb$ will have exactly same information/nuisance spaces as the square-root of the multiclass kernel matrix i.e.~$\left(\E[\Jc(\W_0)\Jc(\W_0)^T]\right)^{\frac{1}{2}}$ since these subspaces are governed by the left eigenvectors. Applying Lemmas \ref{minspectJ} (with a scaling of the Jacobian by $1/\sqrt{kK}$ due to the different scaling of $\V$), we find that if 
\begin{align}
k\geq \frac{1000\K^2B^4\|\X\|^4\log^2(2n)}{\delta^2}\label{kk bound}
\end{align}
then,\vspace{-23pt}
\begin{align}
\opnorm{\Jc(\W_0)\Jc(\W_0)^T-\E[\Jc(\W_0)\Jc(\W_0)^T]}\leq \frac{\delta\vrn^2}{K}.\label{ref jac}
\end{align}
Let $\Jcb(\W)$ obtained by zero-padding last $\max(\K n-p,0)$ columns of $\Jc(\W)$. Then, using \eqref{ref jac} and Lemma \ref{psd pert}, there exists $\Jb$ satisfying $\Jb\Jb^T=\E[\Jc(\W_0)\Jc(\W_0)^T]$ and\vspace{-5pt}
\begin{align*}
%&\sigma_{\min}\left(\mathcal{J}(\W_0)\right)\ge \frac{1}{\sqrt{2}}\twonorm{\vct{v}}\sqrt{\lambda(\X)},\\
\opnorm{\Jcb(\W_0)-\Jb}\le 2\sqrt{\frac{\delta\vrn^2}{K}}.
\end{align*}
Therefore, $\Jb$ is an $\eps_0^2=4\frac{\delta\vrn^2}{K}$ reference Jacobian. Now set
\[
\Theta=\min\left(c\frac{\upz\alpha_0}{B\Gamma^2\opnorm{\X}\sqrt{nK}},\left(\frac{\zeta B\sqrt{K}\opnorm{\X}}{\alpha_0}\right)^2,\frac{\zeta}{\Gamma}\right)
\]
and note that using $\alpha=\frac{\vrn}{\sqrt{k}}\alpha_0$ and $\tn{\rb_0}\le 2\sqrt{n}$
\begin{align}
\label{tt2}
\Theta=&\min\left(c\frac{\upz\alpha_0}{B\Gamma^2\opnorm{\X}\sqrt{nK}},\left(\frac{\zeta B\sqrt{K}\opnorm{\X}}{\alpha_0}\right)^2,\frac{\zeta}{\Gamma}\right)\nn\\
=&\min\left(c\frac{\upz\alpha}{\vrn B\Gamma^2\opnorm{\X}\sqrt{n}},\left(\frac{\vrn\zeta B\opnorm{\X}}{\alpha}\right)^2,\frac{\zeta}{\Gamma}\right)\nn\\
\le&2\cdot\min\left(c\frac{\upp\alpha}{\vrn B\Gamma^2\tn{\rb_0}\opnorm{\X}},\frac{\zeta^2\vrn^2 B^2\opnorm{\X}^2}{\alpha^2},\frac{\zeta}{\Gamma}\right)
\end{align}
To continue further, note that $\upz$ calculated with respect to $(\Iden_\K \otimes \bSi(\X))^{1/2}$ with cutoff $\alpha_0$ is exactly same as $\upp$ calculated with respect to $\Jb$ with cutoff $\alpha=\frac{\vrn \alpha_0}{\sqrt{\K}}$ which is a square-root of $\E[\Jc(\W_0)\Jc(\W_0)^T]$. Thus, using \eqref{tt2} to ensure \eqref{ref bound eps} holds it suffices to show
\[
\eps_0^2=4\frac{\delta\vrn^2}{\K}\leq  \frac{\alpha^2}{25}\frac{\Theta}{2}=\frac{\vrn^2\alpha_0^2}{50\K}\Theta.%\min(\frac{\upz^2}{\tn{\rb_0}^2},\frac{\zeta}{\Gamma})%\iff \delta\leq \frac{\sigma^2\alpha_0^2}{400\tf{\Vb}^2}\min(\frac{\upz^2}{\tn{\y}^2},\frac{\zeta}{\Gamma})% \frac{\alpha_0^3\upz{\sigma}^2 }{200\Gamma^2B\K^{1/2} \|\X\|\tn{\y}\tf{\Vb}^2}.
\]
Hence, to ensure \eqref{ref bound eps} holds we need to ensure that $\delta$ obeys%reference Jacobian $\Jb$. Substituting, this yields
\[
\delta\leq \frac{\alpha_0^2}{200}\Theta.%\frac{B\alpha_0^3\upz }{400\Gamma^2\K^{1/2} \|\X\|\tn{\y}}.
\]
Thus using $\delta=\frac{\alpha_0^2}{200}\Theta$ to ensure \eqref{ref bound eps} we need to make sure $k$ is sufficiently large so that \eqref{kk bound} holds with this value of $\delta$. Thus it suffices to have
\begin{align}
k\ge&12\times 10^7\frac{\Gamma^4\K^4B^8\|\X\|^6n\log^2(2n)}{c^4\zeta^4\alpha_0^8}\label{k1}\\
\ge&12\times 10^7\frac{\Gamma^4\K^4B^8\|\X\|^8\log^2(2n)}{c^4\zeta^4\alpha_0^8}\nn\\
\ge&4\times 10^7\cdot\left(\frac{4K^2B^4\Gamma^4\opnorm{\X}^4}{c^4\alpha_0^4}+\frac{1}{\zeta^4 }+\frac{\Gamma^2}{\zeta^2}\right)\frac{\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4}\nn\\
\ge&4\times 10^7\cdot\left(\frac{4KB^4\Gamma^4\opnorm{\X}^4}{c^4\alpha_0^4}+\frac{1}{\zeta^4 }+\frac{\Gamma^2}{\zeta^2}\right)\frac{\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4}\nn\\
\ge&4\times 10^7\cdot\left(\frac{4KB^4\Gamma^4\opnorm{\X}^4}{c^4\alpha_0^4}+\frac{\alpha_0^4}{\zeta^4 B^4K^2\opnorm{\X}^4}+\frac{\Gamma^2}{\zeta^2}\right)\frac{\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4}\nn\\
\overset{(a)}{\ge}&4\times 10^7\cdot\left(\frac{nKB^2\Gamma^4\opnorm{\X}^2}{c^2\upz^2\alpha_0^2}+\frac{\alpha_0^4}{\zeta^4 B^4K^2\opnorm{\X}^4}+\frac{\Gamma^2}{\zeta^2}\right)\frac{\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4}\nn\\
\ge&4\times 10^7\cdot\max\left(\frac{nKB^2\Gamma^4\opnorm{\X}^2}{c^2\upz^2\alpha_0^2},\frac{\alpha_0^4}{\zeta^4 B^4K^2\opnorm{\X}^4},\frac{\Gamma^2}{\zeta^2}\right)\frac{\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4}\nn\\
=&4\times 10^7\frac{\cdot\K^2B^4\|\X\|^4\log^2(2n)}{\alpha_0^4\cdot\min\left(\left(\frac{c\upz\alpha_0}{B\Gamma^2\opnorm{\X}\sqrt{nK}}\right)^2,\left(\frac{\zeta B\sqrt{K}\opnorm{\X}}{\alpha_0}\right)^4,\frac{\zeta^2}{\Gamma^2}\right)}\nn\\
=&\frac{1000\K^2B^4\|\X\|^4\log^2(2n)}{\delta^2}
\label{kreq11}
\end{align}
Here, (a) follows from the fact that $\| \bSi(\X)^{1/2}\|:=\la_1\leq B\|\X\|$,  equation \eqref{low bound}, and $\twonorm{\Pi_{\mathcal{I}}(\vct{r}_0)}\ge \frac{c}{2}\twonorm{\y}=\frac{c}{2}\sqrt{n}$ which combined imply
\begin{align}
\label{bri}
\upz\ge \frac{\alpha}{\lambda_1}\twonorm{\Pi_{\mathcal{I}}(\rb_0)}\ge \frac{\alpha}{B\opnorm{\X}}\twonorm{\Pi_{\mathcal{I}}(\rb_0)}\geq \frac{\alpha_0c}{2}\frac{\twonorm{\y}}{B\|\X\|}=\frac{\alpha_0c}{2}\frac{\sqrt{n}}{B\|\X\|}.
\end{align}
To be able to apply Theorem \ref{nn deter2} we must also ensure \eqref{k bound det} holds. Therefore, it suffices to have
\begin{align}
k\ge&64\times10^6\frac{K^4B^8\opnorm{\X}^6\Gamma^4n\log^2(2n)}{\zeta^4\alpha_0^8}\\\overset{(a)}{\ge}&25600\frac{K^4B^6\opnorm{\X}^6\Gamma^4n}{\zeta^2\vrn^2\alpha_0^8}\label{k2}\\
k\ge&12800\left(\frac{\alpha_0^2}{\zeta^2B^2K\opnorm{\X}^2}+1\right)\frac{K^4B^6\opnorm{\X}^6\Gamma^4n}{\vrn^2\alpha_0^8}\nn\\
\overset{(b)}{\ge}&3200\left(\frac{\alpha_0^2}{\zeta^2B^2K\opnorm{\X}^2}+\frac{4\Gamma^2 n}{\upp^2}\right)\frac{K^4B^6\opnorm{\X}^6\Gamma^2\upp^2}{\vrn^2\alpha_0^8}\nn\\
\ge&3200\left(\frac{\alpha_0^2}{\zeta^2B^2K\opnorm{\X}^2}+\frac{\Gamma^2 \tn{\rb_0}^2}{\upp^2}\right)\frac{K^4B^6\opnorm{\X}^6\Gamma^2\upp^2}{\vrn^2\alpha_0^8}\nn\\
\ge&1600\left(\frac{\alpha_0}{\zeta\sqrt{K} B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{K^4B^6\opnorm{\X}^6\Gamma^2\upp^2}{\vrn^2\alpha_0^8}\nn\\
=&1600\left(\frac{\alpha}{\zeta\vrn B\opnorm{\X}}+\frac{\Gamma \tn{\rb_0}}{\upp}\right)^2\frac{\vrn^6B^6\opnorm{\X}^6\Gamma^2\upp^2}{\alpha^8}
\end{align}
Here, (a) follows from the fact that $n\ge K$ and the relationship between $\zeta$ and $\vrn$ per \eqref{simplified cond} and (b) follows from the fact that per equation \eqref{upp up bound} we have
\begin{align*}
\upp\le \Gamma\twonorm{\rb_0}\le 2\Gamma\sqrt{n}
\end{align*}
Note that \eqref{k1} and \eqref{k2} are implied by
\begin{align}
k\ge12\times 10^7\frac{\Gamma^4\K^4B^8\|\X\|^6n\log^2(2n)}{c^4\zeta^4\alpha_0^8},\label{kreq2}
\end{align}
which is the same as \eqref{k condition}. What remains is stating the optimization bounds in terms of the labels $\y$. This follows by substituting \eqref{y diff diff}, \eqref{upp lip}, and the fact that $\twonorm{\rb_0}\le 2\sqrt{n}$ into \eqref{eqqq23}, \eqref{main res eq23}, and \eqref{row boundsss2}, respectively.
\end{proof}


\subsubsection{Generalization result (completing the proof of Theorem \ref{gen main})}
\label{comp22}%a change of variable on $\bar{\alpha}$ (uses $\bar{\alpha}=\frac{\alpha_0}{\sqrt{\K} B\|\X\|}$) and 
Theorem below is a restatement of Theorem \ref{gen main} after substituting the upper bound on the early stopping distance $\dpz$ of Def. \eqref{earlyval}.
\begin{theorem} [Neural Net -- Generalization] \label{gen mainnn}
Consider a training data set $\{(\x_i,\y_i)\}_{i=1}^n\in\R^d\times \R^K$ generated i.i.d.~according to a distribution $\Dc$ where the input samples have unit Euclidean norm and the concatenated label vector obeys $\tn{\y}=\sqrt{n}$ (e.g.~one-hot encoding). Consider a neural net with $k$ hidden layers as described in \eqref{neural net func} parameterized by $\W$ where the activation function $\phi$ obeys $\abs{\phi'(z)}, \abs{\phi''(z)}\le B$. Let $\W_0$ be the initial weight matrix with i.i.d.~$\Nn(0,1)$ entries. Fix a precision level $\zeta\le \frac{c}{2}$ and set 
\begin{align}
\vrn=\frac{\zeta}{50B\sqrt{\log(2\K)}}.\label{simplified cond}
\end{align}
Also assume the output layer $\Vb$ has i.i.d.~Rademacher entries scaled by $\frac{\vrn}{\sqrt{k\K}}$. Furthermore, set $\mtx{J}:=(\Iden_\K \otimes \bSi(\X))^{1/2}$ and define the information $\calF$ and nuisance $\calS$ spaces and the truncated Jacobian $\mtx{J}_{\calF}$ associated with the Jacobian $\mtx{J}$ based on a cut-off spectrum value of $\alpha_0=\bar{\alpha}\sqrt[4]{n}\sqrt{K\opnorm{\X}}B \leq B\|\X\|$ per Definition \ref{tjac neural} chosen to ensure $\tn{\Pi_{\Ic}(\y)}\geq c\tn{\y}$ for some constant $c>0$. Assume\vspace{-6pt}
\begin{align}
\label{hidnum}
k\ge 12\times 10^7\frac{\Gamma^4\K^4B^8\|\X\|^4n^2\log^2(2n)}{c^4\zeta^4\alpha_0^8}
\end{align}
with $\Gamma\ge 1$. We run gradient descent iterations of the form \eqref{grad dec me} with a learning rate $\eta\le \frac{1}{\vrn^2B^2\opnorm{\X}^2}$. Then, after $T=\frac{\Gamma K}{\eta\vrn^2\alpha_0^2}$ iterations, classification error $\err{\W_{T}}$ is upper bounded by \vspace{-6pt}
\[
\err{\W_T}\le 2\frac{\tn{ \Pi_{\Rcb}(\y)}+e^{-\Gamma}\twonorm{\Pi_{\mathcal{I}}(\y)}}{\sqrt{n}}+\frac{12B\sqrt{\K}}{\sqrt{n}}\dpz+12\Big(1+\frac{\Gamma}{\bar{\alpha}\sqrt[4]{n\|\X\|^2}}\Big)\zeta+10\sqrt{\frac{\log(2/\delta)}{n}},
\]
holds with probability at least $1-(2\K)^{-100}-\delta$.
\end{theorem}
\begin{proof}
Under the stated assumptions, Theorem \ref{apply 1} holds with probability $1-(2\K)^{-100}$. The proof will condition on outcomes of the Theorem \ref{apply 1}. Specifically, we shall apply \eqref{err pop bound} of Lemma \ref{generalize corollary} with $M_{\mathcal{W}}$ and $R$ dictated by Theorem \ref{apply 1} where the output layer $\Vb$ is fixed. Observe that $\tf{\Vb}=\sqrt{\K k}\tin{\Vb}=\vrn$, we have
\begin{align}
\label{tempkillme}
\err{\W_T}\leq 2\left[\frac{\twonorm{f(\W_T)-\y}}{\sqrt{n}}+3\vrn B\left(\frac{M_{\mathcal{W}}}{\sqrt{n}}+\frac{R^2}{\sqrt{k}}\right)+\sqrt{\frac{5\log(2/\delta)}{n}}\right].
\end{align}
Theorem \ref{apply 1} yields
\begin{align}
\label{killme1}
\frac{\tn{f(\W_T)-\y}}{\sqrt{n}}\leq \frac{\tn{ \Pi_{\Rcb}(\y)}+ \e^{-\Gamma}\tn{\Pi_{{\Rc}}(\y)}}{\sqrt{n}}+4\zeta.
\end{align}
Using \eqref{main res eq24} for $M_{\mathcal{W}}$
\begin{align}
\label{killme2}
\frac{{\vrn} BM_{\mathcal{W}}}{\sqrt{n}}\leq \frac{2B\sqrt{\K} \dpz(\y)}{\sqrt{n}}+\frac{2B\sqrt{\K}\Gamma\zeta}{\alpha_0}.
\end{align}
Using \eqref{row boundsss3} on row bound $R$ and lower bound on $k$
\begin{align}
\label{killme3}
3{\vrn} B\frac{R^2}{\sqrt{k}}=&\frac{48n\Gamma^2B^3K^2\opnorm{\X}^2}{\vrn\alpha_0^4\sqrt{k}}\nn\\
\le&\frac{c^2\zeta^2}{230\vrn B\log(2n)}\nn\\
\le& \zeta.
\end{align}
Plugging in \eqref{killme1}, \eqref{killme2}, and \eqref{killme3} into \eqref{tempkillme} concludes the proof.
\end{proof}

